Carry Your Fault: A Fault Propagation Attack on Side-Channel Protected LWE-based KEM

Post-quantum cryptographic (PQC) algorithms, especially those based on the learning with errors (LWE) problem, have been subjected to several physical attacks in the recent past. Although the attacks broadly belong to two classes - passive side-channel attacks and active fault attacks, the attack strategies vary significantly due to the inherent complexities of such algorithms. Exploring further attack surfaces is, therefore, an important step for eventually securing the deployment of these algorithms. Also, it is important to test the robustness of the already proposed countermeasures in this regard. In this work, we propose a new fault attack on side-channel secure masked implementation of LWE-based key-encapsulation mechanisms (KEMs) exploiting fault propagation. The attack typically originates due to an algorithmic modification widely used to enable masking, namely the Arithmetic-to-Boolean (A2B) conversion. We exploit the data dependency of the adder carry chain in A2B and extract sensitive information, albeit masking (of arbitrary order) being present. As a practical demonstration of the exploitability of this information leakage, we show key recovery attacks of Kyber, although the leakage also exists for other schemes like Saber. The attack on Kyber targets the decapsulation module and utilizes Belief Propagation (BP) for key recovery. To the best of our knowledge, it is the first attack exploiting an algorithmic component introduced to ease masking rather than only exploiting the randomness introduced by masking to obtain desired faults (as done by Delvaux). Finally, we performed both simulated and electromagnetic (EM) fault-based practical validation of the attack for an open-source first-order secure Kyber implementation running on an STM32 platform.

==> algorithms.tex <==
\section{Algorithms \JPside{This section should be removed once the relevant algorithms are copied in the paper}}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\centering
\caption{Performance breakdown of the implementation of masked comparison algorithms in the Cortex-M4 platform.}
\label{tab:Compararator}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|llllrlrrrrr|rrrrrr}
\hline
\multicolumn{1}{c|}{}                                                                                                                                             &                          &                                  &                          &                          & \multicolumn{6}{c}{Before}                                                                                                                                                     & \multicolumn{1}{l|}{}            & \multicolumn{1}{l}{}             & \multicolumn{5}{c}{Improved}                                                                                                                                                                                                                                                                   \\ \cline{4-18} 
\multicolumn{1}{c|}{\multirow{-2}{*}{Masked Comparator}}                                                                                                          &                          & \multicolumn{1}{c}{Order}        &                          &                          & \multicolumn{2}{c}{1st}                            & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{2nd}        & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{3rd}        & \multicolumn{1}{c|}{}            & \multicolumn{1}{l}{}             & \multicolumn{1}{c}{1st}                                       & \multicolumn{1}{c}{}                                     & \multicolumn{1}{c}{2nd}                                        & \multicolumn{1}{c}{}                                     & \multicolumn{1}{c}{3rd}                                        \\ \hline
                                                                                                                                                                  & \multicolumn{2}{l}{CPU [k]cycles}                           &                          &                          & \multicolumn{2}{r}{649}                            & \textbf{}                        & 2,101                          & \textbf{}                        & 3,594                          & \textbf{}                        & \textbf{}                        & \textbf{586}                                                  &                                                          & \textbf{1,750}                                                 &                                                          & \textbf{2,950}                                                 \\
                                                                                                                                                                  & \multicolumn{1}{l|}{}    & all \texttt{A2B} conversion      &                          &                          & \multicolumn{2}{r}{612}                            &                                  & 2,047                          &                                  & 3,519                          &                                  &                                  & 549                                                           &                                                          & 1,696                                                          &                                                          & 2,875                                                          \\
                                                                                                                                                                  & \multicolumn{1}{l|}{}    & \texttt{BooleanAllBitsOneTest}   &                          &                          & \multicolumn{2}{r}{7}                              &                                  & 22                             &                                  & 38                             &                                  &                                  & 7                                                             &                                                          & 22                                                             &                                                          & 38                                                             \\
                                                                                                                                                                  & \multicolumn{1}{l|}{}    & Other operations                 &                          &                          & \multicolumn{2}{r}{28}                             &                                  & 31                             &                                  & 36                             &                                  &                                  & 28                                                            &                                                          & 31                                                             &                                                          & 36                                                             \\
\multirow{-5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Decompressed} \\ \textbf{comparison}\\ (Section~\ref{subsubsec:decompressed_masked_comparison})\end{tabular}} & \multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}\# random bytes} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \multicolumn{2}{r}{\cellcolor[HTML]{EFEFEF}11,984} & \cellcolor[HTML]{EFEFEF}         & \cellcolor[HTML]{EFEFEF}47,728 & \cellcolor[HTML]{EFEFEF}         & \cellcolor[HTML]{EFEFEF}95,456 & \cellcolor[HTML]{EFEFEF}         & \cellcolor[HTML]{EFEFEF}         & \cellcolor[HTML]{EFEFEF}\textbf{9,360}                        & \cellcolor[HTML]{EFEFEF}\textbf{}                        & \cellcolor[HTML]{EFEFEF}\textbf{37,232}                        & \cellcolor[HTML]{EFEFEF}\textbf{}                        & \cellcolor[HTML]{EFEFEF}\textbf{74,464}                        \\ \hline
                                                                                                                                                                  & \multicolumn{2}{l}{CPU [k]cycles}                           &                          &                          & \multicolumn{2}{r}{{\color[HTML]{000000} 352}}     & {\color[HTML]{000000} \textbf{}} & {\color[HTML]{000000} 1,126}   & {\color[HTML]{000000} \textbf{}} & {\color[HTML]{000000} 1,934}   & {\color[HTML]{000000} \textbf{}} & {\color[HTML]{000000} \textbf{}} & {\color[HTML]{3531FF} \textbf{320}}                           & {\color[HTML]{3531FF} }                                  & {\color[HTML]{3531FF} \textbf{951}}                            & {\color[HTML]{3531FF} }                                  & {\color[HTML]{3531FF} \textbf{1,612}}                          \\
                                                                                                                                                                  & \multicolumn{1}{l|}{}    & all \texttt{A2B} conversion      &                          &                          & \multicolumn{2}{r}{308}                            &                                  & 1,023                          &                                  & 1,766                          &                                  &                                  & 276                                                           &                                                          & 848                                                            &                                                          & 1,444                                                          \\
                                                                                                                                                                  & \multicolumn{1}{l|}{}    & \texttt{BooleanAllBitsOneTest}   &                          &                          & \multicolumn{2}{r}{27}                             &                                  & 83                             &                                  & 143                            &                                  &                                  & 27                                                            &                                                          & 83                                                             &                                                          & 143                                                            \\
                                                                                                                                                                  & \multicolumn{1}{l|}{}    & Other operations                 &                          &                          & \multicolumn{2}{r}{16}                             &                                  & 20                             &                                  & 24                             &                                  &                                  & 16                                                            &                                                          & 20                                                             &                                                          & 24                                                             \\
\multirow{-5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Simple} \\ \textbf{comparison}\\ (Section~\ref{subsubsec:new_masked_comparison})\end{tabular}}           & \multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}\# random bytes} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \multicolumn{2}{r}{\cellcolor[HTML]{EFEFEF}6,672}  & \cellcolor[HTML]{EFEFEF}         & \cellcolor[HTML]{EFEFEF}25,904 & \cellcolor[HTML]{EFEFEF}         & \cellcolor[HTML]{EFEFEF}51,808 & \cellcolor[HTML]{EFEFEF}         & \cellcolor[HTML]{EFEFEF}         & \cellcolor[HTML]{EFEFEF}{\color[HTML]{3531FF} \textbf{5,360}} & \cellcolor[HTML]{EFEFEF}{\color[HTML]{3531FF} \textbf{}} & \cellcolor[HTML]{EFEFEF}{\color[HTML]{3531FF} \textbf{20,656}} & \cellcolor[HTML]{EFEFEF}{\color[HTML]{3531FF} \textbf{}} & \cellcolor[HTML]{EFEFEF}{\color[HTML]{3531FF} \textbf{41,312}} \\ \hline
\end{tabular}%
}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\caption{The comparison between Saber and Kyber regarding the performance and the random bytes requirement.}
\label{tab:performance_comp}
\begin{tabular}{clcccccccccccccc}
\hline
\multicolumn{3}{c}{}                                                                                                             &                      &                      & \multicolumn{11}{c}{CPU [k]cycles}                                                                                                                  \\ \cline{5-16} 
\multicolumn{3}{c}{\multirow{-2}{*}{Scheme}}                                                                                     &                      &                      & No mask &  & 1st            &           &           & 2nd             &           &           & 3rd              &           &                      \\ \hline
                                 & \multicolumn{1}{c}{}                                                   &                      &                      & \multicolumn{12}{c}{Performance     CPU [k]cycles}                                                                                                                         \\ \hline
{\color[HTML]{3531FF} \textbf{}} & {\color[HTML]{000000} \textbf{Higher order masked Saber (this work)}}  &                      &                      &                      & 1,121   &  & 3,146          &           &           & \textbf{5,915}  & \textbf{} & \textbf{} & \textbf{9,237}   & \textbf{} &                      \\
\multicolumn{1}{l}{}             & {\color[HTML]{000000} \textbf{Higher order masked uSaber (this work)}} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 1,062   &  & \textbf{2,546} & \textbf{} & \textbf{} & \textbf{4,702}  & \textbf{} & \textbf{} & \textbf{7,380}   &           & \multicolumn{1}{l}{} \\
\multicolumn{1}{l}{}             & Higher order masked Saber~\cite{BronchainC22}                          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 835     &  & 5,027          &           &           & 7,320           &           &           & 9,988            &           & \multicolumn{1}{l}{} \\
                                 & Higher order masked Kyber~\cite{ho-mask-comparator-kyber-bos-2021}     &                      &                      &                      & 882     &  & 3,116*         &           &           & 44,347          &           &           & 115,481          &           &                      \\
\multicolumn{1}{l}{}             & Higher order masked Kyber~\cite{BronchainC22}                          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 882     &  & 7,716          &           &           & 11,880          &           &           & 16,715           &           & \multicolumn{1}{l}{} \\
                                 & First order masked Saber~\cite{FO-masked-saber}                        &                      &                      &                      & 1,123   &  & 2,833          &           &           & -               &           &           & -                &           &                      \\
                                 & First order masked Kyber~\cite{FO-masked-kyber-HeinzKLPSS22}           &                      &                      &                      & 882     &  & 2,978          &           &           & -               &           &           & -                &           &                      \\
\multicolumn{1}{l}{}             & Saber NTT~\cite{Abdulrahman_Chen_Chen_Hwang_Kannwischer_Yang_2021}     & \multicolumn{1}{l}{} &                      &                      & 835     &  & -              &           &           & -               &           &           & -                &           & \multicolumn{1}{l}{} \\
                                 & Fastest Kyber~\cite{fast-kyber-AbdulrahmanHKS22}                       &                      &                      &                      & 796     &  & -              &           &           & -               &           &           & -                &           &                      \\ \hline
\multicolumn{3}{c}{\textbf{}}                                                                                                    &                      & \multicolumn{12}{c}{# Random bytes}                                                                                                                                        \\ \hline
                                 & {\color[HTML]{000000} \textbf{Higher order masked Saber (this work)}}  &                      &                      &                      & 0       &  & 14,000         &           &           & \textbf{49,072} &           &           & \textbf{104,288} &           &                      \\
                                 & Higher order masked Kyber~\cite{ho-mask-comparator-kyber-bos-2021}     &                      &                      &                      & 0       &  & 12,072*        &           &           & 902,126         &           &           & 2,434,170        &           &                      \\ \hline
\end{tabular}
\text{*: uses optimized implementation for first-order implementation}
\end{table}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\caption{The comparison between Saber and Kyber regarding the performance and the random bytes requirement.}
\label{tab:performance_comp}
\begin{tabular}{clcccccccccccccc}
\hline
\multicolumn{3}{c}{}                                                                                                         &  &  & \multicolumn{11}{c}{CPU [k]cycles}                                                                                         \\ \cline{5-16} 
\multicolumn{3}{c}{\multirow{-2}{*}{Scheme}}                                                                                 &  &  & No mask &  & 1st     &  &  & 2nd             &           &           & 3rd              &           &                      \\ \hline
                                 & \multicolumn{1}{c}{}                                               &                      &  & \multicolumn{12}{c}{Performance     CPU [k]cycles}                                                                            \\ \hline
{\color[HTML]{3531FF} \textbf{}} & {\color[HTML]{3531FF} \textbf{Higher order masked Saber}}                   &                      &  &  & 1,121   &  & 3,902   &  &  & \textbf{6,981}  & \textbf{} & \textbf{} & \textbf{10,601}  & \textbf{} &                      \\
                                 & Higher order masked Kyber~\cite{ho-mask-comparator-kyber-bos-2021} &                      &  &  & 882     &  & 3,116*  &  &  & 44,347          &           &           & 115,481          &           &                      \\
                                 & First order masked Saber~\cite{FO-masked-saber}                    &                      &  &  & 1,123   &  & 2,833   &  &  & -               &           &           & -                &           &                      \\
                                 & First order masked Kyber~\cite{FO-masked-kyber-HeinzKLPSS22}       &                      &  &  & 882     &  & 2,978   &  &  & -               &           &           & -                &           &                      \\
\multicolumn{1}{l}{}             & Saber NTT~\cite{Abdulrahman_Chen_Chen_Hwang_Kannwischer_Yang_2021}                            & \multicolumn{1}{l}{} &  &  & 777     &  & -       &  &  & -               &           &           & -                &           & \multicolumn{1}{l}{} \\
                                 & Fastest Kyber~\cite{fast-kyber-AbdulrahmanHKS22}                   &                      &  &  & 796     &  & -       &  &  & -               &           &           & -                &           &                      \\ \hline
\multicolumn{3}{c}{\textbf{}}                                                                                                &  & \multicolumn{12}{c}{# Random bytes}                                                                                           \\ \hline
                                 & {\color[HTML]{3531FF} \textbf{Higher order masked Saber}}          &                      &  &  & 0       &  & 14,000  &  &  & \textbf{49,072} &           &           & \textbf{104,288} &           &                      \\
                                 & Higher order masked Kyber~\cite{ho-mask-comparator-kyber-bos-2021} &                      &  &  & 0       &  & 12,072* &  &  & 902,126         &           &           & 2,434,170        &           &                      \\ \hline
\end{tabular}
\text{*: uses optimized implementation for first-order implementation}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\centering
\caption{Performance cost of all the modules of higher-order masked decapsulation procedure of Saber.}
\label{tab:masked_saber_performance}
\begin{tabular}{lllllllllccccccccccl}
\hline
                      &  & \multicolumn{5}{l}{}                                                         &  &  & \multicolumn{11}{c}{CPU {[}k{]}cycles}                                                                                                                                                                                         \\ \cline{9-20} 
                      &  & \multicolumn{5}{c}{Order}                                                    &  &  & No mask               &                      & 1st   &                           &                      & 2nd   &                           &                      & 3rd    &                           & \multicolumn{1}{c}{} \\ \hline
\multicolumn{7}{l}{{\color[HTML]{3531FF} \textbf{Saber-Decapsulation}}}                         &  &  & 1,121                 &                      & 3,902 & (3.48x)                   &                      & 6,981 & (6.22x)                   &                      & 10,601 & (9.45x)                   & \multicolumn{1}{c}{} \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{CPA-PKE-Decryption}}                              &  &  & 129                   &                      & 410   & (3.17x)                   &                      & 715   & (5.54x)                   &                      & 1,034  & (8.01x)                   & \multicolumn{1}{c}{} \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial arithmetic}         &  &  & 126                   &                      & 239   & (1.89x)                   &                      & 352   & (2.79x)                   &                      & 467    & (3.70x)                   &                      \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Compression}                   &  &  & 2                     &                      & 171   & (85.5x)                   &                      & 362   & (181x)                    &                      & 566    & (283x)                    &                      \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{Hash $\mathcal{G}$ (SHA3-512)}}                   &  &  & 13                    &                      & 122   & (9.38x)                   &                      & 242   & (18.61x)                  &                      & 378    & (29.07x)                  & \multicolumn{1}{c}{} \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{CPA-PKE-Encryption}}                              &  &  & 853                   &                      & 3,242 & (3.80x)                   &                      & 5,896 & (6.91x)                   &                      & 9,060  & (10.62x)                  & \multicolumn{1}{c}{} \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Secret generation}             &  &  & 69                    &                      & 925   & (13.40x)                  &                      & 2,022 & (29.30x)                  &                      & 3,595  & (52.10x)                  &                      \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & XOF (SHAKE-128)        &  &  & 63                    &                      & 611   & (9.69x)                   &                      & 1,210 & (19.20x)                  &                      & 1,887  & (29.95x)                  &                      \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & CBD (Binomial Sampler) &  &  & 6                     &                      & 314   & (52.33x)                  &                      & 811   & (135.16x)                 &                      & 1,708  & (284.66x)                 &                      \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial arithmetic}         &  &  &                       & \multicolumn{1}{l}{} & 1,234 &                           & \multicolumn{1}{l}{} & 1,688 &                           & \multicolumn{1}{l}{} & 2,135  &                           &                      \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial Comparison}         &  &  & \multirow{-2}{*}{783} & \multicolumn{1}{l}{} & 1,082 & \multirow{-2}{*}{(2.95x)} & \multicolumn{1}{l}{} & 2,186 & \multirow{-2}{*}{(4.94x)} & \multicolumn{1}{l}{} & 3,329  & \multirow{-2}{*}{(6.97x)} &                      \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{Other operations}                                         &  &  & 126                   &                      & 127   & (1.00x)                   &                      & 127   & (1.00x)                   &                      & 127    & (1.00x)                   & \multicolumn{1}{c}{} \\ \hline
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\centering
\caption{Performance breakdown of the implementation of masked comparison algorithms in the Cortex-M4 platform.}
\label{tab:Compararator}
\begin{tabular}{lllllclcccccccccccl}
\hline
     &     & \multicolumn{1}{c}{}                           &  &  & \multicolumn{13}{c}{CPU [k]cycles}                                                                                                                                                                                                                                                                                                                                              &                      \\ \cline{5-19} 
     &     & \multicolumn{1}{c}{\multirow{-2}{*}{Order}}    &  &  & \multicolumn{2}{c}{1st}                                   &                         & 2nd                                   &  & 3rd                                   &                         & 4th                                   &                         & 5th                                   &                         & 6th                                   &  &                      \\ \hline
\multicolumn{3}{l}{\textbf{Decompressed comparison} [Section~\ref{subsubsec:decompressed_masked_comparison}]} &  &  & \multicolumn{2}{c}{\textbf{1,731}}                        &                         & \textbf{3,643}                        &  & \textbf{5,691}                        &                         & \textbf{8,744}                        &                         & \textbf{11,854}                       &                         & \textbf{15,879}                       &  &                      \\
     &     & all \texttt{A2B} conversion                    &  &  & \multicolumn{2}{c}{1,627}                                 &                         & 3,493                                 &  & 5,498                                 &                         & 8,490                                 &                         & 11,541                                &                         & 15,511                                &  &                      \\
     &     & \texttt{BooleanAllBitsOneTest}                 &  &  & \multicolumn{2}{c}{7}                                     &                         & 22                                    &  & 38                                    &                         & 64                                    &                         & 87                                    &                         & 119                                   &  &                      \\
     &     & Other operations                               &  &  & \multicolumn{2}{c}{97}                                    &                         & 128                                   &  & 155                                   &                         & 190                                   &                         & 226                                   &                         & 249                                   &  &                      \\ \hline
\multicolumn{3}{l}{\textbf{New masked comparison} [Section~\ref{subsubsec:new_masked_comparison}]}          &  &  & \multicolumn{2}{c}{{\color[HTML]{3531FF} \textbf{1,082}}} & {\color[HTML]{3531FF} } & {\color[HTML]{3531FF} \textbf{2,186}} &  & {\color[HTML]{3531FF} \textbf{3,329}} & {\color[HTML]{3531FF} } & {\color[HTML]{3531FF} \textbf{5,060}} & {\color[HTML]{3531FF} } & {\color[HTML]{3531FF} \textbf{6,800}} & {\color[HTML]{3531FF} } & {\color[HTML]{3531FF} \textbf{8,950}} &  &                      \\
     &     & all \texttt{A2B} conversion                    &  &  & \multicolumn{2}{c}{813}                                   &                         & 1,749                                 &  & 2,749                                 &                         & 4,248                                 &                         & 5,778                                 &                         & 7,758                                 &  &                      \\
     &     & \texttt{BooleanAllBitsOneTest}                 &  &  & \multicolumn{2}{c}{27}                                    &                         & 83                                    &  & 144                                   &                         & 241                                   &                         & 326                                   &                         & 448                                   &  &                      \\
     &     & Other operations                               &  &  & \multicolumn{2}{c}{242}                                   &                         & 354                                   &  & 436                                   &                         & 571                                   &                         & 696                                   &                         & 744                                   &  &                      \\ \hline
\multicolumn{3}{l}{\cite{ho-mask-comparator-D'Anvers2021}}  &  &  & \multicolumn{2}{c}{\textbf{1,510}}                        &                         & \textbf{3,363}                        &  & \textbf{6,543}                        &                         &                                       &                         &                                       &                         &                                       &  &                      \\
     &     & all \texttt{A2B} conversion                    &  &  & \multicolumn{2}{c}{978}                                   &                         & 1,926                                 &  & 3,015                                 &                         &                                       &                         &                                       &                         &                                       &  & \multicolumn{1}{c}{} \\
     &     & \texttt{BooleanAllBitsOneTest}                 &  &  & \multicolumn{2}{c}{27}                                    &                         & 73                                    &  & 128                                   &                         &                                       &                         &                                       &                         &                                       &  & \multicolumn{1}{c}{} \\
     &     & Other operations                               &  &  & \multicolumn{2}{c}{505}                                   &                         & 1,362                                 &  & 3,402                                 &                         &                                       &                         &                                       &                         &                                       &  & \multicolumn{1}{c}{} \\ \hline
\end{tabular}
\end{table}

\begin{algorithm}[!ht]
\caption{ Secure computation of \texttt{MSB} using~\cite{Coron2014_A2B} }
\label{algo:A2B}

\Input{$\{A_i\}_{1\leq i \leq n}$ such that $\sum_{i=1}^{n} A_i \mod{q}= {x} \in \mathbb{R}_q $}
\Output{$\{y_i\}_{1\leq i \leq n}$ where each $ y_i \in \mathbb{R}_2$ and $\bigoplus_{i=1}^{n} y_i = \texttt{MSB}(x)$}
\BlankLine
\If{$n=1$} {$y_1 \leftarrow A_1$\\ \algorithmicreturn{ $y_1$}} 
\Else{
$\{u_i\}_{1\leq i \leq \lfloor n/2\rfloor} \leftarrow \mathtt{A2B} (\{A_i\}_{1\leq i \leq \lfloor n/2\rfloor})$\\
$\{u_i\}_{1\leq i \leq n} \leftarrow \mathtt{RefreshXOR} (\{u_i\}_{1\leq i \leq \lfloor n/2\rfloor},n,k)$\\
$\{v_i\}_{1\leq i \leq \lceil n/2\rceil} \leftarrow \mathtt{A2B} (\{A_i\}_{\lfloor n/2\rfloor + 1\leq i \leq n })$\\
$\{v_i\}_{1\leq i \leq n} \leftarrow \mathtt{RefreshXOR}(\{v_i\}_{1\leq i \leq \lfloor n/2\rfloor},n,k)$\\
$\{y_i\}_{1\leq i \leq n} \leftarrow \mathtt{SecAdd}(\{u_i\}_{1\leq i \leq n},\{v_i\}_{1\leq i \leq n})$\\
\algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}
}
\end{algorithm}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\caption{}
\label{tab:performance_comp}
\begin{tabular}{lllllccccccccccc}
\hline
     & \multicolumn{2}{c}{}                               &  & \multicolumn{12}{c}{Order}                                                                                                                                                                                                 \\ \cline{5-16} 
     & \multicolumn{2}{c}{\multirow{-2}{*}{Scheme}}       &  &  & No mask & \multicolumn{1}{l}{} & 1st     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 2nd             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 3rd              & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
     &                & \multicolumn{1}{c}{}              &  & \multicolumn{12}{c}{Performance   CPU [k]cycles}                                                                                                                                                                           \\ \hline
\multicolumn{3}{l}{{\color[HTML]{3531FF} \textbf{Saber}}} &  &  & 1,121   &                      & 3,902   & (1.25x)              &                      & \textbf{6,981}  & (0.15x)              &                      & \textbf{10,601}  & (0.09x)              &                      \\
\multicolumn{3}{l}{Kyber}                                 &  &  & 882     &                      & 3,116*  &                      &                      & 44,347          &                      &                      & 115,481          &                      &                      \\ \hline
     &                &                                   &  & \multicolumn{12}{c}{\# Random bytes}                                                                                                                                                                                       \\ \hline
\multicolumn{3}{l}{{\color[HTML]{3531FF} \textbf{Saber}}} &  &  & 0       &                      & 14,000  & (1.25x)              &                      & \textbf{49,072} & (0.05x)              & \textbf{}            & \textbf{104,288} & (0.04x)              & \textbf{}            \\
\multicolumn{3}{l}{Kyber}                                 &  &  & 0       &                      & 12,072* &                      &                      & 902,126         &                      &                      & 2,434,170        &                      &                      \\ \hline
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage{lscape}
\begin{landscape}
\begin{table}[]
\caption{Performance cost and the randomness cost of all the modules of higher-order masked Saber-CCA-KEM-Decapsulation}
\label{tab:masked-saber-decaps}
\begin{tabular}{llll|lclccccccccccccc|lcccccccl}
\hline
                &                 &                                             &  &  & \multicolumn{15}{c|}{CPU [k]cycles}                                                                                                                                                   & \multicolumn{8}{c}{# Random bytes}          & \multicolumn{1}{c}{} \\ \cline{5-29} 
                &                 & \multicolumn{1}{c}{Order}                   &  &  & No mask               &  &  & 1st  &                           &  & 2nd  &                           &  & 3rd   &                           &  & 4th   & \multicolumn{1}{l}{}      &  &  & 1st   &  & 2nd   &  & 3rd    &  & 4th    &                      \\ \hline
\multicolumn{3}{l}{{\color[HTML]{3531FF} \textbf{Saber-CCA-KEM-Decapsulation}}} &  &  & 1121                  &  &  & 3902 & (3.48x)                   &  & 6981 & (6.22x)                   &  & 10601 & (9.45x)                   &  & 16383 & (14.61x)                  &  &  & 14000 &  & 49072 &  & 104288 &  & 199936 &                      \\
                &                 & CPA-PKE-Decryption                          &  &  & 129                   &  &  & 410  & (3.17x)                   &  & 715  & (5.54x)                   &  & 1034  & (8.01x)                   &  & 1453  & (11.26x)                  &  &  & 1184  &  & 4736  &  & 9472   &  & 17760  &                      \\
                &                 & Hash $\mathcal{G}$ (SHA3-512)               &  &  & 13                    &  &  & 122  & (9.38x)                   &  & 242  & (18.61x)                  &  & 378   & (29.07x)                  &  & 631   & (48.53x)                  &  &  & 192   &  & 576   &  & 1152   &  & 1920   &                      \\
                &                 & CPA-PKE-Encryption                          &  &  & 853                   &  &  & 3242 & (3.80x)                   &  & 5896 & (6.91x)                   &  & 9060  & (10.62x)                  &  & 14169 & (16.61x)                  &  &  & 12624 &  & 43760 &  & 93664  &  & 180256 &                      \\
                &                 & Other operations                            &  &  & 126                   &  &  & 127  & (1.00x)                   &  & 127  & (1.00x)                   &  & 127   & (1.00x)                   &  & 128   & (1.01x)                   &  &  & 0     &  & 0     &  & 0      &  & 0      &                      \\ \hline
\multicolumn{3}{l}{\textbf{CPA-PKE-Decryption}}                                 &  &  & 129                   &  &  & 410  & (3.17x)                   &  & 715  & (5.54x)                   &  & 1034  & (8.01x)                   &  & 1453  & (11.26)                   &  &  & 1184  &  & 4736  &  & 9472   &  & 17760  &                      \\
                &                 & Polynomial arithmetic                       &  &  & 126                   &  &  & 239  & (1.89x)                   &  & 352  & (2.79x)                   &  & 467   & (3.70x)                   &  & 580   & (4.60x)                   &  &  & 0     &  & 0     &  & 0      &  & 0      &                      \\
                &                 & Compression                                 &  &  & 2                     &  &  & 171  & (85.5x)                   &  & 362  & (181x)                    &  & 566   & (283x)                    &  & 872   & (436x)                    &  &  & 1184  &  & 4736  &  & 9472   &  & 17760  &                      \\ \hline
\multicolumn{3}{l}{\textbf{CPA-PKE-Encryption}}                                 &  &  & 853                   &  &  & 3242 & (3.80x)                   &  & 5896 & (6.91x)                   &  & 9060  & (10.62x)                  &  & 14169 & (16.61x)                  &  &  & 12624 &  & 43760 &  & 93664  &  & 180256 &                      \\
                &                 & Secret generation                           &  &  & 69                    &  &  & 925  & (13.40x)                  &  & 2022 & (29.30x)                  &  & 3595  & (52.10x)                  &  & 6514  & (94.40x)                  &  &  & 5952  &  & 17856 &  & 41856  &  & 84096  &                      \\
                &                 & Polynomial arithmetic                       &  &  &                       &  &  & 1234 &                           &  & 1688 &                           &  & 2135  &                           &  & 2593  &                           &  &  & 0     &  & 0     &  & 0      &  & 0      &                      \\
                &                 & Polynomial Comparison                       &  &  & \multirow{-2}{*}{783} &  &  & 1082 & \multirow{-2}{*}{(2.95x)} &  & 2186 & \multirow{-2}{*}{(4.94x)} &  & 3329  & \multirow{-2}{*}{(6.97x)} &  & 5060  & \multirow{-2}{*}{(9.77x)} &  &  & 6672  &  & 25904 &  & 51808  &  & 96160  &                      \\ \hline
\multicolumn{3}{l}{\textbf{Secret generation}}                                  &  &  & 69                    &  &  & 925  & (13.40x)                  &  & 2022 & (29.30x)                  &  & 3595  & (52.10x)                  &  & 6514  & (94.40x)                  &  &  & 5952  &  & 17856 &  & 41856  &  & 84096  &                      \\
                &                 & XOF (SHAKE-128)                             &  &  & 63                    &  &  & 611  & (9.69x)                   &  & 1210 & (19.20x)                  &  & 1887  & (29.95x)                  &  & 3150  & (50.00x)                  &  &  & 960   &  & 2880  &  & 5760   &  & 9600   &                      \\
                &                 & CBD (Binomial Sampler)                      &  &  & 6                     &  &  & 314  & (52.33x)                  &  & 811  & (135.16x)                 &  & 1708  & (284.66x)                 &  & 3364  & (560.66x)                 &  &  & 4992  &  & 14976 &  & 36096  &  & 74496  &                      \\ \hline
\end{tabular}
\end{table}
\end{landscape}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{}
\label{tab:my-table}
\begin{tabular}{lllllcccccccccccccl}
\hline
                &                 &                                             &  &  & \multicolumn{14}{c}{CPU [k]cycles}                                                                                                                                                 \\ \cline{5-19} 
                &                 & \multicolumn{1}{c}{Order}                   &  &  & No mask               &  & 1st  &                           &  & 2nd  &                           &  & 3rd   &                           &  & 4th   & \multicolumn{1}{l}{}      &  \\ \hline
\multicolumn{3}{l}{{\color[HTML]{3531FF} \textbf{Saber-CCA-KEM-Decapsulation}}} &  &  & 1121                  &  & 3902 & (3.48x)                   &  & 6981 & (6.22x)                   &  & 10601 & (9.45x)                   &  & 16383 & (14.61x)                  &  \\
                &                 & CPA-PKE-Decryption                          &  &  & 129                   &  & 410  & (3.17x)                   &  & 715  & (5.54x)                   &  & 1034  & (8.01x)                   &  & 1453  & (11.26x)                  &  \\
                &                 & Hash $\mathcal{G}$ (SHA3-512)               &  &  & 13                    &  & 122  & (9.38x)                   &  & 242  & (18.61x)                  &  & 378   & (29.07x)                  &  & 631   & (48.53x)                  &  \\
                &                 & CPA-PKE-Encryption                          &  &  & 853                   &  & 3242 & (3.80x)                   &  & 5896 & (6.91x)                   &  & 9060  & (10.62x)                  &  & 14169 & (16.61x)                  &  \\
                &                 & Other operations                            &  &  & 126                   &  & 127  & (1.00x)                   &  & 127  & (1.00x)                   &  & 127   & (1.00x)                   &  & 128   & (1.01x)                   &  \\ \hline
\multicolumn{3}{l}{\textbf{CPA-PKE-Decryption}}                                 &  &  & 129                   &  & 410  & (3.17x)                   &  & 715  & (5.54x)                   &  & 1034  & (8.01x)                   &  & 1453  & (11.26)                   &  \\
                &                 & Polynomial arithmetic                       &  &  & 126                   &  & 239  & (1.89x)                   &  & 352  & (2.79x)                   &  & 467   & (3.70x)                   &  & 580   & (4.60x)                   &  \\
                &                 & Compression                                 &  &  & 2                     &  & 171  & (85.5x)                   &  & 362  & (181x)                    &  & 566   & (283x)                    &  & 872   & (436x)                    &  \\ \hline
\multicolumn{3}{l}{\textbf{CPA-PKE-Encryption}}                                 &  &  & 853                   &  & 3242 & (3.80x)                   &  & 5896 & (6.91x)                   &  & 9060  & (10.62x)                  &  & 14169 & (16.61x)                  &  \\
                &                 & Secret generation                           &  &  & 69                    &  & 925  & (13.40x)                  &  & 2022 & (29.30x)                  &  & 3595  & (52.10x)                  &  & 6514  & (94.40x)                  &  \\
                &                 & Polynomial arithmetic                       &  &  &                       &  & 1234 &                           &  & 1688 &                           &  & 2135  &                           &  & 2593  &                           &  \\
                &                 & Comparison                       &  &  & \multirow{-2}{*}{783} &  & 1082 & \multirow{-2}{*}{(2.95x)} &  & 2186 & \multirow{-2}{*}{(4.94x)} &  & 3329  & \multirow{-2}{*}{(6.97x)} &  & 5060  & \multirow{-2}{*}{(9.77x)} &  \\ \hline
\multicolumn{3}{l}{\textbf{Secret generation}}                                  &  &  & 69                    &  & 925  & (13.40x)                  &  & 2022 & (29.30x)                  &  & 3595  & (52.10x)                  &  & 6514  & (94.40x)                  &  \\
                &                 & XOF (SHAKE-128)                             &  &  & 63                    &  & 611  & (9.69x)                   &  & 1210 & (19.20x)                  &  & 1887  & (29.95x)                  &  & 3150  & (50.00x)                  &  \\
                &                 & CBD (Binomial Sampler)                      &  &  & 6                     &  & 314  & (52.33x)                  &  & 811  & (135.16x)                 &  & 1708  & (284.66x)                 &  & 3364  & (560.66x)                 &  \\ \hline
\end{tabular}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{}
\label{tab:my-table}
\begin{tabular}{lllllccccccccl}
\hline
                &                 &                                             &  &  & \multicolumn{9}{c}{Random bytes}                 \\ \cline{6-14} 
                &                 & \multicolumn{1}{c}{Order}                   &  &  &  & 1st   &  & 2nd   &  & 3rd    &  & 4th    &  \\ \hline
\multicolumn{3}{l}{{\color[HTML]{3531FF} \textbf{Saber-CCA-KEM-Decapsulation}}} &  &  &  & 14000 &  & 49072 &  & 104288 &  & 199936 &  \\
                &                 & CPA-PKE-Decryption                          &  &  &  & 1184  &  & 4736  &  & 9472   &  & 17760  &  \\
                &                 & Hash $\mathcal{G}$ (SHA3-512)               &  &  &  & 192   &  & 576   &  & 1152   &  & 1920   &  \\
                &                 & CPA-PKE-Encryption                          &  &  &  & 12624 &  & 43760 &  & 93664  &  & 180256 &  \\
                &                 & Other operations                            &  &  &  & 0     &  & 0     &  & 0      &  & 0      &  \\ \hline
\multicolumn{3}{l}{\textbf{CPA-PKE-Decryption}}                                 &  &  &  & 1184  &  & 4736  &  & 9472   &  & 17760  &  \\
                &                 & Polynomial arithmetic                       &  &  &  & 0     &  & 0     &  & 0      &  & 0      &  \\
                &                 & Compression                                 &  &  &  & 1184  &  & 4736  &  & 9472   &  & 17760  &  \\ \hline
\multicolumn{3}{l}{\textbf{CPA-PKE-Encryption}}                                 &  &  &  & 12624 &  & 43760 &  & 93664  &  & 180256 &  \\
                &                 & Secret generation                           &  &  &  & 5952  &  & 17856 &  & 41856  &  & 84096  &  \\
                &                 & Polynomial arithmetic                       &  &  &  & 0     &  & 0     &  & 0      &  & 0      &  \\
                &                 & Polynomial Comparison                       &  &  &  & 6672  &  & 25904 &  & 51808  &  & 96160  &  \\ \hline
\multicolumn{3}{l}{\textbf{Secret generation}}                                  &  &  &  & 5952  &  & 17856 &  & 41856  &  & 84096  &  \\
                &                 & XOF (SHAKE-128)                             &  &  &  & 960   &  & 2880  &  & 5760   &  & 9600   &  \\
                &                 & CBD (Binomial Sampler)                      &  &  &  & 4992  &  & 14976 &  & 36096  &  & 74496  &  \\ \hline
\end{tabular}
\end{table}








\begin{figure}[ht!]
\centering
  \includegraphics[scale=.1]{saber_draw.png}
  \caption{Saber-KEM-Decapsulation}
  \label{fig:Decapsulation}
\end{figure}

\begin{algorithm}[!ht]
\caption{ Secure Arithmetic to Boolean conversion (A2B)~\cite{Coron2014_A2B} }
\label{algo:A2B}

\Input{$\{A_i\}_{1\leq i \leq n}$ such that $\sum_{i=1}^{n} A_i = {x} \in \mathbb{R}_q $}
\Output{$\{y_i\}_{1\leq i \leq n}$ where each $ y_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{n} y_i = x$}
\BlankLine
\If{$n=1$} {$y_1 \leftarrow A_1$\\ \algorithmicreturn{ $y_1$}} 
\Else{
$\{u_i\}_{1\leq i \leq \lfloor n/2\rfloor} \leftarrow \mathtt{A2B} (\{A_i\}_{1\leq i \leq \lfloor n/2\rfloor})$\\
$\{u_i\}_{1\leq i \leq n} \leftarrow \mathtt{RefreshXOR} (\{u_i\}_{1\leq i \leq \lfloor n/2\rfloor},n,k)$\\
$\{v_i\}_{1\leq i \leq \lceil n/2\rceil} \leftarrow \mathtt{A2B} (\{A_i\}_{\lfloor n/2\rfloor + 1\leq i \leq n })$\\
$\{v_i\}_{1\leq i \leq n} \leftarrow \mathtt{RefreshXOR}(\{v_i\}_{1\leq i \leq \lfloor n/2\rfloor},n,k)$\\
$\{y_i\}_{1\leq i \leq n} \leftarrow \mathtt{SecAdd}(\{u_i\}_{1\leq i \leq n},\{v_i\}_{1\leq i \leq n})$\\
\algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}
}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{ RefreshXOR~\cite{Coron2014_A2B}}
\label{algo:RefreshXOR}

\Input{$(\{x_i\}_{1\leq i \leq m}, n, k)$ where each $x_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{m} x_i = x$}
\Output{$\{y_i\}_{1\leq i \leq n}$ with each $y_i \in \mathbb{R}_2^k$ such that $\bigoplus_{i=1}^{n} y_i = x$}
\BlankLine
\For{\texttt{i=1 to n}}
{
    $y_i\leftarrow x_i$\\
}
\For{\texttt{i=1 to n-1}}
{
   \For{\texttt{j=i+1 to n}}
    {
        $r\leftarrow \mathcal{U}(\mathbb{R}_2^k)$\\
        $y_i\leftarrow y_i\xor r$\\
        $y_j\leftarrow y_j\xor r$\\
    }
}
\algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}

\end{algorithm}

\begin{algorithm}[!ht]
\caption{ SecAdd~\cite{Coron2014_A2B} }
\label{algo:SecAdd}

\Input{$\{x_i\}_{1\leq i \leq n}$, $\{y_i\}_{1\leq i \leq n}$ with each $x_i,y_i \in \mathbb{R}_2^k$ such that $\bigoplus_{i=1}^{m} x_i = x$ and $\bigoplus_{i=1}^{m} y_i = y$}
\Output{$\{z_i\}_{1\leq i \leq n}$ where each $z_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{m} z_i = x+y \mod{2^k}$}
\BlankLine
\For{\texttt{i=1 to n}}
{
    $u_i\leftarrow x_i+y_i$\\
}
$\{g_i\}_{1\leq i \leq n} \leftarrow \mathtt{SecAnd}(\{x_i\}_{1\leq i \leq n},\{y_i\}_{1\leq i \leq n})$\\
$w\leftarrow \lceil \log_2(k-1) +1 \rceil $\\
\For{\texttt{j=1 to w}}
{
    $p\leftarrow 2^{j-1}$\\
    \For{\texttt{i=1 to n}}
    {
        $v_i\leftarrow g_i<<p$\\
    }
    $\{v_i\}_{1\leq i \leq n}\leftarrow \mathtt{SecAnd}(\{u_i\}_{1\leq i \leq n},\{v_i\}_{1\leq i \leq n})$\\
    \For{\texttt{i=1 to n}}
    {
        $g_i\leftarrow g_i\xor v_i$\\
        $a_i\leftarrow u_i<<p$
    }
    $\{a_i\}_{1\leq i \leq n} \leftarrow \mathtt{RefreshXOR}(\{a_i\}_{1\leq i \leq n},n,k)$\\
    $\{u_i\}_{1\leq i \leq n}\leftarrow \mathtt{SecAnd}(\{u_i\}_{1\leq i \leq n},\{a_i\}_{1\leq i \leq n})$\\
}
\For{\texttt{i=1 to n}}
{
    $v_i\leftarrow g_i<< 2^w$\\
}
$\{v_i\}_{1\leq i \leq n}\leftarrow \mathtt{SecAnd}(\{u_i\}_{1\leq i \leq n},\{v_i\}_{1\leq i \leq n})$\\
\For{\texttt{i=1 to n}}
{
    $g_i\leftarrow g_i\xor a$\\
    $g_i\leftarrow g_i<<1$
    $z_i\leftarrow x_i\xor y_i\xor g_i$\\
}
\algorithmicreturn{ $\{z_i\}_{1\leq i \leq n}$}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{ SecAnd~\cite{Coron2014_A2B} }
\label{algo:SecAnd}

\Input{$\{x_i\}_{1\leq i \leq n}$, $\{y_i\}_{1\leq i \leq n}$ with each $x_i,y_i \in \mathbb{R}_2^k$ such that $\bigoplus_{i=1}^{m} x_i = x$ and $\bigoplus_{i=1}^{m} y_i = y$}
\Output{$\{z_i\}_{1\leq i \leq n}$ where each $z_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{m} z_i = x \wedge y $}
\BlankLine
\For{\texttt{i=1 to n}}
{
    $z_i\leftarrow x_i\wedge y_i$\\
}
\For{\texttt{i=1 to n-1}}
{
   \For{\texttt{j=i+1 to n}}
    {
        $r_{i,j}\leftarrow \mathcal{U}(\mathbb{R}_2^k)$\\
        $r_{j,i}\leftarrow (x_i\wedge y_j)\xor r_{i,j}$\\
        $r_{j,i}\leftarrow (x_j\wedge y_i)\xor r_{j,i}$\\
        $z_i\leftarrow z_i\xor r_{i,j}$\\
        $z_j\leftarrow z_j\xor r_{j,i}$\\
    }
}
\algorithmicreturn{ $\{z_i\}_{1\leq i \leq n}$}
\end{algorithm}


\begin{algorithm}[!ht]
\caption{ SecBitAdd~\cite{Tobias2019_binomial_sampler} }
\label{algo:SecBitAdd}

\Input{$\{x_i\}_{1\leq i \leq n}$ where $x_i \in \mathbb{R}_2^\kappa$ such that $\bigoplus_{i=1}^{n} x_i = x$ and $\lambda=\lceil \log_2(\kappa+1)\rceil+1$}
\Output{$\{z_i\}_{1\leq i \leq n}$ where each $z_i \in \mathbb{R}_2^\lambda$ and $\bigoplus_{i=1}^{n} z_i =$ HW$(x) $}
\BlankLine

$\{z_i\}_{1\leq i \leq n}\leftarrow 0$\\
\For{\texttt{j=1 to $\kappa$}}
{
   $\{t_i[1]\}_{1\leq i \leq n}\leftarrow \{z_i[1]\}_{1\leq i \leq n} \xor \{x_i[j]\}_{1\leq i \leq n}$ \\
   $\{w_i\}_{1\leq i \leq n}\leftarrow \{x_i[j]\}_{1\leq i \leq n}$ \\
   \For{\texttt{l=2 to $\lambda$}}
    {
       $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\{z_i[l-1]\}_{1\leq i \leq n})$ \\
       $\{t_i[l]\}_{1\leq i \leq n}\leftarrow \{z_i[l]\}_{1\leq i \leq n} \xor \{w_i\}_{1\leq i \leq n}$ \\
    }
    $\{z_i\}_{1\leq i \leq n}\leftarrow \{t_i\}_{1\leq i \leq n}$\\
}
\algorithmicreturn{ $\{z_i\}_{1\leq i \leq n}$}
\end{algorithm}


\begin{algorithm}[!ht]
\caption{ SecBitSub~\cite{Tobias2019_binomial_sampler} }
\label{algo:SecBitSub}

\Input{$\{y_i\}_{1\leq i \leq n},\{z_i\}_{1\leq i \leq n}$ where $y_i,z_i \in \mathbb{R}_2^\kappa$ such that $\bigoplus_{i=1}^{n} y_i = y, \bigoplus_{i=1}^{n} z_i = z$ and $\lambda=\lceil \log_2(\kappa+1)\rceil+1$}
\Output{$\{z_i\}_{1\leq i \leq n}$ where each $z_i \in \mathbb{R}_2^\lambda$ and $\bigoplus_{i=1}^{m} z_i = z-$HW$(y) $}
\BlankLine

$\{t_i\}_{1\leq i \leq n}\leftarrow 0$\\
\For{\texttt{j=1 to $\kappa$}}
{
   $\{t_i[1]\}_{1\leq i \leq n}\leftarrow \{z_i[1]\}_{1\leq i \leq n} \xor \{y_i[j]\}_{1\leq i \leq n}$ \\
   $\{w_i\}_{1\leq i \leq n}\leftarrow \{y_i[j]\}_{1\leq i \leq n}$ \\
   \For{\texttt{l=2 to $\lambda$}}
    {
        $\{u_i[l]\}_{1\leq i \leq n}\leftarrow \{z_i[l-1]\}_{1\leq i \leq n}$ \\
        $u_1\leftarrow ~u_1$ \\
        $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\{u_i\}_{1\leq i \leq n})$ \\
        $\{t_i[l]\}_{1\leq i \leq n}\leftarrow \{z_i[l]\}_{1\leq i \leq n} \xor \{w_i\}_{1\leq i \leq n}$ \\
    }
    $\{z_i\}_{1\leq i \leq n}\leftarrow \{t_i\}_{1\leq i \leq n}$\\
}
\algorithmicreturn{ $\{z_i\}_{1\leq i \leq n}$}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{ SecConstAdd~\cite{Tobias2019_binomial_sampler} }
\label{algo:SecConstAdd}

\Input{$\{x_i\}_{1\leq i \leq n}$ where $x_i \in \mathbb{R}_2^\lambda$ such that $\bigoplus_{i=1}^{n} x_i = x$}
\Output{$\{y_i\}_{1\leq i \leq n}$ where each $y_i \in \mathbb{R}_2^\lambda$ and $\bigoplus_{i=1}^{n} y_i =x+4 $}
\BlankLine

$\{y_i\}_{1\leq i \leq n}\leftarrow \{x_i\}_{1\leq i \leq n}$\\
$\{y_i[3]\}_{1\leq i \leq n}\leftarrow \{y_i[3]\}_{1\leq i \leq n} \xor \{y_i[2]\}_{1\leq i \leq n}$\\
$y_0[2]\leftarrow y_0[2]\xor 1$\\

\algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}
\end{algorithm}


% \begin{algorithm}[!ht]
% \caption{ Binomial Sampler (SecSampler)~\cite{Tobias2019_binomial_sampler} }
% \label{algo:SecSampler}

% \Input{$\{x_i\}_{1\leq i \leq n},\{y_i\}_{1\leq i \leq n}$ where $x_i,y_i \in \mathbb{R}_2^\kappa$ such that $\bigoplus_{i=1}^{n} x_i = x, \bigoplus_{i=1}^{n} y_i = y$}
% \Output{$\{A_i\}_{1\leq i \leq n}$ where  $A_i \in \mathbb{R}_q$ and $\sum_{i=1}^{n} A_i =$ HW$(x)-$ HW$(y) \mod q $}
% \BlankLine

% $\{z_i\}_{1\leq i \leq n}\leftarrow$ SecBitAdd$(\{x_i\}_{1\leq i \leq n})$\\
% $\{z_i\}_{1\leq i \leq n}\leftarrow$ SecBitSub$(\{z_i\}_{1\leq i \leq n},\{y_i\}_{1\leq i \leq n})$\\
% $\{z_i\}_{1\leq i \leq n}\leftarrow$ SecConstAdd$(\{z_i\}_{1\leq i \leq n})$\\
% $\{A_i\}_{1\leq i \leq n}\leftarrow$ B2A$(\{z_i\}_{1\leq i \leq n})$\\
% $A_1\leftarrow A_1-\kappa \mod q$\\

% \algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}
% \end{algorithm}












\begin{algorithm}[!ht]
\caption{ Secure Boolean to Arithmetic conversion (B2A)~\cite{Bettale2018_B2A} }
\label{algo:B2A}

\Input{$\{y_i\}_{1\leq i \leq n}$ where each $ y_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{n} y_i = x$}
\Output{$\{A_i\}_{1\leq i \leq n}$ such that $\sum_{i=1}^{n} A_i = {x} \in \mathbb{R}_q $}

\BlankLine
$\{A_i\}_{1\leq i \leq n} \leftarrow \mathtt{RecB2A}(\{y_i\}_{1\leq i \leq n},0)$\\
\algorithmicreturn{ $\{A_i\}_{1\leq i \leq n}$}

\end{algorithm}


\begin{algorithm}[!ht]
\caption{ RecB2A (n+1 shares to n shares)~\cite{Bettale2018_B2A} }
\label{algo:B2A}

\Input{$\{y_i\}_{1\leq i \leq n+1}$ where each $ y_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{n+1} y_i = x$}
\Output{$\{A_i\}_{1\leq i \leq n}$ such that $\sum_{i=1}^{n} A_i = {x} \in \mathbb{R}_q $}

\BlankLine

\If{n=1}{
$A_1\leftarrow x_1\xor x_2$\\
\algorithmicreturn{ $A_1$}
}
\Else{
$\{z_i\}_{1\leq i \leq n+1}\leftarrow RefreshMask(\{y_i\}_{1\leq i \leq n+1},k)$\\
$x_1\leftarrow \overline{(n\wedge 1)}\cdot z_1 \xor ((z_1\xor z_2)-z_2)$\\
\For{\texttt{i=2 to n}}
{
    $x_i\leftarrow(z_1\xor z_{i+1}) - z_{i+1}$\\
}
$\{B_i\}_{1\leq i \leq n} \leftarrow \mathtt{RecB2A}(\{z_i\}_{2\leq i \leq n+1})$\\
$\{C_i\}_{1\leq i \leq n} \leftarrow \mathtt{RecB2A}(\{x_i\}_{1\leq i \leq n})$\\
\For{\texttt{i=1 to n-2}}
{
    $A_i\leftarrow B_i+C_i$\\
}
$A_{n-1}\leftarrow B_{n-1}$\\
$A_{n}\leftarrow C_{n-1}$\\
\algorithmicreturn{$\{A_i\}_{1\leq i \leq n}$}}

\end{algorithm}


\begin{algorithm}[!ht]
\caption{ RefreshMask~\cite{Bettale2018_B2A} }
\label{algo:RefreshMask}

\Input{$(\{x_i\}_{1\leq i \leq n}, k)$ where each $x_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{n} x_i = x$}
\Output{$\{y_i\}_{1\leq i \leq n}$ with each $y_i \in \mathbb{R}_2^k$ such that $\bigoplus_{i=1}^{n} y_i = x$}

\BlankLine

$y_1\leftarrow x_1$\\

\For{\texttt{i=2 to n}}
{
   $r\leftarrow \mathcal{U}(\mathbb{R}_2^k)$\\
    $y_i\leftarrow x_i\xor r$\\
    $y_1\leftarrow y_1\xor r$\\
}
\algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}

\end{algorithm}


\begin{algorithm}[!ht]
\caption{ Masked Comparison (MaskComp) }
\label{algo:MaskComp}

\Input{$\{\mathbf{b}'_i\}_{1\leq i \leq n}$ where each $\mathbf{b}'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} \mathbf{b}'_i = \mathbf{b}'$,\\
$\{c'_i\}_{1\leq i \leq n}$ where each $c'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} c'_i = c'$,\\
publicly avilable $\mathbf{b}$ and $c$}
\Output{$\{b_i\}_{1\leq i \leq n}$ with each $b_i \in \{0,1\}$ such that $\bigoplus_{i=1}^{n} b_i = 1$ iff\\ $\mathbf{b}''=\mathbf{b}'>>(\epsilon_q-\epsilon_p)=3$ and $c''=c'>>(\epsilon_p-\epsilon_t)=6$, else $0$}
\BlankLine

//\texttt{for $\mathbf{b}$ part of ciphertext}\\
\For{\texttt{j1=} $1$ \texttt{to } $l=3$}
{
    \For{\texttt{j2=} $1$ \texttt{to } $N=256$}
    {
        $\mathbf{eb}[j1][j2]\leftarrow(\mathbf{b}[j1][j2]<<3)+8$\\
        $\mathbf{b}'_{n}[j1][j2]\leftarrow \mathbf{b}'_{n}[j1][j2]-\mathbf{eb}[j1][j2]$\\
         $\{\mathbf{y}_i[j1][j2]\}_{1\leq i \leq n}\leftarrow$ A2B$(\{\mathbf{b}'_i[j1][j2]\}_{1\leq i \leq n})$\\
    
        \For{\texttt{s=} $1$ \texttt{to } $\epsilon_p=10$}
        {
            $\{\mathbf{x}_i[s][j1][j2]\}_{1\leq i \leq n}\leftarrow (\{\mathbf{y}_i[j1][j2]\}_{1\leq i \leq n}>>(s+3-1))$\\
        }
    }
    \For{\texttt{s=} $1$ \texttt{to } $\epsilon_p=10$}
    {
        $\{\mathbf{u}_i[s][j1]\}_{1\leq i \leq n}\leftarrow$ Bitslice$(\{\mathbf{x}_i[s][j1]\}_{1\leq i \leq n})$
    }
}

//\texttt{for $c$ part of ciphertext}\\
\For{\texttt{j2=} $1$ \texttt{to } $N=256$}
{
    $ec[j2]\leftarrow(c[j2]<<6)+64$\\
    $c'_{n}[j2]\leftarrow c'_{n}[j2]-ec[j2]$\\
    $\{y_i[j2]\}_{1\leq i \leq n}\leftarrow$ A2B$(\{c'_i[j2]\}_{1\leq i \leq n})$\\

    \For{\texttt{s=} $1$ \texttt{to } $\epsilon_t=4$}
    {
        $\{z_i[s][j2]\}_{1\leq i \leq n}\leftarrow(\{y_i[j2]\}_{1\leq i \leq n}>>(s+6-1))$\\
    }
}
\For{\texttt{s=} $1$ \texttt{to } $\epsilon_t=4$}
{
    $\{v_i[s]\}_{1\leq i \leq n}\leftarrow$ Bitslice$(\{z_i[s]\}_{1\leq i \leq n})$
}
//Secure And on results of both parts of ciphertexts\\
$\{w_i\}_{1\leq i \leq n}\leftarrow \{v_i[1]\}_{1\leq i \leq n}$\\
\For{\texttt{s=} $2$ \texttt{to } $\epsilon_t=4$}
{
    $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\{v_i[s]\}_{1\leq i \leq n})$\\
}
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow \{\mathbf{u}_i[1][j]\}_{1\leq i \leq n}$\\
    \For{\texttt{s=} $2$ \texttt{to } $\epsilon_p=10$}
    {
        $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{\mathbf{y}_i[j]\}_{1\leq i \leq n},\{\mathbf{u}_i[s][j]\}_{1\leq i \leq n})$\\
    }
}
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\mathbf{y}_i[j]\}_{1\leq i \leq n})$\\
}
\For{\texttt{j=} $\log_2 256-1$ \texttt{to } $0$}
{
    $\{w'_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n}>>2^j $\\
    $\{w_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n} \mod(2^{2^j}-1)$\\
    $\{w_i\}_{1\leq i \leq n}\leftarrow SecAnd(\{w_i\}_{1\leq i \leq n}, \{w'_i\}_{1\leq i \leq n})$\\
}
$\{b_i\}_{1\leq i \leq n}\leftarrow \{w_i\}_{1\leq i \leq n}$\\
\algorithmicreturn{ $\{b_i\}_{1\leq i \leq n}$}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{ Masked Comparison (MaskComp) }
\label{algo:MaskComp}

\Input{$\{\mathbf{b}'_i\}_{1\leq i \leq n}$ where each $\mathbf{b}'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} \mathbf{b}'_i = \mathbf{b}'$,\\
$\{c'_i\}_{1\leq i \leq n}$ where each $c'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} c'_i = c'$,\\
publicly avilable $\mathbf{b}$ and $c$}
\Output{$\{b_i\}_{1\leq i \leq n}$ with each $b_i \in \{0,1\}$ such that $\bigoplus_{i=1}^{n} b_i = 1$ iff\\ $\mathbf{b}''=\mathbf{b}'>>(\epsilon_q-\epsilon_p)=3$ and $c''=c'>>(\epsilon_p-\epsilon_t)=6$, else $0$}
\BlankLine

//\texttt{for $\mathbf{b}$ part of ciphertext}\\
\For{\texttt{j1=} $1$ \texttt{to } $l=3$}
{
    \For{\texttt{j2=} $1$ \texttt{to } $N=256$}
    {
        $\mathbf{eb}[j1][j2]\leftarrow(\mathbf{b}[j1][j2]<<3)+8$\\
        $\mathbf{b}'_{n}[j1][j2]\leftarrow \mathbf{b}'_{n}[j1][j2]-\mathbf{eb}[j1][j2]$\\
         $\{\mathbf{y}_i[j1][j2]\}_{1\leq i \leq n}\leftarrow$ A2B$(\{\mathbf{b}'_i[j1][j2]\}_{1\leq i \leq n})$\\
    
        \For{\texttt{s=} $1$ \texttt{to } $\epsilon_p=10$}
        {
            $\{\mathbf{x}_i[s][j1][j2]\}_{1\leq i \leq n}\leftarrow (\{\mathbf{y}_i[j1][j2]\}_{1\leq i \leq n}>>(s+3-1))$\\
        }
    }
    \For{\texttt{s=} $1$ \texttt{to } $\epsilon_p=10$}
    {
        $\{\mathbf{u}_i[s][j1]\}_{1\leq i \leq n}\leftarrow$ Bitslice$(\{\mathbf{x}_i[s][j1]\}_{1\leq i \leq n})$
    }
}

//\texttt{for $c$ part of ciphertext}\\
\For{\texttt{j2=} $1$ \texttt{to } $N=256$}
{
    $ec[j2]\leftarrow(c[j2]<<6)+64$\\
    $c'_{n}[j2]\leftarrow c'_{n}[j2]-ec[j2]$\\
    $\{y_i[j2]\}_{1\leq i \leq n}\leftarrow$ A2B$(\{c'_i[j2]\}_{1\leq i \leq n})$\\

    \For{\texttt{s=} $1$ \texttt{to } $\epsilon_t=4$}
    {
        $\{z_i[s][j2]\}_{1\leq i \leq n}\leftarrow(\{y_i[j2]\}_{1\leq i \leq n}>>(s+6-1))$\\
    }
}
\For{\texttt{s=} $1$ \texttt{to } $\epsilon_t=4$}
{
    $\{v_i[s]\}_{1\leq i \leq n}\leftarrow$ Bitslice$(\{z_i[s]\}_{1\leq i \leq n})$
}
//Secure And on results of both parts of ciphertexts\\
$\{w_i\}_{1\leq i \leq n}\leftarrow \{v_i[1]\}_{1\leq i \leq n}$\\
\For{\texttt{s=} $2$ \texttt{to } $\epsilon_t=4$}
{
    $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\{v_i[s]\}_{1\leq i \leq n})$\\
}
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow \{\mathbf{u}_i[1][j]\}_{1\leq i \leq n}$\\
    \For{\texttt{s=} $2$ \texttt{to } $\epsilon_p=10$}
    {
        $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{\mathbf{y}_i[j]\}_{1\leq i \leq n},\{\mathbf{u}_i[s][j]\}_{1\leq i \leq n})$\\
    }
}
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\mathbf{y}_i[j]\}_{1\leq i \leq n})$\\
}
\For{\texttt{j=} $\log_2 256-1$ \texttt{to } $0$}
{
    $\{w'_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n}>>2^j $\\
    $\{w_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n} \mod(2^{2^j}-1)$\\
    $\{w_i\}_{1\leq i \leq n}\leftarrow SecAnd(\{w_i\}_{1\leq i \leq n}, \{w'_i\}_{1\leq i \leq n})$\\
}
$\{b_i\}_{1\leq i \leq n}\leftarrow \{w_i\}_{1\leq i \leq n}$\\
\algorithmicreturn{ $\{b_i\}_{1\leq i \leq n}$}
\end{algorithm}

==> images/kyberKEM.tex <==
\begin{figure}[ht]
\fbox{\begin{varwidth}{0.98\textwidth}
\begin{subfigure}[t]{0.47\textwidth}
    \begin{small}
    \raggedright 
    $\mathtt{Kyber}{.}\mathtt{KEM}{.}\mathtt{KeyGen} ()$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $(seed_{\pmb{A}}, \pmb{b}, \pmb{s})  = \mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{KeyGen} ()$ \\
        \item $pk = (seed_{\pmb{A}}, \pmb{b})$ \\
        \item $pkh = \mathcal{H}(pk) $ \\
        \item $z \leftarrow  \mathcal{U}(\{0,1\}^{256}$) \\
        \item \textbf{return} $(pk = (seed_{\pmb{A}}, \pmb{b}), sk =  (\pmb{s},z, pkh))$
    \end{enumerate} 
    \end{small}
    \vspace{3mm}
\end{subfigure}
\begin{subfigure}[t]{0.47\textwidth}
    \begin{small}
    \raggedright
    $\mathtt{Kyber}{.}\mathtt{KEM}{.}\mathtt{Encaps} (pk = (seed_{\pmb{A}}, \pmb{b}))$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $m  \leftarrow  \mathcal{U}(\{0,1\}^{256}) $ \\
        \item $m  = \mathcal{H}(m)$ \\
        \item $(\hat{K}, r) = \mathcal{G}(\mathcal{H}(pk), m)$ \\
        \item $c = \mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{Enc} (pk, m; r )$ \\
        \item $K = \mathtt{KDF}(\hat{K}, \mathcal{H}(c))$
        \item \textbf{return} $(c, K)$
    \end{enumerate} 
    \end{small}
\end{subfigure}
\begin{subfigure}[t]{\textwidth}
    \begin{small}
    \raggedright
    $\mathtt{Kyber}{.}\mathtt{KEM}{.}\mathtt{Decaps} (sk = (\pmb{s}, z, pkh),pk = (seed_{\pmb{A}}, \pmb{b}), c)$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $m'  =  \mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{Dec} (\pmb{s}, c )$ \\
        \item $(\hat{K}', r') = \mathcal{G}(pkh, m')$ \\
        \item $c_* = \mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{Enc} (pk, m'; r')$ \\
        \item \textbf{if: } $c=c_*$
        \item \quad \textbf{return} $ K = \mathtt{KDF}(\hat{K}', \mathcal{H}(c))$
        \item \textbf{else: }
        \item \quad \textbf{return} $ K = \mathtt{KDF}(z, \mathcal{H}(c))$  
    \end{enumerate} 
    \end{small}
\end{subfigure}
\end{varwidth}}
\caption{CCA secure $\mathtt{Kyber}{.}\KEM$~\cite{Kyber-Kem}}
\label{fig:kyberkem}
\end{figure}

==> images/kyberPKE.tex <==
\begin{figure}[ht]
% \begin{adjustbox}
\fbox{\begin{varwidth}{0.98\textwidth}
\begin{subfigure}[t]{0.47\textwidth}
    \raggedright 
    \begin{small}
    $\mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{KeyGen} ()$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
            \item $seed_{\pmb{A}} \leftarrow  \mathcal{U}(\{0,1\}^{256})$ \\
            \item $seed_{\pmb{se}} \leftarrow  \mathcal{U}(\{0,1\}^{256})$ \\
            \item $\pmb{\tilde{A}} = \mathtt{NTT} (\pmb{A}) \leftarrow  \mathcal{U}(R^{l \times l}_q; \seeda) $ \\
            \item $\pmb{s} \leftarrow  \beta_{\eta_1} ( R^{l}_q; seed_{se})$ \\
            \item $\pmb{e} \leftarrow  \beta_{\eta_1} ( R^{l}_q; seed_{se})$ \\
            \item $\pmb{\tilde{s}} = \mathtt{NTT} (\pmb{s}) \in R^{l}_q$ \\
            \item $\pmb{\tilde{e}} = \mathtt{NTT} (\pmb{e}) \in R^{l}_q$ \\
            \item $\pmb{\tilde{b}} =  (\pmb{\tilde{A}} \pmb{\tilde{s}} + \pmb{\tilde{e}}) \in R^{l}_q$ \\
            \item \textbf{return} $(pk = (seed_{\pmb{A}}, \pmb{\tilde{b}}), sk =  (\pmb{\tilde{s}}))$
    \end{enumerate} 
    \end{small}
\end{subfigure}
\begin{subfigure}[t]{0.52\textwidth}
    \raggedright
    \begin{small}
    $\mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{Enc} (pk = (seed_{\pmb{A}}, \pmb{b}), m \in R_2; r )$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $\pmb{\tilde{A}} \leftarrow \mathcal{U}(R^{l \times l}_q; \seeda) $ \\
        \item \textbf{if: } $r$  is not specified:
        \item \quad $ r \leftarrow  \mathcal{U}(\{0,1\}^{256})$\\
        \item $\pmb{s'} \leftarrow  \beta_{\eta_1} ( R^{l}_q ; r)	$\\
        \item $\pmb{e_1} \leftarrow  \beta_{\eta_2} ( R^{l}_q ; r)	$\\
        \item ${e_2} \leftarrow  \beta_{\mu e2} ( R_q ; r)	$\\
        \item $\pmb{\tilde{s'}} = \mathtt{NTT} (\pmb{s'}) \in R^{l}_q$ \\
        \item $\pmb{b'} = ( \mathtt{INTT}(\pmb{\tilde{A}}^T \pmb{\tilde{s'}}) + \pmb{e_1}) \in R^{l}_q$\\
        \item $ c_m = \mathtt{INTT}(\pmb{\tilde{b}}^T \pmb{\tilde{s'}}) + {e_2} + \mathtt{Encode}(m) \in R_q$\\
        \item $\pmb{u} = \mathtt{Compress}(\pmb{b'}, p)  \in R^{l}_p$\\
        \item $v = \mathtt{Compress}(c_m, t) \in R_{t} $\\
        \item \textbf{return} $c =(\pmb{u}, v)$
    \end{enumerate} 
    \end{small}
\end{subfigure}
\begin{subfigure}[t]{\textwidth}
    \raggedright
    \begin{small}
    $\mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{Dec}(sk=\pmb{s},c=(\pmb{u}, v))$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $\pmb{u'} = \mathtt{Decompress}(\pmb{u}, p)  \in R^{l}_q$\\
        \item $v' = \mathtt{Decompress}(v, t) \in R_{q} $\\
        \item $\pmb{\tilde{u'}} = \mathtt{NTT} (\pmb{u'}) \in R^{l}_q$ \\
        \item ${\tilde{u''}} = \pmb{\tilde{u'}} \pmb{\tilde{s'}} \in R_q$ \\
        \item $m'' = v' - \mathtt{INTT}({\tilde{u''}}) \in R_q$ \\
        \item $m' = \mathtt{Decode}(m'') \in R_2$  \\
        \item \textbf{return} $m'$
    \end{enumerate} 
    \end{small}
\end{subfigure}
\end{varwidth}}
\caption{CPA secure $\mathtt{Kyber}{.}\mathtt{PKE}$~\cite{Kyber-Kem}}
\label{fig:kyberpke}
% \end{adjustbox}
\end{figure}

==> images/kybermasked.tex <==
\begin{figure}[!ht]
    \centering
\setlength{\nodedistance}{4mm}
\resizebox{0.75\textwidth}{!}{
\begin{tikzpicture}[ % <--- used style are moved here 
node distance = \nodedistance,
operation/.style = {circle, draw=black},
bigoperation/.style = {rounded corners, draw=black},
operationsecret/.style = {circle, draw=black, fill=black!20!white, text=black, very thick},
bigoperationsecret/.style = {rounded corners, draw=black, fill=black!20!white, text=black, very thick},
Bigoperationsecret/.style = {rounded corners, draw=black, fill=black!20!white, text=black, very thick, minimum height=4\nodedistance, , minimum width=2\nodedistance},
operant/.style = {},
halfblockdraw/.style = {draw, rounded corners},
line/.style = {draw, -Latex},
connect with angle/.style=
{to path={let \p1=(\tikztostart), 
\p2=(\tikztotarget) in -- ++(0, {(\x2-\x1)*tan(#1-90)-(\y1-\y2)}) -- (\tikztotarget)}},
connect with angle hor/.style=
{to path={let \p1=(\tikztostart), 
\p2=(\tikztotarget) in -- ++({(\x2-\x1)-(\y1-\y2)*tan(#1-90)}, 0) -- (\tikztotarget)}},
                       ]
% Place nodes

% bp * s
\node (decom) [bigoperation]  {$\mathtt{Decomp}$};
\node (bp) [operant, left=of decom.west]  {$\pmb{u}$};
\draw[->] (bp) -- (decom);

% bp * s
\node (multbps) [operationsecret, right=of decom]  {X};
\draw[->] (decom) -- (multbps);

% % bp * s
% \node (multbps) [operationsecret]  {X};
% \node (bp) [operant, left=of multbps.west]  {$\pmb{u}$};
% \draw[->] (bp) -- (multbps);

\node (s) [operant, above=of multbps.north]  {$\pmb{s}_1$};
\draw[->, very thick] (s) -- (multbps);

%% 2
% \node (multbps2) [operationsecret, below=of multbps]  {X};
% \draw[->] (bp) -- (bp |- multbps2) -- (multbps2);

\node (multbps2) [operationsecret, below=of multbps]  {X};
\draw[->] (decom) -- (decom |- multbps2) -- (multbps2);

\node (s) [operant, below=of multbps2]  {$\pmb{s}_2$};
\draw[->, very thick] (s) -- (multbps2);

\coordinate  (addvh) at ($(multbps.east)$);

% % v + h addition
% \node (addvh) [operationsecret, right=of multbps]  {$+$};
% \draw[->, very thick] (multbps.east) -- (addvh.west);
% \node (h2) [operant, above=of addvh.north]  {$\pmb{h}_2$};
% \draw[->] (h2) -- (addvh);

% cm
\node (cm) [operant, below=6\nodedistance of bp]  {$v$};
\node (shiftcm) [bigoperation, right=of cm]  {$\mathtt{Decomp}$};
\draw[->] (cm) -- (shiftcm);

% cm - v
\coordinate [right= of addvh](addvhright);
\node (subcmv) [operationsecret, right=of multbps2] {$-$};
\draw[->, very thick] (multbps2) -- (subcmv);
\draw[->] (shiftcm) -- (subcmv |- shiftcm) -- (subcmv);

% tobin
\node (tobin) [Bigoperationsecret, right=2\nodedistance of $(subcmv.east)!0.5!(addvh.east)$]  {$\mathtt{Decode}$};
\draw[->, very thick] (addvh) -- (tobin.west |- addvh);
\draw[->, very thick] (subcmv) -- (tobin.west |- subcmv);

\node[draw=red, -, very thick, fit=(tobin)] {};

% G(pk, m)
\node (g) [Bigoperationsecret, right= 2\nodedistance of tobin]  {$\mathcal{G}$};
\node (pkh) [operant, above=of g]  {$pkh$};
\coordinate  (m1) at ($(tobin.east |- addvh)!0.6!(g.west |- addvh)$);
\coordinate  (m2) at ($(tobin.east |- subcmv)!0.3!(g.west |- subcmv)$);
\draw[->, transform canvas={xshift=0.5em}] (pkh) -- (g);
\draw[->, transform canvas={xshift=-0.5em}] (pkh) -- (g);
\draw[->, very thick] (tobin.east |- addvh) -- (g.west |- addvh);
\draw[->, very thick] (tobin.east |- subcmv) -- (g.west |- subcmv);

\node (K) [operant, below=of g]  {$\hat{K}'$};
\draw[->, very thick, transform canvas={xshift=0.5em}] (g) -- (K);
\draw[->, very thick, transform canvas={xshift=-0.5em}] (g) -- (K);

% extra shit in betamu
\node (xof) [Bigoperationsecret, right= 2\nodedistance of g]  {$XOF$};
\draw[->, very thick] (g.east |- addvh) -- (xof.west |- addvh);
\draw[->, very thick] (g.east |- subcmv) -- (xof.west |- subcmv);

% extra shit in betamu
\node (xofe1) [Bigoperationsecret, above=of xof]  {$XOF$};
\coordinate  (xofe1m1) at ($(g.east |- addvh)!0.3!(xof.west |- addvh)$);
\coordinate [above= 5\nodedistance of xofe1m1 ](xofe1m1mid);
\coordinate  (xofe1m2) at ($(g.east |- subcmv)!0.7!(xof.west |- subcmv)$);
\coordinate [above= 5\nodedistance of xofe1m2 ](xofe1m2mid);
\draw[->, very thick] (xofe1m1) -- (xofe1m1mid) -- (xofe1.west |- xofe1m1mid);
\draw[->, very thick] (xofe1m2) -- (xofe1m2mid) -- (xofe1.west |- xofe1m2mid);

% extra shit in betamu
\node (xofe2) [Bigoperationsecret, below=of xof]  {$XOF$};
\coordinate  (xofe2m1) at ($(g.east |- addvh)!0.15!(xof.west |- addvh)$);
\coordinate [below= 7.5\nodedistance of xofe2m1 ](xofe2m1mid);
\coordinate  (xofe2m2) at ($(g.east |- subcmv)!0.55!(xof.west |- subcmv)$);
\coordinate [below= 2.5\nodedistance of xofe2m2 ](xofe2m2mid);
\draw[->, very thick] (xofe2m1) -- (xofe2m1mid) -- (xofe2.west |- xofe2m1mid);
\draw[->, very thick] (xofe2m2) -- (xofe2m2mid) -- (xofe2.west |- xofe2m2mid);

% gen secret
\node (beta) [Bigoperationsecret, right=of xof]  {$\beta_{\mu}$};
\draw[->, very thick] (xof.east |- addvh) -- (beta.west |- addvh);
\draw[->, very thick] (xof.east |- subcmv) -- (beta.west |- subcmv);

% gen secret
\node (beta1) [Bigoperationsecret, right=of xofe1]  {$\beta_{\mu}$};
\draw[->, very thick] (xofe1.east |- xofe1m1mid) -- (beta1.west |- xofe1m1mid);
\draw[->, very thick] (xofe1.east |- xofe1m2mid) -- (beta1.west |- xofe1m2mid);

% gen secret
\node (beta2) [Bigoperationsecret, right=of xofe2]  {$\beta_{\mu}$};
\draw[->, very thick] (xofe2.east |- xofe2m1mid) -- (beta2.west |- xofe2m1mid);
\draw[->, very thick] (xofe2.east |- xofe2m2mid) -- (beta2.west |- xofe2m2mid);


%-------------------------------------
% a * sp
\coordinate (betaout1) at (beta.east |- addvh);
\coordinate (betaout2) at (beta.east |- subcmv);

\node (multasp) [operationsecret, right= 2\nodedistance of betaout1]  {X};
\node (multasp2) [operationsecret, above=5\nodedistance of multasp]  {X};

% \node (gena) [bigoperation, above left=2\nodedistance and \nodedistance of multasp2]  {$\mathcal{U}$};
% \draw[->] (gena) edge[connect with angle=135] (multasp2);
% \draw[->] (gena) edge[connect with angle=135] (multasp);

\node (gena) [bigoperation, above left=2\nodedistance and \nodedistance of multasp2]  {$\mathcal{U}$};
\draw[->] (gena) edge[connect with angle=135] (multasp2);
\draw[->] (gena) edge[connect with angle=135] (multasp);

% \node (seeda) [operant, above=of gena]  {$\seeda$};
% \draw[->] (seeda) -- (gena);
\node (seeda) [operant, left=of gena]  {$\seeda$};
\draw[->] (seeda) -- (gena);

% b * sp
\node (multbsp) [operationsecret, below=of multasp]  {X};
\node (multbsp2) [operationsecret, below=5\nodedistance of multbsp]  {X};

\node (b) [operant,  below left=2\nodedistance and 0.8\nodedistance of multbsp2]  {$\pmb{b}$};
\draw[->] (b) edge[connect with angle=45] (multbsp);
\draw[->] (b) edge[connect with angle=45] (multbsp2);

% connection shit between beta and mults
\coordinate  (r1) at ($(betaout1)!0.2!(multasp)$);
\coordinate  (r2) at ($(betaout2)!0.6!(multasp)$);

\draw[->, very thick]  (betaout1) -- (multbsp); 
\draw[->, very thick]  (betaout1) -- (multasp2); 

\draw[->, very thick]  (betaout2) -- (multbsp2); 
\draw[->, very thick]  (betaout2) -- (multasp); 

% add h1
\node (addh1) [operationsecret, right= 5\nodedistance of $(beta1.east |- xofe1m1mid)$]  {$+$};
\draw[->, very thick] (beta1.east |- xofe1m1mid) -- (addh1.west);
\draw[->, very thick] (multasp2) -- (addh1);

% add h3
\node (addh3) [operationsecret, right= 5\nodedistance of $(beta1.east |- xofe1m2mid)$]  {$+$};
\draw[->, very thick] (beta1.east |- xofe1m2mid) -- (addh3.west);
\draw[->, very thick] (multasp) -- (addh3);

% add h4
\node (addh4) [operationsecret, right= 5\nodedistance of $(beta2.east |- xofe2m1mid)$]  {$+$};
\draw[->, very thick] (beta2.east |- xofe2m1mid) -- (addh4.west);
\draw[->, very thick] (multbsp2) -- (addh4);

% add h5
\node (addh5) [operationsecret, right= 5\nodedistance of $(beta2.east |- xofe2m2mid)$]  {$+$};
\draw[->, very thick] (beta2.east |- xofe2m2mid) -- (addh5.west);
\draw[->, very thick] (multbsp) -- (addh5);

%b2a
\node (b2a) [Bigoperationsecret, below= 3\nodedistance of xofe2]  {$\mathtt{Encode}$};


%add m
\node (addm) [operationsecret, right=of addh4]  {$+$};
\node (addm1) [operationsecret, right=of addh5]  {$+$};
\coordinate [below=6.5\nodedistance of xofe2](tmp2);
\coordinate [below=4.5\nodedistance of xofe2](tmp1); 
\draw[->, very thick] (m2) -- (m2 |- tmp2) -- (b2a.west |- tmp2);
\draw[->, very thick] (b2a.east |- tmp2) -- (addm |- tmp2) -- (addm);
\coordinate (iammakingthiscodeugly) at ($(addm)!0.5!(addh4)$);
\draw[->, very thick] (m1) -- (m1 |- tmp1)  -- (b2a.west |- tmp1); 
\draw[very thick] (b2a.east |- tmp1) -- (iammakingthiscodeugly |- tmp1) edge[->,connect with angle=45] (addm1);

\draw[->, very thick] (addh5) -- (addm1);
\draw[->, very thick] (addh4) -- (addm);

% divide
\coordinate[right= 2\nodedistance of addm] (dividex);
\coordinate (dividey1) at ($(addh1)!0.5!(addh3)$);
\coordinate (dividey2) at ($(addm)!0.5!(addm1)$);
\node (divide2) [Bigoperationsecret] at (dividex |- dividey1)  {$\mathtt{Comp}$};
\node (divide1) [Bigoperationsecret] at (dividex |- dividey2)  {$\mathtt{Comp}$};
\draw[->, very thick] (addm) -- (divide1.west |- addm);
\draw[->, very thick] (addh1) -- (divide2.west |- addh1);
\draw[->, very thick] (addm1) -- (divide1.west |- addm1);
\draw[->, very thick] (addh3) -- (divide2.west |- addh3);

% b*, v*
\coordinate[right= 2\nodedistance of divide1] (output);
\node (bp2) [operant] at (output |- addh1)  {$\pmb{u}_{*1}$};
\node (bp22) [operant] at (output |- addh3)  {$\pmb{u}_{*2}$};
\node (cm22) [operant] at (output |- addm1)  {${v}_{*1}$};
\node (cm2) [operant] at (output |- addm)  {${v}_{*2}$};
\draw[->, very thick] (divide1.east |- bp2) -- (bp2);
\draw[->, very thick] (divide1.east |- bp22) -- (bp22);
\draw[->, very thick] (divide2.east |- cm22) -- (cm22);
\draw[->, very thick] (divide2.east |- cm2) -- (cm2);

% compare
\node[draw=black, dotted, thick, fit=(bp2) (cm2)](ciphertext2) {};
\node[draw=black, dotted, thick, fit=(bp) (cm)](ciphertext) {};
\coordinate [below=1.5\nodedistance of b2a](x); 
\coordinate (y) at ($(ciphertext)!0.5!(ciphertext2)$);
\node (comp) [operationsecret, very thick] at (y |- x)  {$=?$};

\draw[->] (ciphertext) -- (ciphertext |- x) -- (comp);
\draw[->, very thick] (ciphertext2) -- (ciphertext2 |- x) -- (comp);

% two end results
\node (correct) [bigoperation, below left=2\nodedistance and 2\nodedistance of comp]  {return $\mathcal{H}(\hat{K}', c)$};
\draw[->] (comp.south) -- (correct);
\node[operant,  below left=0.5\nodedistance and 1.3\nodedistance of comp] (yes) {yes};

\node (correct) [bigoperation, below right=2\nodedistance and 2\nodedistance of comp]  {return $\mathcal{H}(z, c)$};
\draw[->] (comp.south) -- (correct);
\node[operant,  below right=0.5\nodedistance and 1.3\nodedistance of comp] (no) {no};
\end{tikzpicture}}

\caption{First-order masked $\mathtt{Kyber}.\mathtt{KEM}.\mathtt{Decaps}$ algorithm. The highlighted operations in color gray are influenced by the non-ephemeral secret-key $\pmb{s}$ and use masking to prevent SCA. The component we concentrate on in this work is enveloped with the red rectangle.}%~\cite{Fritzmann_2021}.}

\label{fig:kybermaskeddecaps}
\end{figure}

==> images/saberKEM.tex <==
\begin{figure}[ht]
\fbox{\begin{varwidth}{0.98\textwidth}
\begin{subfigure}[t]{0.47\textwidth}
    \begin{small}
    \raggedright 
    $\mathtt{Saber}/\mathtt{Kyber}{.}\mathtt{KEM}{.}\mathtt{KeyGen} ()$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $(seed_{\pmb{A}}, \pmb{b}, \pmb{s})  = \mathtt{Saber}/\mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{KeyGen} ()$ \\
        \item $pk = (seed_{\pmb{A}}, \pmb{b})$ \\
        \item $pkh = \mathcal{H}(pk) $ \\
        \item $z \leftarrow \mathcal{U}(\{0,1\}^{256}$) \\
        \item \textbf{return} $(pk = (seed_{\pmb{A}}, \pmb{b}), sk =  (\pmb{s},z, pkh))$
    \end{enumerate} 
    \end{small}
    \vspace{3mm}
\end{subfigure}
\begin{subfigure}[t]{0.47\textwidth}
    \begin{small}
    \raggedright
    $\mathtt{Saber}/\mathtt{Kyber}{.}\mathtt{KEM}{.}\mathtt{Encaps} (pk = (seed_{\pmb{A}}, \pmb{b}))$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $m  \leftarrow  \mathcal{U}(\{0,1\}^{256}) $ \\
        \item $m  = \mathcal{H}(m)$ \\
        \item $(\hat{K}, r) = \mathcal{G}(\mathcal{H}(pk), m)$ \\
        \item $c = \mathtt{Saber}/\mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{Enc} (pk, m; r )$ \\
        \item $K = \mathtt{KDF}(\hat{K}, \mathcal{H}(c))$
        \item \textbf{return} $(c, K)$
    \end{enumerate} 
    \end{small}
\end{subfigure}
\begin{subfigure}[t]{\textwidth}
    \begin{small}
    \raggedright
    $\mathtt{Saber}/\mathtt{Kyber}{.}\mathtt{KEM}{.}\mathtt{Decaps} (sk = (\pmb{s}, z, pkh),pk = (seed_{\pmb{A}}, \pmb{b}), c)$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $m'  =  \mathtt{Saber}/\mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{Dec} (\pmb{s}, c )$ \\
        \item $(\hat{K}', r') = \mathcal{G}(pkh, m')$ \\
        \item $c_* = \mathtt{Saber}/\mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{Enc} (pk, m'; r')$ \\
        \item \textbf{if: } $c=c_*$
        \item \quad \textbf{return} $ K = \mathtt{KDF}(\hat{K}', \mathcal{H}(c))$
        \item \textbf{else: }
        \item \quad \textbf{return} $ K = \mathtt{KDF}(z, \mathcal{H}(c))$  
    \end{enumerate} 
    \end{small}
\end{subfigure}
\end{varwidth}}
\caption{CCA secure $\mathtt{Saber}/\mathtt{Kyber}{.}\KEM$~\cite{Saber_kem,Kyber-Kem}}
\label{fig:saberkem}
\end{figure}

==> images/saberPKE.tex <==
\begin{figure}[ht]
% \begin{adjustbox}
\fbox{\begin{varwidth}{\textwidth}
\begin{subfigure}[t]{0.46\textwidth}
    \raggedright 
    \begin{small}
    $\mathtt{Saber}{.}\mathtt{PKE}{.}\mathtt{KeyGen} ()$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
            \item $seed_{\pmb{A}} \leftarrow  \mathcal{U}(\{0,1\}^{256})$ \\
            \item $\pmb{A} \leftarrow \mathcal{U}(R^{l \times l}_q; \seeda) $ \\
            \item $r \leftarrow \mathcal{U}(\{0,1\}^{256})$ \\
            \item $\pmb{s} \leftarrow \beta_\mu ( R^{l}_q; r)$ \\
            \item $\pmb{b} =  ((\pmb{A}^T \pmb{s} + \pmb{h}) \bmod{q}) \gg (\epsilon_q - \epsilon_p) \in R^{l}_p$ \\
            \item \textbf{return} $(pk = (seed_{\pmb{A}}, \pmb{b}), sk =  (\pmb{s}))$
    \end{enumerate} 
    \end{small}
\end{subfigure}
\begin{subfigure}[t]{0.52\textwidth}
    \raggedright
    \begin{small}
    $\mathtt{Saber}{.}\mathtt{PKE}{.}\mathtt{Enc} (pk = (seed_{\pmb{A}}, \pmb{b}), m \in R_2; r )$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $\pmb{A} \leftarrow \mathcal{U}(R^{l \times l}_q; \seeda) $ \\
        \item \textbf{if: } $r$  is not specified:
        \item \quad $ r \leftarrow \mathcal{U}(\{0,1\}^{256})$
        \item $\pmb{s'} \leftarrow \beta_\mu ( R^{l}_q ; r)	$
        \item $\pmb{u} = ( ( \pmb{A}  \pmb{s}' + \pmb{h}) \bmod{q})  \gg (\epsilon_q - \epsilon_p)  \in R^{l}_p$
        \item $ c_m = \pmb{b}^T  (\pmb{s}' \bmod{p})  \in R_p$
        \item $v = (c_m  + h_1 - 2^{\epsilon_p-1} m \bmod{p}) \gg (\epsilon_p - \epsilon_t) \in R_{t} $
        \item \textbf{return} $c =(\pmb{u}, v)$
    \end{enumerate} 
    \end{small}
\end{subfigure}
\begin{subfigure}[t]{\textwidth}
    \raggedright
    \begin{small}
    $\mathtt{Saber}{.}\mathtt{PKE}{.}\mathtt{Dec}(sk=\pmb{s},c=(\pmb{u}, v))$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $u'' = \pmb{u}^{T} (\pmb{s} \bmod{p}) \in R_p $\\
        \item $m'' = (u''-2^{\epsilon_p-\epsilon_t}v + h_2) \bmod{p}$
        \item $m' = m'' \gg (\epsilon_p-1) \in R_2$  \\
        \item \textbf{return} $m'$
    \end{enumerate} 
    \end{small}
\end{subfigure}
\end{varwidth}}
\caption{CPA secure $\mathtt{Saber}{.}\mathtt{PKE}$~\cite{Saber_kem}}
\label{fig:saberpke}
% \end{adjustbox}
\end{figure}

==> images/saberunmasked.tex <==
\begin{figure}
     \centering
\setlength{\nodedistance}{4mm}
\resizebox{0.90\textwidth}{!}{%
\begin{tikzpicture}[ % <--- used style are moved here 
node distance = \nodedistance,
operation/.style = {circle, draw=black},
bigoperation/.style = {rounded corners, draw=black},
operationsecret/.style = {circle, draw=black, fill=black!20!white, text=black, very thick},
bigoperationsecret/.style = {rounded corners, draw=black, fill=black!20!white, text=black, very thick},
operant/.style = {},
halfblockdraw/.style = {draw, rounded corners},
     line/.style = {draw, -Latex}
                       ]
% Place nodes
% bp * s
\node (multbps) [operationsecret]  {X};
\node (bp) [operant, left=of multbps.west]  {$\pmb{b}'$};
\draw[->] (bp) -- (multbps);

\node (s) [operant, above=of multbps.north]  {$\pmb{s}$};
\draw[->, very thick] (s) -- (multbps);

% v + h addition
\node (addvh) [operationsecret, right=of multbps]  {$+$};
\draw[->, very thick] (multbps.east) -- (addvh.west);
\node (h2) [operant, above=of addvh.north]  {$\pmb{h}_2$};
\draw[->] (h2) -- (addvh);

% cm
\node (cm) [operant, below=of bp]  {${c}_m$};
\node (shiftcm) [bigoperation, right=of cm]  {$\ll$};
\draw[->] (cm) -- (shiftcm);

% cm - v
\coordinate [right=of addvh](addvhright);
\node (subcmv) [operationsecret, very thick] at (addvhright |- shiftcm) {$-$};
\draw[->, very thick] (addvh) -- (addvhright) -- (subcmv);
\draw[->] (shiftcm) -- (subcmv);

% tobin
\node (tobin) [bigoperationsecret, right=of subcmv]  {$\gg$};
\draw[->, very thick] (subcmv) -- (tobin);

% G(pk, m)
\node (g) [bigoperationsecret, right=of tobin]  {$\mathcal{G}$};
\coordinate  (m) at ($(tobin.east)!0.5!(g.west)$);
\node (pkh) [operant, above=of g]  {$pkh$};
\draw[->] (pkh) -- (g);
\draw[->, very thick] (tobin) -- (g);

\node (K) [operant, below=of g]  {$\hat{K}'$};
\draw[->, very thick] (g) -- (K);

% gen secret
\node (beta1) [bigoperationsecret, right=of g]  {XOF};
\draw[->, very thick] (g) -- (beta1);

\node (beta2) [bigoperationsecret, right=of beta1]  {$\beta_\mu$};
\draw[->, very thick] (beta1) -- (beta2);

% a * sp
\node (multasp) [operationsecret, right=of beta2]  {X};
\draw[->, very thick] (beta2) -- (multasp);

\node (gena) [bigoperation, above=of multasp]  {$\mathcal{U}$};
\draw[->] (gena) -- (multasp);

\node (seeda) [operant, above=of gena]  {$\seeda$};
\draw[->] (seeda) -- (gena);

% b * sp
\node (multbsp) [operationsecret, below=of multasp]  {X};
\coordinate  (r) at ($(beta2.east)!0.4!(multasp.west)$);
\draw[->, very thick]  (r) -- (r |- multbsp) -- (multbsp); 

\node (b) [operant, below=of multbsp]  {$\pmb{b}$};
\draw[->] (b) -- (multbsp);

% add h1
\node (addh1) [operationsecret, right=of multasp]  {$+$};
\draw[->, very thick] (multasp) -- (addh1);
\node (h1) [operant, above=of addh1]  {$\pmb{h}$};
\draw[->] (h1) -- (addh1);

% add h
\node (addh2) [operationsecret, right=of multbsp]  {$+$};
\draw[->, very thick] (multbsp) -- (addh2);
\node (h) [operant, below=of addh2]  {$h_1$};
\draw[->] (h) -- (addh2);

% add m
\node (addm) [operationsecret, right=of addh2]  {$+$};
\coordinate [below=0.5\nodedistance of h](tmp); 
\draw[->, very thick] (addh2) -- (addm);
\draw[->, very thick] (m) -- (m |- tmp) -- (addm |- tmp) -- (addm);

% divide
\node (divide2) [bigoperationsecret, right=of addm]  {$\gg$};
\node (divide1) [bigoperationsecret] at (divide2 |- addh1)  {$\gg$};
\draw[->, very thick] (addm) -- (divide2);
\draw[->, very thick] (addh1) -- (divide1);

% b*, v*
\node (bp2) [operant, right=of divide1]  {$\pmb{b}'_*$};
\node (cm2) [operant, right=of divide2]  {${c}_{m*}$};
\draw[->, very thick] (divide1) -- (bp2);
\draw[->, very thick] (divide2) -- (cm2);

% compare
\node[draw=black, dotted, thick, fit=(bp2) (cm2)](ciphertext2) {};
\node[draw=black, dotted, thick, fit=(bp) (cm)](ciphertext) {};
\coordinate [below=1.5\nodedistance of tmp](x); 
\coordinate (y) at ($(ciphertext)!0.5!(ciphertext2)$);
\node (comp) [operationsecret, very thick] at (y |- x)  {$=?$};

\draw[->] (ciphertext) -- (ciphertext |- x) -- (comp);
\draw[->, very thick] (ciphertext2) -- (ciphertext2 |- x) -- (comp);

% two end results
\node (correct) [bigoperation, below left=2\nodedistance and 2\nodedistance of comp]  {return $\mathcal{H}(\hat{K}', c)$};
\draw[->] (comp.south) -- (correct);
\node[operant,  below left=0.5\nodedistance and 1.3\nodedistance of comp] (yes) {yes};

\node (correct) [bigoperation, below right=2\nodedistance and 2\nodedistance of comp]  {return $\mathcal{H}(z, c)$};
\draw[->] (comp.south) -- (correct);
\node[operant,  below right=0.5\nodedistance and 1.3\nodedistance of comp] (no) {no};
\end{tikzpicture}}

\caption{Pictorial version of $\mathtt{Saber}.\mathtt{KEM}.\mathtt{Decaps}$ algorithm. The highlighted operations in color gray are influenced by the non-ephemeral secret-key $\pmb{s}$. So, these operations can be exploited during side-channel attacks \cite{FO-masked-saber}.}
\label{fig:saberdecaps}
\end{figure}

==> images/usaberunmasked.tex <==
\begin{figure}
     \centering
\setlength{\nodedistance}{4mm}
\resizebox{0.7\textwidth}{!}{%
\begin{tikzpicture}[ % <--- used style are moved here 
node distance = \nodedistance,
operation/.style = {circle, draw=black},
bigoperation/.style = {rounded corners, draw=black},
operationsecret/.style = {circle, draw=black, fill=black!20!white, text=black, very thick},
bigoperationsecret/.style = {rounded corners, draw=black, fill=black!20!white, text=black, very thick},
operant/.style = {},
halfblockdraw/.style = {draw, rounded corners},
     line/.style = {draw, -Latex}
                       ]
% Place nodes
% bp * s
\node (multbps) [operationsecret]  {X};
\node (bp) [operant, left=of multbps.west]  {$\pmb{b}'$};
\draw[->] (bp) -- (multbps);

\node (s) [operant, above=of multbps.north]  {$\pmb{s}$};
\draw[->, very thick] (s) -- (multbps);

% v + h addition
\node (addvh) [operationsecret, right=of multbps]  {$+$};
\draw[->, very thick] (multbps.east) -- (addvh.west);
\node (h2) [operant, above=of addvh.north]  {$\pmb{h}_2$};
\draw[->] (h2) -- (addvh);

% cm
\node (cm) [operant, below=of bp]  {${c}_m$};
\node (shiftcm) [bigoperation, right=of cm]  {$\ll$};
\draw[->] (cm) -- (shiftcm);

% cm - v
\coordinate [right=of addvh](addvhright);
\node (subcmv) [operationsecret, very thick] at (addvhright |- shiftcm) {$-$};
\draw[->, very thick] (addvh) -- (addvhright) -- (subcmv);
\draw[->] (shiftcm) -- (subcmv);

% tobin
\node (tobin) [bigoperationsecret, right=of subcmv]  {$\gg$};
\draw[->, very thick] (subcmv) -- (tobin);

% G(pk, m)
\node (g) [bigoperationsecret, right=of tobin]  {$\mathcal{G}$};
\coordinate  (m) at ($(tobin.east)!0.5!(g.west)$);
\node (pkh) [operant, above=of g]  {$pkh$};
\draw[->] (pkh) -- (g);
\draw[->, very thick] (tobin) -- (g);

\node (K) [operant, below=of g]  {$\hat{K}'$};
\draw[->, very thick] (g) -- (K);

% gen secret
\node (beta1) [bigoperationsecret, right=of g]  {XOF};
\draw[->, very thick] (g) -- (beta1);

\node (beta2) [bigoperationsecret, right=of beta1]  {$\mathcal{U}_u$};
\draw[->, very thick] (beta1) -- (beta2);

\node[ellipse, draw=blue, thick, fit= (beta2)] {}; %(ciphertext2) {};

% a * sp
\node (multasp) [operationsecret, right=of beta2]  {X};
\draw[->, very thick] (beta2) -- (multasp);

\node (gena) [bigoperation, above=of multasp]  {$\mathcal{U}$};
\draw[->] (gena) -- (multasp);

\node (seeda) [operant, above=of gena]  {$\seeda$};
\draw[->] (seeda) -- (gena);

% b * sp
\node (multbsp) [operationsecret, below=of multasp]  {X};
\coordinate  (r) at ($(beta2.east)!0.4!(multasp.west)$);
\draw[->, very thick]  (r) -- (r |- multbsp) -- (multbsp); 

\node (b) [operant, below=of multbsp]  {$\pmb{b}$};
\draw[->] (b) -- (multbsp);

% add h1
\node (addh1) [operationsecret, right=of multasp]  {$+$};
\draw[->, very thick] (multasp) -- (addh1);
\node (h1) [operant, above=of addh1]  {$\pmb{h}$};
\draw[->] (h1) -- (addh1);

% add h
\node (addh2) [operationsecret, right=of multbsp]  {$+$};
\draw[->, very thick] (multbsp) -- (addh2);
\node (h) [operant, below=of addh2]  {$h_1$};
\draw[->] (h) -- (addh2);

% add m
\node (addm) [operationsecret, right=of addh2]  {$+$};
\coordinate [below=0.5\nodedistance of h](tmp); 
\draw[->, very thick] (addh2) -- (addm);
\draw[->, very thick] (m) -- (m |- tmp) -- (addm |- tmp) -- (addm);

% divide
\node (divide2) [bigoperationsecret, right=of addm]  {$\gg$};
\node (divide1) [bigoperationsecret] at (divide2 |- addh1)  {$\gg$};
\draw[->, very thick] (addm) -- (divide2);
\draw[->, very thick] (addh1) -- (divide1);

% b*, v*
\node (bp2) [operant, right=of divide1]  {$\pmb{b}'_*$};
\node (cm2) [operant, right=of divide2]  {${c}_{m*}$};
\draw[->, very thick] (divide1) -- (bp2);
\draw[->, very thick] (divide2) -- (cm2);

% compare
\node[draw=black, dotted, thick, fit=(bp2) (cm2)](ciphertext2) {};
\node[draw=black, dotted, thick, fit=(bp) (cm)](ciphertext) {};
\coordinate [below=1.5\nodedistance of tmp](x); 
\coordinate (y) at ($(ciphertext)!0.5!(ciphertext2)$);
\node (comp) [operationsecret, very thick] at (y |- x)  {$=$};

\draw[->] (ciphertext) -- (ciphertext |- x) -- (comp);
\draw[->, very thick] (ciphertext2) -- (ciphertext2 |- x) -- (comp);

% two end results
\node (correct) [bigoperation, below left=2\nodedistance and 2\nodedistance of comp]  {return $\mathcal{H}(\hat{K}', c)$};
\draw[->] (comp.south) -- (correct);
\node[operant,  below left=0.5\nodedistance and 1.3\nodedistance of comp] (yes) {yes};

\node (correct) [bigoperation, below right=2\nodedistance and 2\nodedistance of comp]  {return $\mathcal{H}(z, c)$};
\draw[->] (comp.south) -- (correct);
\node[operant,  below right=0.5\nodedistance and 1.3\nodedistance of comp] (no) {no};
\end{tikzpicture}}

\caption{Decapsulation of uSaber. In grey the operations that are influenced by the long term secret $\pmb{s}$ and thus vulnerable to side-channel attacks. The different component of uSaber from Saber is in the blue circle.}
\label{fig:usaberdecaps}
\end{figure}

==> note.tex <==
Jan-Pieter D'Anvers, Angshuman Karmakar Sujoy Sinha Roy, and Frederik Vercauteren. Saber: Module-LWR based key exchange, CPA-secure encryption and CCA-secure KEM. Africacrypt, 2018. (for Saber scheme)
Michiel Van Beirendonck, Jan-Pieter D'Anvers, Aangshuman Karmakar, Josep Balasch, and Ingrid Verbauwhede, "A Side-Channel Resistant Implementation of SABER," ACM Journal on Emerging Technologies in Computing Systems. (first order secure Saber)
Luk Bettale, Jean-Sébastien Coron, and Rina Zeitoun. Improved High-Order Conversion From Boolean to Arithmetic Masking. TCHES, 2018. (for B2A conversion)
Jean-Sébastien Coron, Johann Großschädl, and Praveen Kumar Vadnala. Secure Conversion between Boolean and Arithmetic Masking of Any Order. In CHES. Springer, 2014. (for A2B conversion)
Tobias Schneider, Clara Paglialonga, Tobias Oder, and Tim Güneysu. Efficiently Masking Binomial Sampling at Arbitrary Orders for Lattice-Based Crypto. Public Key Cryptography, 2019. (for CBD $\beta_μ$) 
Hannes Gross, David Schaffenrath, Stefan Mangard. Higher-Order Side-Channel Protected Implementations of KECCAK. DSD, 2017. (for G, XOF)
Joppe W. Bos, Marc Gourjon, Joost Renes, Tobias Schneider, and Christine van Vredendaal. Masking Kyber: First- and Higher-Order Implementations. IACR Cryptol. ePrint Arch., 2021. (for higher order comparison)


==> old_sections/attack_saber.tex <==
\clearpage
\section{Fault attack on Saber}

In the Encapsulation algorithm: Public ciphertext $(a, b)$, where $b = (a.s + e)$
For simplicity, we take the public matrix of polynomials $a$ and the public key vector of polynomials $b$ as a polynomial.
\begin{center}
    $b' = a.s' + e'$, and $c_m = (b.s' + e'' + m*2^9)$.
\end{center}
In the Decryption module of Decapsulation algorithm: Public ciphertext $(b', c_m)$.
For simplicity, we take the secret vector of polynomials $s = ( s_1, s_2, s_3 )$ as a polynomial.
\\
Now,
\begin{center}
\begin{tabular}{ll}
$v$ &$= (c_m * 2^6) + h_2 - b'.s$, where $h_2$ is a constant polynomial\\
  &$= (b.s' + e'' + m*2^9) - (a.s' + e').s $\\
  &$= (a.s + e).s' + e'' + m*2^9 - (a.s' + e').s $\\ 
  &$= e.s' + e'' + m*2^9 - e'.s $\\ 
  &$= e.s' - e'.s + e'' + m*2^9 $\\
  &$= d + m*2^9$\\
\end{tabular}
\end{center}

Let, $v[i]$ and $m[i]$ are coefficients of $v$ and $m$ for $0 \leq i \leq 256$, respectively. Then $10$-th bit of $v[i] = m[i]$ i.e. $m[i] = v[i] \gg 9$.

Now, most probable values of $v[i]$ in $[148, 360]$ if $m[i] = 0$ and most probable values of $v[i]$ in $[660, 872]$ if $m[i] = 1$. 

In first-order mask settings, each $v[i]$ is divided into two shares, $v[i] = v_1[i] + v_2[i] $ $\mod$ ${1024}$, where $v_1[i]$ is randomly chosen from $\mathbb{Z}_{1024}$ and $v_2[i] = v[i] - v_1[i]$ $\mod$ ${1024}$. So, for each $v[i]$ there are $1024$ possible ways to create two shares.  

\subsection{\texttt{Stuck-at-0} fault at one share of the $9$-th bit of $v[i]$}

Approximately half of the most possible values of $v[i]$ in $[148, 360]$ cause decryption failure when $m[i] = 0$. Also, approximately half of the possible values of $v[i]$ in $[660, 872]$ cause decryption failure when $m[i] = 1$. The values of $v[i]$ cause decryption failure are shown inside the red rectangle in the Figure \ref{fig:stuck-at-0}.

\begin{figure}[htp]
    \centering
    \includegraphics[width=12cm]{images/stuck_0.png}
    \caption{Stuck-at-0 fault}
    \label{fig:stuck-at-0}
\end{figure}

Now, as we mentioned earlier each $v[i]$ can be divided into two shares in $1024$ possible ways. However, the decryption failure only occurs in $512$ combinations out of $1024$ possible ways. So, only decryption failure can give us a correct inequality.  


\subsubsection*{Verification:}

We denote $j$-th bit of a variable $x \in \mathbb{Z}_{1024}$ by $x^i$. Here $\xor$ represents bit-wise xor operation and $\&$ represents bit-wise and operation. For simplicity, we rename $v_1[i]$ as $x$ and $v_2[i]$ as $y$. So now, $v[i] = x + y$ $\mod$ ${1024}$.\\
\begin{center}
    $m[i] = v[i]^{10} = x^{10} \xor y^{10} \xor c^9$, where $c^9$ is the carry for $10$-th bit.\\
    $c^9 = (x^9 \& y^9) \xor ((x^9 \xor y^9) \& c^8) = ((y^9 \xor c^8) \& x^9) \xor (y^9 \& c^8)$.\\
\end{center}
Assumption: \texttt{Stuck-at-0} fault at $x^9$\\
Now, decryption failure will occur if after giving fault the new message $m'[i] \neq m[i]$. It is possible if new $c'^9 \neq c^9$. That means $c'^9 \neq c^9$ happens if $x^9 = 1$ and $(y^9 \xor c^8) = 1$, it implies $v[i]^9 = x^9 \xor y^9 \xor c^8 = 1 \xor 1 = 0$. \\
As we mentioned earlier each $v[i] = x + y$ can be divided into two shares in $1024$ possible ways and, the decryption failure only occurs in $512$ combinations out of $1024$ possible ways. It happens because in other $512$ combinations, $x^9$ is already $0$ and \texttt{Stuck-at-0} does not induce any fault.


\subsection{\texttt{Stuck-at-1} fault at one share of the $9$-th bit of $v[i]$}

Like \texttt{Stuck-at-0} fault, similar situation arises for \texttt{Stuck-at-1} fault at one share of the $9$-th bit of $v[i]$. The values of $v[i]$ cause decryption failure are shown inside the red rectangle in the Figure \ref{fig:stuck-at-1}.

\begin{figure}[htp]
    \centering
    \includegraphics[width=14cm]{images/stuck_1.png}
    \caption{Stuck-at-1 fault}
    \label{fig:stuck-at-1}
\end{figure}
Assumption: \texttt{Stuck-at-1} fault at $x^9$\\
Similarly, decryption failure will occur if after fault the new message $m'[i] \neq m[i]$, i.e. if new $c'^9 \neq c^9$. That means $c'^9 \neq c^9$ happens if $x^9 = 0$ and $(y^9 \xor c^8) (\neq 0) = 1$, it implies $v[i]^9 = x^9 \xor y^9 \xor c^8 = 0 \xor 1 = 1$. \\
Like previous case, each $v[i] = x + y$ can be divided into two shares in $1024$ possible ways and, the decryption failure only occurs in $512$ combinations out of $1024$ possible ways. It happens here because in other $512$ combinations, $x^9$ is already $1$ and \texttt{Stuck-at-1} does not induce any fault.

==> old_sections/masking_saber.tex <==
\section{Masking Saber}

\input{images/saberunmasked}

\input{images/sabermasked}

\subsection{Arithmetic operations}
\newpage
\subsection{Compression} \label{subsec:compresssion} 

\begin{algorithm}[!ht]
\caption{ Secure Arithmetic to Boolean conversion (A2B)~\cite{Coron2014_A2B} }
\label{algo:A2B}

\Input{$\{A_i\}_{1\leq i \leq n}$ such that $\sum_{i=1}^{n} A_i = {x} \in \mathbb{R}_q $}
\Output{$\{y_i\}_{1\leq i \leq n}$ where each $ y_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{n} y_i = x$}
\BlankLine
\If{$n=1$} {$y_1 \leftarrow A_1$\\ \algorithmicreturn{ $y_1$}} 
\Else{
$\{u_i\}_{1\leq i \leq \lfloor n/2\rfloor} \leftarrow \mathtt{A2B} (\{A_i\}_{1\leq i \leq \lfloor n/2\rfloor})$\\
$\{u_i\}_{1\leq i \leq n} \leftarrow \mathtt{RefreshXOR} (\{u_i\}_{1\leq i \leq \lfloor n/2\rfloor},n,k)$\\
$\{v_i\}_{1\leq i \leq \lceil n/2\rceil} \leftarrow \mathtt{A2B} (\{A_i\}_{\lfloor n/2\rfloor + 1\leq i \leq n })$\\
$\{v_i\}_{1\leq i \leq n} \leftarrow \mathtt{RefreshXOR}(\{v_i\}_{1\leq i \leq \lfloor n/2\rfloor},n,k)$\\
$\{y_i\}_{1\leq i \leq n} \leftarrow \mathtt{SecAdd}(\{u_i\}_{1\leq i \leq n},\{v_i\}_{1\leq i \leq n})$\\
\algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}
}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{ RefreshXOR~\cite{Coron2014_A2B}}
\label{algo:RefreshXOR}

\Input{$(\{x_i\}_{1\leq i \leq m}, n, k)$ where each $x_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{m} x_i = x$}
\Output{$\{y_i\}_{1\leq i \leq n}$ with each $y_i \in \mathbb{R}_2^k$ such that $\bigoplus_{i=1}^{n} y_i = x$}
\BlankLine
\For{\texttt{i=1 to n}}
{
    $y_i\leftarrow x_i$\\
}
\For{\texttt{i=1 to n-1}}
{
   \For{\texttt{j=i+1 to n}}
    {
        $r\leftarrow \mathcal{U}(\mathbb{R}_2^k)$\\
        $y_i\leftarrow y_i\xor r$\\
        $y_j\leftarrow y_j\xor r$\\
    }
}
\algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}

\end{algorithm}

\begin{algorithm}[!ht]
\caption{ SecAdd~\cite{Coron2014_A2B} }
\label{algo:SecAdd}

\Input{$\{x_i\}_{1\leq i \leq n}$, $\{y_i\}_{1\leq i \leq n}$ with each $x_i,y_i \in \mathbb{R}_2^k$ such that $\bigoplus_{i=1}^{m} x_i = x$ and $\bigoplus_{i=1}^{m} y_i = y$}
\Output{$\{z_i\}_{1\leq i \leq n}$ where each $z_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{m} z_i = x+y \mod{2^k}$}
\BlankLine
$\{c_i^{(0)}\}_{1\leq i \leq n}\leftarrow 0$\\
\For{\texttt{j=0 to k-2 }}
{
    $\{xy_i^{(j)}\}_{1\leq i \leq n} \leftarrow \mathtt{SecAnd}(\{x_i^{(j)}\}_{1\leq i \leq n},\{y_i^{(j)}\}_{1\leq i \leq n})$\\
    $\{xc_i^{(j)}\}_{1\leq i \leq n} \leftarrow \mathtt{SecAnd}(\{x_i^{(j)}\}_{1\leq i \leq n},\{c_i^{(j)}\}_{1\leq i \leq n})$\\
    $\{yc_i^{(j)}\}_{1\leq i \leq n} \leftarrow \mathtt{SecAnd}(\{y_i^{(j)}\}_{1\leq i \leq n},\{c_i^{(j)}\}_{1\leq i \leq n})$\\
    $\{c_i^{(j+1)}\}_{1\leq i \leq n} \leftarrow \{(xy_i^{(j)})\}_{1\leq i \leq n}\xor \{(xc_i^{(j)})\}_{1\leq i \leq n}\xor \{(yc_i^{(j)})\}_{1\leq i \leq n}$\\
}
$\{z_i\}_{1\leq i \leq n} = \{x_i\}_{1\leq i \leq n} \xor \{y_i\}_{1\leq i \leq n} \xor \{c_i\}_{1\leq i \leq n}$ \\
\algorithmicreturn{ $\{z_i\}_{1\leq i \leq n}$}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{ SecAdd (new)~\cite{BronchainC22} }
\label{algo:SecAdd}

\Input{$\{x_i\}_{1\leq i \leq n}$, $\{y_i\}_{1\leq i \leq n}$ with each $x_i,y_i \in \mathbb{R}_2^k$ such that $\bigoplus_{i=1}^{m} x_i = x$ and $\bigoplus_{i=1}^{m} y_i = y$}
\Output{$\{z_i\}_{1\leq i \leq n}$ where each $z_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{m} z_i = x+y \mod{2^k}$}
\BlankLine
$\{c_i^{(0)}\}_{1\leq i \leq n}\leftarrow 0$\\
\For{\texttt{j=0 to k-2 }}
{
    $\{xXORy_i^{(j)}\}_{1\leq i \leq n} \leftarrow \{x_i^{(j)}\}_{1\leq i \leq n} \xor \{y_i^{(j)}\}_{1\leq i \leq n}$\\
    $\{xXORc_i^{(j)}\}_{1\leq i \leq n} \leftarrow \{x_i^{(j)}\}_{1\leq i \leq n} \xor \{c_i^{(j)}\}_{1\leq i \leq n}$\\
    $\{xXORy\&xXORc_i^{(j)}\}_{1\leq i \leq n} \leftarrow \mathtt{SecAnd}(\{xXORy_i^{(j)}\}_{1\leq i \leq n},\{xXORc_i^{(j)}\}_{1\leq i \leq n})$\\
    $\{c_i^{(j+1)}\}_{1\leq i \leq n} \leftarrow \{xXORy\&xXORc_i^{(j)}\}_{1\leq i \leq n}\xor \{x_i\}_{1\leq i \leq n}$\\
}
$\{z_i\}_{1\leq i \leq n} = \{x_i\}_{1\leq i \leq n} \xor \{y_i\}_{1\leq i \leq n} \xor \{c_i\}_{1\leq i \leq n}$ \\
\algorithmicreturn{ $\{z_i\}_{1\leq i \leq n}$}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{ SecAnd~\cite{Coron2014_A2B} }
\label{algo:SecAnd}

\Input{$\{x_i\}_{1\leq i \leq n}$, $\{y_i\}_{1\leq i \leq n}$ with each $x_i,y_i \in \mathbb{R}_2^k$ such that $\bigoplus_{i=1}^{m} x_i = x$ and $\bigoplus_{i=1}^{m} y_i = y$}
\Output{$\{z_i\}_{1\leq i \leq n}$ where each $z_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{m} z_i = x \wedge y $}
\BlankLine
\For{\texttt{i=1 to n}}
{
    $z_i\leftarrow x_i\wedge y_i$\\
}
\For{\texttt{i=1 to n-1}}
{
   \For{\texttt{j=i+1 to n}}
    {
        $r_{i,j}\leftarrow \mathcal{U}(\mathbb{R}_2^k)$\\
        $r_{j,i}\leftarrow (x_i\wedge y_j)\xor r_{i,j}$\\
        $r_{j,i}\leftarrow (x_j\wedge y_i)\xor r_{j,i}$\\
        $z_i\leftarrow z_i\xor r_{i,j}$\\
        $z_j\leftarrow z_j\xor r_{j,i}$\\
    }
}
\algorithmicreturn{ $\{z_i\}_{1\leq i \leq n}$}
\end{algorithm}

\clearpage
\subsection{Masked centered binomial sampler} \label{subsec:binomial_sampler}


% \begin{algorithm}[!ht]
% \caption{ Masked centered binomial sampler~\cite{Tobias2019_binomial_sampler} }
% \label{algo:SecSampler}

% \Input{$\{x_i\}_{0\leq i \leq n},\{y_i\}_{0\leq i \leq n}$ where $x_i,y_i \in \mathbb{R}_2^\kappa$ such that $\bigoplus_{i=0}^{n} x_i = x, \bigoplus_{i=0}^{n} y_i = y$}
% \Output{$\{A_i\}_{0\leq i \leq n}$ where  $A_i \in \mathbb{R}_q$ and $\sum_{i=0}^{n} A_i =$ $($\texttt{HW}$(x)-$ \texttt{HW}$(y)) \bmod q $}
% \BlankLine

% $\{z_i\}_{0\leq i \leq n}\leftarrow$ \texttt{SecBitAdd}$(\{x_i\}_{0\leq i \leq n})$~\cite{FO-masked-saber} \\
% $\{z_i\}_{0\leq i \leq n}\leftarrow$ \texttt{SecBitSub}$(\{z_i\}_{0\leq i \leq n},\{y_i\}_{0\leq i \leq n})$~\cite{Tobias2019_binomial_sampler} \\
% $\{z_i\}_{0\leq i \leq n}\leftarrow$ \texttt{SecConstAdd}$(\{z_i\}_{0\leq i \leq n})$~\cite{FO-masked-saber}\\
% $\{A_i\}_{0\leq i \leq n}\leftarrow$ \texttt{B2A}$(\{z_i\}_{0\leq i \leq n})$~\cite{Bettale2018_B2A}\\
% $A_1\leftarrow (A_1- \mu/2) \bmod q$\\

% \algorithmicreturn{ $\{y_i\}_{0\leq i \leq n}$}
% \end{algorithm}

\begin{algorithm}[!ht]
\caption{ Masked centered binomial sampler~\cite{Tobias2019_binomial_sampler} }
\label{algo:SecSampler}

\Input{$\{x_i\}_{0\leq i \leq n},\{y_i\}_{0\leq i \leq n}$ where $x_i,y_i \in \mathbb{R}_2^\kappa$ such that $\bigoplus_{i=0}^{n} x_i = x, \bigoplus_{i=0}^{n} y_i = y$}
\Output{$\{A_i\}_{0\leq i \leq n}$ where  $A_i \in \mathbb{R}_q$ and $\sum_{i=0}^{n} A_i =$ $($\texttt{HW}$(x)-$ \texttt{HW}$(y)) \bmod q $}
\BlankLine

$\{z_i\}_{0\leq i \leq n}\leftarrow$ \texttt{SecBitAdd}$(\{x_i\}_{0\leq i \leq n})$~\cite{FO-masked-saber} \\
$\{z_i\}_{0\leq i \leq n}\leftarrow$ \texttt{SecBitSub}$(\{z_i\}_{0\leq i \leq n},\{y_i\}_{0\leq i \leq n})$~\cite{Tobias2019_binomial_sampler} \\
$\{z_i\}_{0\leq i \leq n}\leftarrow$ \texttt{SecConstAdd}$(\{z_i\}_{0\leq i \leq n})$~\cite{FO-masked-saber}\\
$\{A_i\}_{0\leq i \leq n}\leftarrow$ \texttt{B2A}$(\{z_i\}_{0\leq i \leq n})$~\cite{Bettale2018_B2A}\\
$A_1\leftarrow (A_1- \mu/2) \bmod q$\\

\algorithmicreturn{ $\{y_i\}_{0\leq i \leq n}$}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{ SecBitAdd~\cite{Tobias2019_binomial_sampler} }
\label{algo:SecBitAdd}

\Input{$\{x_i\}_{1\leq i \leq n}$ where $x_i \in \mathbb{R}_2^\kappa$ such that $\bigoplus_{i=1}^{n} x_i = x$ and $\lambda=\lceil \log_2(\kappa+1)\rceil+1$}
\Output{$\{z_i\}_{1\leq i \leq n}$ where each $z_i \in \mathbb{R}_2^\lambda$ and $\bigoplus_{i=1}^{n} z_i =$ HW$(x) $}
\BlankLine

$\{z_i\}_{1\leq i \leq n}\leftarrow 0$\\
\For{\texttt{j=1 to $\kappa$}}
{
   $\{t_i[1]\}_{1\leq i \leq n}\leftarrow \{z_i[1]\}_{1\leq i \leq n} \xor \{x_i[j]\}_{1\leq i \leq n}$ \\
   $\{w_i\}_{1\leq i \leq n}\leftarrow \{x_i[j]\}_{1\leq i \leq n}$ \\
   \For{\texttt{l=2 to $\lambda$}}
    {
       $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\{z_i[l-1]\}_{1\leq i \leq n})$ \\
       $\{t_i[l]\}_{1\leq i \leq n}\leftarrow \{z_i[l]\}_{1\leq i \leq n} \xor \{w_i\}_{1\leq i \leq n}$ \\
    }
    $\{z_i\}_{1\leq i \leq n}\leftarrow \{t_i\}_{1\leq i \leq n}$\\
}
\algorithmicreturn{ $\{z_i\}_{1\leq i \leq n}$}
\end{algorithm}


\begin{algorithm}[!ht]
\caption{ SecBitSub~\cite{Tobias2019_binomial_sampler} }
\label{algo:SecBitSub}

\Input{$\{y_i\}_{1\leq i \leq n},\{z_i\}_{1\leq i \leq n}$ where $y_i,z_i \in \mathbb{R}_2^\kappa$ such that $\bigoplus_{i=1}^{n} y_i = y, \bigoplus_{i=1}^{n} z_i = z$ and $\lambda=\lceil \log_2(\kappa+1)\rceil+1$}
\Output{$\{z_i\}_{1\leq i \leq n}$ where each $z_i \in \mathbb{R}_2^\lambda$ and $\bigoplus_{i=1}^{m} z_i = z-$HW$(y) $}
\BlankLine

$\{t_i\}_{1\leq i \leq n}\leftarrow 0$\\
\For{\texttt{j=1 to $\kappa$}}
{
   $\{t_i[1]\}_{1\leq i \leq n}\leftarrow \{z_i[1]\}_{1\leq i \leq n} \xor \{y_i[j]\}_{1\leq i \leq n}$ \\
   $\{w_i\}_{1\leq i \leq n}\leftarrow \{y_i[j]\}_{1\leq i \leq n}$ \\
   \For{\texttt{l=2 to $\lambda$}}
    {
        $\{u_i[l]\}_{1\leq i \leq n}\leftarrow \{z_i[l-1]\}_{1\leq i \leq n}$ \\
        $u_1\leftarrow ~u_1$ \\
        $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\{u_i\}_{1\leq i \leq n})$ \\
        $\{t_i[l]\}_{1\leq i \leq n}\leftarrow \{z_i[l]\}_{1\leq i \leq n} \xor \{w_i\}_{1\leq i \leq n}$ \\
    }
    $\{z_i\}_{1\leq i \leq n}\leftarrow \{t_i\}_{1\leq i \leq n}$\\
}
\algorithmicreturn{ $\{z_i\}_{1\leq i \leq n}$}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{ SecConstAdd~\cite{Tobias2019_binomial_sampler} }
\label{algo:SecConstAdd}

\Input{$\{x_i\}_{1\leq i \leq n}$ where $x_i \in \mathbb{R}_2^\lambda$ such that $\bigoplus_{i=1}^{n} x_i = x$}
\Output{$\{y_i\}_{1\leq i \leq n}$ where each $y_i \in \mathbb{R}_2^\lambda$ and $\bigoplus_{i=1}^{n} y_i =x+4 $}
\BlankLine

$\{y_i\}_{1\leq i \leq n}\leftarrow \{x_i\}_{1\leq i \leq n}$\\
$\{y_i[3]\}_{1\leq i \leq n}\leftarrow \{y_i[3]\}_{1\leq i \leq n} \xor \{y_i[2]\}_{1\leq i \leq n}$\\
$y_0[2]\leftarrow y_0[2]\xor 1$\\

\algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}
\end{algorithm}


% \begin{algorithm}[!ht]
% \caption{ Binomial Sampler (SecSampler)~\cite{Tobias2019_binomial_sampler} }
% \label{algo:SecSampler}

% \Input{$\{x_i\}_{1\leq i \leq n},\{y_i\}_{1\leq i \leq n}$ where $x_i,y_i \in \mathbb{R}_2^\kappa$ such that $\bigoplus_{i=1}^{n} x_i = x, \bigoplus_{i=1}^{n} y_i = y$}
% \Output{$\{A_i\}_{1\leq i \leq n}$ where  $A_i \in \mathbb{R}_q$ and $\sum_{i=1}^{n} A_i =$ HW$(x)-$ HW$(y) \mod q $}
% \BlankLine

% $\{z_i\}_{1\leq i \leq n}\leftarrow$ SecBitAdd$(\{x_i\}_{1\leq i \leq n})$\\
% $\{z_i\}_{1\leq i \leq n}\leftarrow$ SecBitSub$(\{z_i\}_{1\leq i \leq n},\{y_i\}_{1\leq i \leq n})$\\
% $\{z_i\}_{1\leq i \leq n}\leftarrow$ SecConstAdd$(\{z_i\}_{1\leq i \leq n})$\\
% $\{A_i\}_{1\leq i \leq n}\leftarrow$ B2A$(\{z_i\}_{1\leq i \leq n})$\\
% $A_1\leftarrow A_1-\kappa \mod q$\\

% \algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}
% \end{algorithm}


\begin{algorithm}[!ht]
\caption{ Secure Boolean to Arithmetic conversion (B2A)~\cite{Bettale2018_B2A} }
\label{algo:B2A}

\Input{$\{y_i\}_{1\leq i \leq n}$ where each $ y_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{n} y_i = x$}
\Output{$\{A_i\}_{1\leq i \leq n}$ such that $\sum_{i=1}^{n} A_i = {x} \in \mathbb{R}_q $}

\BlankLine
$\{A_i\}_{1\leq i \leq n} \leftarrow \mathtt{RecB2A}(\{y_i\}_{1\leq i \leq n},0)$\\
\algorithmicreturn{ $\{A_i\}_{1\leq i \leq n}$}

\end{algorithm}


\begin{algorithm}[!ht]
\caption{ RecB2A (n+1 shares to n shares)~\cite{Bettale2018_B2A} }
\label{algo:B2A}

\Input{$\{y_i\}_{1\leq i \leq n+1}$ where each $ y_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{n+1} y_i = x$}
\Output{$\{A_i\}_{1\leq i \leq n}$ such that $\sum_{i=1}^{n} A_i = {x} \in \mathbb{R}_q $}

\BlankLine

\If{n=1}{
$A_1\leftarrow x_1\xor x_2$\\
\algorithmicreturn{ $A_1$}
}
\Else{
$\{z_i\}_{1\leq i \leq n+1}\leftarrow RefreshMask(\{y_i\}_{1\leq i \leq n+1},k)$\\
$x_1\leftarrow \overline{(n\wedge 1)}\cdot z_1 \xor ((z_1\xor z_2)-z_2)$\\
\For{\texttt{i=2 to n}}
{
    $x_i\leftarrow(z_1\xor z_{i+1}) - z_{i+1}$\\
}
$\{B_i\}_{1\leq i \leq n} \leftarrow \mathtt{RecB2A}(\{z_i\}_{2\leq i \leq n+1})$\\
$\{C_i\}_{1\leq i \leq n} \leftarrow \mathtt{RecB2A}(\{x_i\}_{1\leq i \leq n})$\\
\For{\texttt{i=1 to n-2}}
{
    $A_i\leftarrow B_i+C_i$\\
}
$A_{n-1}\leftarrow B_{n-1}$\\
$A_{n}\leftarrow C_{n-1}$\\
\algorithmicreturn{$\{A_i\}_{1\leq i \leq n}$}}

\end{algorithm}


\begin{algorithm}[!ht]
\caption{ RefreshMask~\cite{Bettale2018_B2A} }
\label{algo:RefreshMask}

\Input{$(\{x_i\}_{1\leq i \leq n}, k)$ where each $x_i \in \mathbb{R}_2^k$ and $\bigoplus_{i=1}^{n} x_i = x$}
\Output{$\{y_i\}_{1\leq i \leq n}$ with each $y_i \in \mathbb{R}_2^k$ such that $\bigoplus_{i=1}^{n} y_i = x$}

\BlankLine

$y_1\leftarrow x_1$\\

\For{\texttt{i=2 to n}}
{
   $r\leftarrow \mathcal{U}(\mathbb{R}_2^k)$\\
    $y_i\leftarrow x_i\xor r$\\
    $y_1\leftarrow y_1\xor r$\\
}
\algorithmicreturn{ $\{y_i\}_{1\leq i \leq n}$}

\end{algorithm}
%\clearpage
%\subsection{Masked hashing}\label{subsec:mask_hashing}


\clearpage
\subsection{Masked Comparison}

% \begin{algorithm}[!ht]
% \caption{ Masked Comparison (MaskComp) }
% \label{algo:MaskComp}

% \Input{$\{\mathbf{b}'_i\}_{1\leq i \leq n}$ where each $\mathbf{b}'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} \mathbf{b}'_i = \mathbf{b}'$,\\
% $\{c'_i\}_{1\leq i \leq n}$ where each $c'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} c'_i = c'$,\\
% publicly avilable $\mathbf{b}$ and $c$}
% \Output{$\{b_i\}_{1\leq i \leq n}$ with each $b_i \in \{0,1\}$ such that $\bigoplus_{i=1}^{n} b_i = 1$ iff\\ $\mathbf{b}''=\mathbf{b}'>>(\epsilon_q-\epsilon_p)=3$ and $c''=c'>>(\epsilon_p-\epsilon_t)=6$, else $0$}
% \BlankLine

% //\texttt{for $\mathbf{b}$ part of ciphertext}\\
% \For{\texttt{j1=} $1$ \texttt{to } $l=3$}
% {
%     \For{\texttt{j2=} $1$ \texttt{to } $N=256$}
%     {
%         $\mathbf{eb}[j1][j2]\leftarrow(\mathbf{b}[j1][j2]<<3)+8$\\
%         $\mathbf{b}'_{n}[j1][j2]\leftarrow \mathbf{b}'_{n}[j1][j2]-\mathbf{eb}[j1][j2]$\\
%          $\{\mathbf{y}_i[j1][j2]\}_{1\leq i \leq n}\leftarrow$ A2B$(\{\mathbf{b}'_i[j1][j2]\}_{1\leq i \leq n})$\\
    
%         \For{\texttt{s=} $1$ \texttt{to } $\epsilon_p=10$}
%         {
%             $\{\mathbf{x}_i[s][j1][j2]\}_{1\leq i \leq n}\leftarrow (\{\mathbf{y}_i[j1][j2]\}_{1\leq i \leq n}>>(s+3-1))$\\
%         }
%     }
%     \For{\texttt{s=} $1$ \texttt{to } $\epsilon_p=10$}
%     {
%         $\{\mathbf{u}_i[s][j1]\}_{1\leq i \leq n}\leftarrow$ Bitslice$(\{\mathbf{x}_i[s][j1]\}_{1\leq i \leq n})$
%     }
% }

% //\texttt{for $c$ part of ciphertext}\\
% \For{\texttt{j2=} $1$ \texttt{to } $N=256$}
% {
%     $ec[j2]\leftarrow(c[j2]<<6)+64$\\
%     $c'_{n}[j2]\leftarrow c'_{n}[j2]-ec[j2]$\\
%     $\{y_i[j2]\}_{1\leq i \leq n}\leftarrow$ A2B$(\{c'_i[j2]\}_{1\leq i \leq n})$\\

%     \For{\texttt{s=} $1$ \texttt{to } $\epsilon_t=4$}
%     {
%         $\{z_i[s][j2]\}_{1\leq i \leq n}\leftarrow(\{y_i[j2]\}_{1\leq i \leq n}>>(s+6-1))$\\
%     }
% }
% \For{\texttt{s=} $1$ \texttt{to } $\epsilon_t=4$}
% {
%     $\{v_i[s]\}_{1\leq i \leq n}\leftarrow$ Bitslice$(\{z_i[s]\}_{1\leq i \leq n})$
% }
% //Secure And on results of both parts of ciphertexts\\
% $\{w_i\}_{1\leq i \leq n}\leftarrow \{v_i[1]\}_{1\leq i \leq n}$\\
% \For{\texttt{s=} $2$ \texttt{to } $\epsilon_t=4$}
% {
%     $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\{v_i[s]\}_{1\leq i \leq n})$\\
% }
% \For{\texttt{j=} $1$ \texttt{to } $l=3$}
% {
%     $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow \{\mathbf{u}_i[1][j]\}_{1\leq i \leq n}$\\
%     \For{\texttt{s=} $2$ \texttt{to } $\epsilon_p=10$}
%     {
%         $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{\mathbf{y}_i[j]\}_{1\leq i \leq n},\{\mathbf{u}_i[s][j]\}_{1\leq i \leq n})$\\
%     }
% }
% \For{\texttt{j=} $1$ \texttt{to } $l=3$}
% {
%     $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\mathbf{y}_i[j]\}_{1\leq i \leq n})$\\
% }
% \For{\texttt{j=} $\log_2 256-1$ \texttt{to } $0$}
% {
%     $\{w'_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n}>>2^j $\\
%     $\{w_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n} \mod(2^{2^j}-1)$\\
%     $\{w_i\}_{1\leq i \leq n}\leftarrow SecAnd(\{w_i\}_{1\leq i \leq n}, \{w'_i\}_{1\leq i \leq n})$\\
% }
% $\{b_i\}_{1\leq i \leq n}\leftarrow \{w_i\}_{1\leq i \leq n}$\\
% \algorithmicreturn{ $\{b_i\}_{1\leq i \leq n}$}
% \end{algorithm}

% \begin{algorithm}[!ht]
% \caption{ Masked Comparison (MaskComp) }
% \label{algo:MaskComp}

% \Input{$\{\mathbf{b}'_i\}_{1\leq i \leq n}$ where each $\mathbf{b}'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} \mathbf{b}'_i = \mathbf{b}'$,\\
% $\{c'_i\}_{1\leq i \leq n}$ where each $c'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} c'_i = c'$,\\
% publicly avilable $\mathbf{b}$ and $c$}
% \Output{$\{b_i\}_{1\leq i \leq n}$ with each $b_i \in \{0,1\}$ such that $\bigoplus_{i=1}^{n} b_i = 1$ iff\\ $\mathbf{b}''=\mathbf{b}'>>(\epsilon_q-\epsilon_p)=3$ and $c''=c'>>(\epsilon_p-\epsilon_t)=6$, else $0$}
% \BlankLine

% //\texttt{for $\mathbf{b}$ part of ciphertext}\\
% \For{\texttt{j1=} $1$ \texttt{to } $l=3$}
% {
%     \For{\texttt{j2=} $1$ \texttt{to } $N=256$}
%     {
%         $\mathbf{eb}[j1][j2]\leftarrow(\mathbf{b}[j1][j2]<<3)+8$\\
%         $\mathbf{b}'_{n}[j1][j2]\leftarrow \mathbf{b}'_{n}[j1][j2]-\mathbf{eb}[j1][j2]$\\
%          $\{\mathbf{y}_i[j1][j2]\}_{1\leq i \leq n}\leftarrow$ A2B$(\{\mathbf{b}'_i[j1][j2]\}_{1\leq i \leq n})$\\
    
%         \For{\texttt{s=} $1$ \texttt{to } $\epsilon_p=10$}
%         {
%             $\{\mathbf{x}_i[s][j1][j2]\}_{1\leq i \leq n}\leftarrow (\{\mathbf{y}_i[j1][j2]\}_{1\leq i \leq n}>>(s+3-1))$\\
%         }
%     }
%     \For{\texttt{s=} $1$ \texttt{to } $\epsilon_p=10$}
%     {
%         $\{\mathbf{u}_i[s][j1]\}_{1\leq i \leq n}\leftarrow$ Bitslice$(\{\mathbf{x}_i[s][j1]\}_{1\leq i \leq n})$
%     }
% }

% //\texttt{for $c$ part of ciphertext}\\
% \For{\texttt{j2=} $1$ \texttt{to } $N=256$}
% {
%     $ec[j2]\leftarrow(c[j2]<<6)+64$\\
%     $c'_{n}[j2]\leftarrow c'_{n}[j2]-ec[j2]$\\
%     $\{y_i[j2]\}_{1\leq i \leq n}\leftarrow$ A2B$(\{c'_i[j2]\}_{1\leq i \leq n})$\\

%     \For{\texttt{s=} $1$ \texttt{to } $\epsilon_t=4$}
%     {
%         $\{z_i[s][j2]\}_{1\leq i \leq n}\leftarrow(\{y_i[j2]\}_{1\leq i \leq n}>>(s+6-1))$\\
%     }
% }
% \For{\texttt{s=} $1$ \texttt{to } $\epsilon_t=4$}
% {
%     $\{v_i[s]\}_{1\leq i \leq n}\leftarrow$ Bitslice$(\{z_i[s]\}_{1\leq i \leq n})$
% }
% //Secure And on results of both parts of ciphertexts\\
% $\{w_i\}_{1\leq i \leq n}\leftarrow \{v_i[1]\}_{1\leq i \leq n}$\\
% \For{\texttt{s=} $2$ \texttt{to } $\epsilon_t=4$}
% {
%     $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\{v_i[s]\}_{1\leq i \leq n})$\\
% }
% \For{\texttt{j=} $1$ \texttt{to } $l=3$}
% {
%     $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow \{\mathbf{u}_i[1][j]\}_{1\leq i \leq n}$\\
%     \For{\texttt{s=} $2$ \texttt{to } $\epsilon_p=10$}
%     {
%         $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{\mathbf{y}_i[j]\}_{1\leq i \leq n},\{\mathbf{u}_i[s][j]\}_{1\leq i \leq n})$\\
%     }
% }
% \For{\texttt{j=} $1$ \texttt{to } $l=3$}
% {
%     $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\mathbf{y}_i[j]\}_{1\leq i \leq n})$\\
% }
% \For{\texttt{j=} $\log_2 256-1$ \texttt{to } $0$}
% {
%     $\{w'_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n}>>2^j $\\
%     $\{w_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n} \mod(2^{2^j}-1)$\\
%     $\{w_i\}_{1\leq i \leq n}\leftarrow SecAnd(\{w_i\}_{1\leq i \leq n}, \{w'_i\}_{1\leq i \leq n})$\\
% }
% $\{b_i\}_{1\leq i \leq n}\leftarrow \{w_i\}_{1\leq i \leq n}$\\
% \algorithmicreturn{ $\{b_i\}_{1\leq i \leq n}$}
% \end{algorithm}


\begin{algorithm}[!ht]
\caption{ Simple masked comparison algorithm~\cite{CoronGMZ21} }
\label{algo:MaskComp1}

\Input{$\{\mathbf{b}'_i\}_{0\leq i \leq n}$ where each $\mathbf{b}'_i \in \mathbb{R}_{2^{\epsilon_q}}^l$ and $\bigoplus_{i=0}^{n} \mathbf{b}'_i = \mathbf{b}'$,\\
$\{c'_i\}_{0\leq i \leq n}$ where each $c'_i \in \mathbb{R}_{2^{\epsilon_p}}$ and $\bigoplus_{i=0}^{n} c'_i = c'$,\\
publicly available $\mathbf{b}$ and $c_m$}
\Output{$\{bit_i\}_{0\leq i \leq n}$ with each $bit_i \in \{0,1\}$ such that $\bigoplus_{i=0}^{n} bit_i = 1$ iff\\ $\mathbf{b}=\mathbf{b}'\gg (\epsilon_q-\epsilon_p)$ and $c_m=c'\gg (\epsilon_p-\epsilon_t)$, else $0$}
\BlankLine
\BlankLine
//\text{For $\mathbf{b}$ part of ciphertext}\\
$\{\mathbf{y}_i\}_{0\leq i \leq n}\leftarrow$ \texttt{A2B}$(\{\mathbf{b}'_i\}_{0\leq i \leq n})$\\
    
$\{\mathbf{y}_i\}_{0\leq i \leq n}\leftarrow (\{\mathbf{y}_i\}_{0\leq i \leq n}\gg (\epsilon_q-\epsilon_p))$\\
$\mathbf{y}_1\leftarrow \mathbf{y}_1 \xor \mathbf{b} $\\
\BlankLine
//\text{For $c_m$ part of ciphertext}\\
$\{x_i\}_{0\leq i \leq n}\leftarrow$ \texttt{A2B}$(\{c'_i\}_{0\leq i \leq n})$\\
$\{x_i\}_{0\leq i \leq n}\leftarrow(\{x_i\}_{0\leq i \leq n}\gg (\epsilon_p-\epsilon_t))$\\
${x}_1\leftarrow {x}_1 \xor {c_m}$\\
\BlankLine
//\text{Boolean circuit to test all bits of each coefficient of $(\mathbf{y},x)$ is $0$} \\
$\mathbf{y}_1\leftarrow \lnot \mathbf{y}_1 $\\
${x}_1\leftarrow \lnot {x}_1$\\
$\{bit_i\}_{0\leq i \leq n}\leftarrow$ \texttt{BooleanAllBitsOneTest} $(\{\mathbf{y}_i\}_{0\leq i \leq n},\{{x}_i\}_{0\leq i \leq n},\epsilon_p,\epsilon_t)$\\
\BlankLine
\algorithmicreturn{ $\{bit_i\}_{0\leq i \leq n}$}
\end{algorithm}


\begin{algorithm}[!ht]
\caption{ BooleanAllBitsOneTest }
\label{algo:BooleanAllBitsOneTest}

\Input{$\{\mathbf{y}_i\}_{0\leq i \leq n}$ where each $\mathbf{y}_i \in \mathbb{R}_{2^\mathtt{bmod1}}^l$ and $\bigoplus_{i=0}^{n} \mathbf{y}_i = \mathbf{y}$,\\
$\{x_i\}_{0\leq i \leq n}$ where each $x_i \in \mathbb{R}_{2^\mathtt{bmod2}}$ and $\bigoplus_{i=0}^{n} x_i = x$,\\
$\mathtt{bmod1}$, and $\mathtt{bmod2}$}
\Output{$\{bit_i\}_{0\leq i \leq n}$ with each $bit_i \in \{0,1\}$ such that $\bigoplus_{i=0}^{n} bit_i = 1$ iff\\ each bit of every coefficients of $\mathbf{y}$ and ${x}$ is $1$, else $0$}
\BlankLine
\BlankLine
\For{$\mathtt{j_1=}$ $1$ \texttt{to } $l$}
{
    \For{\texttt{s=} $1$ \texttt{to } $\mathtt{bmod1}$}
    {
        $\{\mathbf{u}_i[s][j_1]\}_{0\leq i \leq n}\leftarrow$ \texttt{Bitslice}$(\{\mathbf{y}_i^{(s)}[j_1]\}_{0\leq i \leq n})$
    }
}
\For{\texttt{s=} $1$ \texttt{to } $\mathtt{bmod2}$}
{
    $\{v_i[s]\}_{0\leq i \leq n}\leftarrow$ \texttt{Bitslice}$(\{x_i^{(s)}\}_{0\leq i \leq n})$
}
//Secure And on both \\
$\{w_i\}_{0\leq i \leq n}\leftarrow \{v_i[1]\}_{0\leq i \leq n}$\\
\For{\texttt{s=} $2$ \texttt{to } $\mathtt{bmod2}$}
{
    $\{w_i\}_{0\leq i \leq n}\leftarrow$ \texttt{SecAnd}$(\{w_i\}_{0\leq i \leq n},\{v_i[s]\}_{0\leq i \leq n})$\\
}
\For{\texttt{j=} $1$ \texttt{to } $l$}
{
    $\{\mathbf{y}_i[j]\}_{0\leq i \leq n}\leftarrow \{\mathbf{u}_i[1][j]\}_{0\leq i \leq n}$\\
    \For{\texttt{s=} $2$ \texttt{to } $\mathtt{bmod1}$}
    {
        $\{\mathbf{y}_i[j]\}_{0\leq i \leq n}\leftarrow$ \texttt{SecAnd}$(\{\mathbf{y}_i[j]\}_{0\leq i \leq n},\{\mathbf{u}_i[s][j]\}_{0\leq i \leq n})$\\
    }
    $\{w_i\}_{0\leq i \leq n}\leftarrow$ \texttt{SecAnd}$(\{w_i\}_{0\leq i \leq n},\mathbf{y}_i[j]\}_{0\leq i \leq n})$\\
}
\For{\texttt{j=} $\log_2 (256)-1$ \texttt{to } $0$}
{
    $\{w'_i\}_{0\leq i \leq n}\leftarrow w_{0\leq i \leq n}\gg 2^j $\\
    $\{w_i\}_{0\leq i \leq n}\leftarrow w_{0\leq i \leq n} \bmod{(2^{2^j})}$\\
    $\{w_i\}_{0\leq i \leq n}\leftarrow$ \texttt{SecAnd}$(\{w_i\}_{0\leq i \leq n}, \{w'_i\}_{0\leq i \leq n})$\\
}
$\{bit_i\}_{0\leq i \leq n}\leftarrow \{w_i\}_{0\leq i \leq n}$\\
\algorithmicreturn{ $\{bit_i\}_{0\leq i \leq n}$}
\end{algorithm}




==> old_sections/old_preliminaries.tex <==
\section{Preliminaries}\label{sec:prelims}

\subsection{Notation}

The $k$-th bit of an integer $u \in \mathbb{Z}$ is denoted as $u^k$. $\mathbb{Z}_q$ is a ring of integer modulo $q$ and ${R}_q$ is a polynomial ring $\mathbb{Z}_q[X]/(X^{n}+1)$. ${R}_q^l$ is a ring containing vectors with $l$ elements of ${R}_q$ and we use ${R}_q^{l\times l}$ to represent a ring with $l\times l $ matrices over ${R}_q$. We denote a single polynomial with lower case letter (e.g., $x \in {R}_q$), a vector of polynomials with bold lower case letter (e.g., $\pmb{y} \in {R}_q^l$), and a matrix of polynomials with bold upper case letter (e.g., $\pmb{A} \in {R}_q^{l\times l}$). We denote the $i$-th ($i \in \{ 0, 1, \ldots, n-1 \}$) coefficient of a polynomial $x$ as $x[i]$ and the $i$-th ($i \in \{ 0, 1, \ldots, n-1 \}$) coefficient of $j$-th ($j \in \{ 0, 1, \ldots, l-1 \}$) polynomial in a vector of polynomials $\mathbf{y}$ as $\mathbf{y}[j][i]$. If an element $v$ is sampled from a set $S$ according to a distribution $\chi$, we present it by $v \leftarrow \chi(S)$. However, if the element $v$ of the set $S$ is generated from a $seed_v$ with the help of pseudorandom number generator $\chi$, then we denote it by $v \leftarrow \chi(S; seed_v)$. We use $\mathcal{U}$ as uniform distribution, and $\mathcal{\beta_\mu}$ as centered binomial distribution (CBD) with standard deviation $\sqrt{\mu/2}$. $\xor$ denotes bit-wise XOR operation and $\&$ denotes bit-wise AND operation. $\lfloor w \rceil$ represents the rounding operation that outputs the closest integer of $w$ and is rounded upwards in case of ties (i.e., if $w = 1/2$ then $\lfloor w \rceil = 1$). $w \ll b$ indicates the logical shifting of $w$ by $b$ positions left, and $w \gg b$ indicates the logical shifting of $w$ by $b$ positions right. Here, $w$ is an integer, and $b$ is a natural number. These operations can be extended for a polynomial $x$ by performing them coefficient-wise (e.g., $x \gg b$ = $x[i] \gg b$, for each $i \in \{ 0, 1, \ldots, n-1 \}$).   


\subsection{Saber}\label{subsec:saber}

Saber is a chosen ciphertext attack (CCA) secure key-encapsulation mechanism (KEM), and its security depends on module learning with rounding (MLWR) problem (MLWR problem: If $\pmb{A} \leftarrow  \mathcal{U}(R^{l \times l}_q)$, $\pmb{s} \leftarrow  \mathcal{\beta_\mu}(R^{l}_q)$, $\pmb{b}' \leftarrow  \mathcal{U}(R^{l}_p)$, $q > p$ and $\pmb{b} = \lfloor (q/p)(\pmb{A} \pmb{s}) \rceil$, then ($\pmb{A}$, $\pmb{b}$) and ($\pmb{A}$, $\pmb{b}'$) are indistinguishable). It consists of three algorithms: (i) Key-generation ($\mathtt{Saber}{.}\mathtt{KEM}{.}\mathtt{KeyGen}$), (ii) Encapsulation ($\mathtt{Saber}{.}\mathtt{KEM}{.}\mathtt{Enc}$), and (iii) Decapsulation ($\mathtt{Saber}{.}\mathtt{KEM}{.}\mathtt{Dec}$), which are presented in \autoref{fig:saberkem}. The Saber KEM is constructed by using chosen plaintext attack (CPA) secure public-key encryption (PKE) together with a post-quantum version of the Fujisaki-Okamoto (FO)~\cite{Jiang2017} transformation to obtain the CCA security. The PKE of Saber also contains three algorithms: (i) Key-generation ($\mathtt{Saber}{.}\mathtt{PKE}{.}\mathtt{KeyGen}$), (ii) Encryption ($\mathtt{Saber}{.}\mathtt{PKE}{.}\mathtt{Encaps}$), and (iii) Decryption ($\mathtt{Saber}{.}\mathtt{PKE}{.}\mathtt{Decaps}$), are shown in \autoref{fig:saberpke}. 

There are three security versions of Saber named LightSaber, Saber, and FireSaber, depending on different values of the parameter set, which has given in Table~\ref{tab:Parameters_saber}. The moduli $q, p, t$ that are used to form the rings $R_q, R_p, R_t$ in Saber algorithms are all power-of-two. The number of bits in each coefficient of a polynomial of the corresponding ring can be calculated as $\log_2(q) = \epsilon_q$, $\log_2(p) = \epsilon_p$, and $\log_2(t) \epsilon_t$. A few other parameters in the Saber PKE protocol on which the security of the scheme depends are the length of vectors $l$ and $\mu$ in the CBD. $\mathcal{G},\ \mathcal{H}$, and $\mathtt{KDF}$ are three hash functions used in Saber KEM. In practice, $\mathcal{G}$ is realized by $\mathtt{SHA3-512}$ and $\mathtt{SHA3-256}$ is used for $\mathcal{H}$, and $\mathtt{KDF}$. Lastly, for performing polynomial multiplication Saber uses a combination of Toom-Cook, Karatsuba, and schoolbook multiplication. Here, we briefly describe the Saber scheme and suggest the original Saber paper \cite{Saber_kem} for further specifics. 

\input{images/saberPKE}
\input{images/saberKEM}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\scriptsize
\centering
\caption{Parameters of Saber with security and failure probability ~\cite{Saber_kem}}
\label{tab:Parameters_saber}
\resizebox{0.90\textwidth}{!}{%
\begin{tabular}{|ll|cccccc|c|c|c|}
\hline
\multicolumn{1}{|c}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Scheme\\ Name\end{tabular}}} & \multirow{3}{*}{} & \multicolumn{6}{c|}{Parameters}                                                                                                                                                                                                                          & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Post-quantum\\ Security\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Failure \\ Probability\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}NIST\\ Security \\ Level\end{tabular}} \\ \cline{3-8}
\multicolumn{1}{|c}{}                                                                       &                   & \multicolumn{1}{c|}{\multirow{2}{*}{l}} & \multicolumn{1}{c|}{\multirow{2}{*}{n}}   & \multicolumn{1}{c|}{\multirow{2}{*}{q}}        & \multicolumn{1}{c|}{\multirow{2}{*}{p}}        & \multicolumn{1}{c|}{\multirow{2}{*}{t}} & \multirow{2}{*}{$\mu$} &                                                                                  &                                                                                 &                                                                                   \\
\multicolumn{1}{|c}{}                                                                       &                   & \multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                   &                        &                                                                                  &                                                                                 &                                                                                   \\ \hline
                                                                                            &                   & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                     & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{}                                                            & \multicolumn{1}{l|}{}                                                           & \multicolumn{1}{l|}{}                                                             \\
LightSaber                                                                                  &                   & \multicolumn{1}{c|}{2}                  & \multicolumn{1}{c|}{\multirow{3}{*}{256}} & \multicolumn{1}{c|}{\multirow{3}{*}{$2^{13}$}} & \multicolumn{1}{c|}{\multirow{3}{*}{$2^{10}$}} & \multicolumn{1}{c|}{$2^{3}$}            & 5                      & $2^{107}$                                                                        & $2^{-120}$                                                                      & 1                                                                                 \\
Saber                                                                                       &                   & \multicolumn{1}{c|}{3}                  & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{$2^{4}$}            & 4                      & $2^{172}$                                                                        & $2^{-136}$                                                                      & 3                                                                                 \\
FireSaber                                                                                   &                   & \multicolumn{1}{c|}{4}                  & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{$2^{6}$}            & 3                      & $2^{236}$                                                                        & $2^{-165}$                                                                      & 5                                                                                 \\ \hline
\end{tabular}%
}
\end{table}


\subsection{Kyber}\label{subsec:kyber}

Like Saber, Kyber also is a chosen ciphertext attack (CCA) secure key-encapsulation mechanism (KEM), but its security base on module learning with errors (MLWE) problem (MLWE problem: If $\pmb{A} \leftarrow  \mathcal{U}(R^{l \times l}_q)$, $\pmb{s} \leftarrow  \mathcal{\beta_\mu}(R^{l}_q)$, $\pmb{e} \leftarrow  \mathcal{\beta_\mu}(R^{l}_q)$, $\pmb{b}' \leftarrow  \mathcal{U}(R^{l}_q)$, and $\pmb{b} = (\pmb{A} \pmb{s}) + \pmb{e}$, then ($\pmb{A}$, $\pmb{b}$) and ($\pmb{A}$, $\pmb{b}'$) are not distinguishable). Kyber KEM consists of the following algorithms: (i) Key-generation ($\mathtt{Kyber}{.}\mathtt{KEM}{.}\mathtt{KeyGen}$), (ii) Encapsulation ($\mathtt{Kyber}{.}\mathtt{KEM}{.}\mathtt{Enc}$), and (iii) Decapsulation ($\mathtt{Kyber}{.}\mathtt{KEM}{.}\mathtt{Dec}$), which are represented in \autoref{fig:saberkem}. The Kyber KEM is also constructed by the help of CPA secure PKE (shown in \autoref{fig:kyberpke}) together with the post-quantum version of the FO transformation proposed in \cite{Jiang2017} to attain the CCA security. 

Three security versions of Kyber named Kyber512, Kyber768, and Kyber1024, depending on different values of the parameter set, and has presented in Table~\ref{tab:Parameters_kyber}. The parameter set of Kyber contains prime modulus $q$ and two power-of-two moduli $p$ and $t$, which form the rings $R_q, R_p, R_t$. In $\mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{Enc}$ (line $10$ and $11$ ), the $\mathtt{Compress}$ function shorten the ciphertext bits and maps each element of $R_q$ to $R_p$ or $R_t$. In this part, similar to Saber, Kyber uses the LWR problem. Conversely, the $\mathtt{Decompress}$ function in $\mathtt{Kyber}{.}\mathtt{PKE}{.}\mathtt{Dec}$ (line $1$ and $2$ ), extend the ciphertext bits and maps each element of $R_p$ or $R_t$ to $R_q$. The $\mathtt{Encode}: \{0, 1\}^{n} \rightarrow R_q$ function converts $n$-bit message to a polynomial in $R_q$, and the $\mathtt{Decode}: R_q \rightarrow \{0, 1\}^{n} $ function reverse the effect of the $\mathtt{Encode}$ function. Algorithmic details of the aforementioned four functions are shown in \autoref{fig:kyberfunc}. Each version of Kyber uses two CBD distributions $\beta_{\eta_1}$ and $\beta_{\eta_2}$ to sample secret and error vector. The three hash functions $\mathcal{G}, \mathcal{H}$, and $\mathtt{KDF}$ of Kyber KEM, are the same as Saber. Kyber uses number-theoretic transformations to perform polynomial multiplication. Here, we brief the Kyber scheme and recommend \cite{Kyber-Kem} for additional details.

\input{images/functionKyberPKE}
\input{images/kyberPKE}
% \input{images/kyberKEM}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\scriptsize
\caption{Parameters of Kyber with security and failure probability ~\cite{Saber_kem}}
\label{tab:Parameters_kyber}
\resizebox{0.90\textwidth}{!}{%
\begin{tabular}{|ll|ccccccc|c|c|c|}
\hline
\multicolumn{1}{|c}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Scheme\\ Name\end{tabular}}} & \multirow{3}{*}{} & \multicolumn{7}{c|}{Parameters}                                                                                                                                                                                                                                                                   & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Post-quantum\\ Security\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Failure \\ Probability\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}NIST\\ Security \\ Level\end{tabular}} \\ \cline{3-9}
\multicolumn{1}{|c}{}                                                                       &                   & \multicolumn{1}{c|}{\multirow{2}{*}{l}} & \multicolumn{1}{c|}{\multirow{2}{*}{n}}   & \multicolumn{1}{c|}{\multirow{2}{*}{q}}    & \multicolumn{1}{c|}{\multirow{2}{*}{p}} & \multicolumn{1}{c|}{\multirow{2}{*}{t}} & \multicolumn{1}{c|}{\multirow{2}{*}{$\eta_1$}} & \multirow{2}{*}{$\eta_2$} &                                                                                  &                                                                                 &                                                                                   \\
\multicolumn{1}{|c}{}                                                                       &                   & \multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{}                          &                           &                                                                                  &                                                                                 &                                                                                   \\ \hline
                                                                                            &                   & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                     & \multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                   & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{}     & \multicolumn{1}{l|}{}                                                            & \multicolumn{1}{l|}{}                                                           & \multicolumn{1}{l|}{}                                                             \\
Kyber512                                                                                    &                   & \multicolumn{1}{c|}{2}                  & \multicolumn{1}{c|}{\multirow{3}{*}{256}} & \multicolumn{1}{c|}{\multirow{3}{*}{3329}} & \multicolumn{1}{c|}{$2^{10}$}           & \multicolumn{1}{c|}{$2^{4}$}            & \multicolumn{1}{c|}{3}                         & 2                         & $2^{107}$                                                                        & $2^{-139}$                                                                      & 1                                                                                 \\
Kyber768                                                                                    &                   & \multicolumn{1}{c|}{3}                  & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{$2^{10}$}           & \multicolumn{1}{c|}{$2^{4}$}            & \multicolumn{1}{c|}{2}                         & 2                         & $2^{165}$                                                                        & $2^{-164}$                                                                      & 3                                                                                 \\
Kyber1024                                                                                   &                   & \multicolumn{1}{c|}{4}                  & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{$2^{11}$}           & \multicolumn{1}{c|}{$2^{5}$}            & \multicolumn{1}{c|}{2}                         & 2                         & $2^{232}$                                                                        & $2^{-174}$                                                                      & 5                                                                                 \\ \hline
\end{tabular}%
}
\end{table}


\subsection{Masking Saber and Kyber}\label{subsec:masked-saber}

There exist quite effective power and electromagnetic side-channel attacks (SCA)~\cite{DBLP:conf/latincrypt/PesslP19,DBLP:journals/tches/KannwischerPP20,DBLP:journals/iacr/MujdeiBBKWV22,DBLP:journals/tches/RaviRCB20} on the schemes in the NIST standardization procedure including Saber and Kyber. Most of these attacks target the decapsulation algorithm of the KEM. In a CCA-secure KEM the secret key is non-ephemeral. It is used to decrypt ciphertexts from many different entities. Therefore, it gives an attacker an opportunity to increase the success rate of its attack by observing multiple traces with different inputs or applying the fault in different places. Although, there exist instances of mounting physical attacks on key-generation and the encapsulation algorithm also to retrieve the secret key ($\pmb{s}$) and/or session-key ($K$) respectively \cite{DBLP:conf/cosade/RaviRBCM19,DBLP:conf/hipeac/ValenciaOGR18}. However, the challenge here is that an attacker can only execute these two algorithms once. In this work, we also target the masked decapsulation procedure of an LWE-based KEM. Therefore for ease of understanding, we briefly describe the first-order masked decapsulation algorithm below which can prevent first-order SCA.

%The implementation of this masked algorithm can prevent first-order SCA. 

The decapsulation of a general LWE-based KEM follows three steps: (i) decryption, (ii) re-encryption, and (iii) ciphertext comparison. The decryption part of the algorithm decodes the received ciphertext and computes the message. The re-encryption takes the message and encrypts it to reproduce the ciphertext. The ciphertext comparison step checks whether the received ciphertext and the newly created ciphertext are identical. If those two ciphertexts are the same, the algorithm outputs a valid message, and it concludes that the decryption is successful. Otherwise, the algorithm outputs a random message signaling a decryption failure. While applying the masking technique to protect the decapsulation algorithm, we must mask each of the three steps. Incorporating the masking technique increases the performance cost, so each of the three modules of the decapsulation algorithm is masked as efficiently as possible. 

LWE-based KEMs primarily utilize linear polynomial arithmetic operations over a ring $R\_q$, such as ring multiplication with one masked and another unmasked input, ring addition, and ring subtraction. These operations are duplicated and performed on each share independently in masked settings. For masking them, arithmetic masking techniques are used. The decapsulation also has non-linear arithmetic over $R\_q$. Those are shift operations on polynomials, and hash functions $\mathcal{H}, \mathcal{G}$, the extension function used for sampling pseudorandom numbers $\mathtt{XOF}$, the CBD $\beta_\mu$, ciphertext equality checking operation $=?$. These operations are expressed in bit operations and masked with Boolean masking. Except for these operations, the masked decapsulation needs two share conversions algorithms arithmetic to Boolean (\texttt{A2B}) and Boolean to arithmetic (\texttt{B2A}) conversions. The \texttt{B2A} conversion occurs inside the masked CBD ($\beta_\mu$). In first-order masking, the sensitive variable $x$ is split into two shares, $x_1$, and $x_2$. For arithmetic masking, the relation between $x$ and $(x_1,\ x_2)$ is $x_1 + x_2 = x \bmod{q}$. The relation between $x$ and $(x_1,\ x_2)$ in the case of Boolean masking is $x_1 \xor x_2 = x$. 

In Saber's decapsulation operation, the ring is $R\_p$ instead of $R\_q$. A pictorial version of this masked decapsulation operation of Saber is presented in \autoref{fig:sabermaskeddecaps}. In this work, we will focus on the part surrounded by the red rectangle in the figure, which includes the \texttt{A2B} conversion and shift operations. A version of \texttt{A2B} conversion used in Saber is shown in Algorithm \ref{algo:A2B}.

%\input{images/saberunmasked}
\input{images/sabermasked}

\begin{algorithm}[!ht]
\caption{ Secure Arithmetic to Boolean conversion (\texttt{A2B})~\cite{Coron2014_A2B} }
\label{algo:A2B}

\Input{$(a_1, a_2)\in \mathbb{R}_q \times \mathbb{R}_q$ such that $ a_1 + a_2= {x} \in \mathbb{R}_q $  and $k$ where $\mathbb{R}_q = \mathbb{R}_2^k$}
\Output{$(b_1, b_2)\in \mathbb{R}_q = \mathbb{R}_2^k$ such that $b_1 \xor b_2 = x$}
\BlankLine
$u_1\leftarrow \mathcal{U}(\mathbb{R}_2^k)$;    $u_2 = u_1 \xor a_1$ \\
$v_1\leftarrow \mathcal{U}(\mathbb{R}_2^k)$;    $v_2 = v_1 \xor a_2$ \\
$(b_1, b_2) = \mathtt{SecAdd} ((u_1, u_2), (v_1, v_2), k)$\\
\algorithmicreturn {$(b_1, b_2)$}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{ SecAdd~\cite{Coron2014_A2B} }
\label{algo:SecAdd}

\Input{$(x_1,\ x_2), (y_1,\ y_2)\in \mathbb{R}_2^k \times \mathbb{R}_2^k$ such that $ x_1 \xor x_2 = x$ and $ y_1 \xor y_2 = y$}
\Output{$(z_1,\ z_2)\in \mathbb{R}_2^k \times \mathbb{R}_2^k$ such that $ z_1 \xor z_2 = x+y \bmod{2^k}$}
\BlankLine
$(c_1^1,\ c_2^1) = (0,\ 0)$\\
$r_0,\ r_1,\ r_2 \leftarrow \mathcal{U}(\mathbb{R}_2^k)$\\
\For{\texttt{i=1 to k-1 }}
{
    $tmp1_1 = (x_1^i \& y_1^i) \xor r_0^i$;    $tmp1_2 = (x_2^i \& y_2^i) \xor r_0^i$\\
    $tmp2_1 = (x_1^i \& c_1^i) \xor r_1^i$;    $tmp2_2 = (x_2^i \& c_2^i) \xor r_1^i$\\
    $tmp3_1 = (y_1^i \& c_1^i) \xor r_2^i$;    $tmp3_2 = (y_2^i \& c_2^i) \xor r_2^i$\\
    $c_1^{i+1} = tmp1_1 \xor tmp2_1 \xor tmp3_1$\\    $c_2^{i+1} = tmp1_2 \xor tmp2_2 \xor tmp3_2$\\
}
$z_1 = x_1 \xor y_1 \xor c_1$;    $z_2 = x_2 \xor y_2 \xor c_2$\\
\algorithmicreturn{ $(z_1,\ z_2)$}
\end{algorithm}

In Kyber, the ring modulus $q$ is prime, the share conversion algorithms \texttt{A2B} (\texttt{A2B}$_q$) and \texttt{B2A} (\texttt{B2A}$_q$) are different compared to Saber, which uses power-of-two modulus. In Kyber, the shares are first transferred from prime to a power-of-two modulus, and an aforementioned \texttt{A2B} conversion (Algorithm \ref{algo:A2B}) or a \texttt{B2A} conversion algorithm with input in power-of-two modulus is performed. For this reason, a couple of extra masking modules, such as $\mathtt{Decode}$, $\mathtt{Encode}$, $\mathtt{Compress}$, and \texttt{transform-power-of-2} are required in masked Kyber. In Kyber, the \texttt{A2B} conversions are used in $\mathtt{Decode}$ and $\mathtt{Comp}$ components, and the \texttt{B2A} conversions are inside the $\mathtt{Encode}$. \autoref{fig:kybermaskeddecaps} is an illustrated version of the first-order masked decapsulation algorithm of Kyber. The function we exploit in this work is the $\mathtt{Decode}$, which is surrounded by the red rectangle in the figure. Below we give brief details regarding the masked $\mathtt{Decode}$ procedure in Algorithm \ref{algo:masked-decode}.   
\input{images/kybermasked}

\begin{algorithm}[!ht]
\caption{ Masked decode algorithm~\cite{1st-order_masked_comparator} }
\label{algo:masked-decode}

\Input{$(m''_1,\ m''_2)\in \mathbb{R}_q \times \mathbb{R}_q$}
\Output{$(m'_1,\ m'_2)\in \mathbb{R}_2$ such that $m'_1 \xor m'_2 = \mathtt{Decode}(m''_1 + m''_2 \bmod{q})$}
\BlankLine
$m''_1 = m''_1 - \lfloor q/4 \rfloor$ \\
\tcc{\text{transfers arithmetic shares from }$\bmod{q}$\text{ to }$\bmod{2^{13}}$}
$(c_1,\ c_2) = \texttt{transform-power-of-2}(m''_1,\ m''_2,\ 13)$ \\
$c_1 = c_1 - \lfloor q/2 \rfloor$ \\
$(d_1,\ d_2) = \texttt{A2B} ((c_1,\ c_2),\ 13)$\\
$m'_1 = d_1^{13};\  m'_2 = d_2^{13}$\\
\algorithmicreturn {$(m'_1,\ m'_2)$}
\end{algorithm}

\subsection{Previous fault attacks on LWE based KEM}

The key generation and the encapsulation algorithm of LWE-based KEMs are also attacked by using fault, as shown in recent works \cite{DBLP:conf/cosade/RaviRBCM19,DBLP:conf/hipeac/ValenciaOGR18}. However, the decapsulation algorithm is especially exploitable to fault attacks as in most of the applications of KEM, the same secret key is used in the decapsulation module for a significant amount of time. Any LWE-based KEM uses a version of FO transformation \cite{Jiang2017} to achieve CCA security. The decapsulation operation includes decryption and re-encryption and only returns a session key if the given ciphertext and re-encrypted ciphertext are the same, else returns a random key. These steps of FO transformation naturally resist differential fault attacks \cite{1st-order_masked_comparator}, which can break block ciphers like advanced encryption standard (AES) \cite{DBLP:conf/wistp/TunstallMA11}. Though, a fault to bypass the equality check of the public ciphertext and re-encrypted ciphertext and consistently delivering the valid session key can remove the CCA security of the KEM scheme. Another kind of fault attack is the ineffective fault attack, and FO transformation can not prevent this kind of fault attack. Several works \cite{DBLP:conf/fdtc/BettaleMR21,PesslP21,HermelinkPP21,Delvaux22} are presented in the category of ineffective fault attacks on LWE-based KEM schemes while utilizing different attack strategies.  In \cite{PesslP21}, Pessl et al. used an instruction skip fault in the $\mathtt{Decode}$ part of the decapsulation of Kyber and then observed if this fault resulted in the correct session key or not. If, after the fault, the decapsulation returns the correct session key, then the fault is ineffective. Otherwise, the introduced fault cause decryption failure, and that means the fault is effective. The effectiveness of the fault depends on the decryption noise, and the decryption noise linearly depends on the long-term secret key $\pmb{s}$. Each decryption failure or success provides an inequality with the unknown variable $\pmb{s}$. After repeating this process, the attacker can accumulate a sufficient number of such inequalities and retrieve $\pmb{s}$ by solving the set of inequalities. The attack proposed in \cite{HermelinkPP21} is similar to \cite{PesslP21} but use different position to inject fault, also belongs to in the category of ineffective fault attack. Later, Jeroen Delvaux extended the fault locations of \cite{HermelinkPP21} and improved the inequality solver in \cite{Delvaux22}. We also use ineffective fault attack techniques in this work, and our attack is related to the articles mentioned in this section.


==> old_sections/performance.tex <==
\section{Performance evaluation}

To demonstrate the performance of all of the proposed methods, we implement them on a 32-bit ARM Cortex-M4 microcontroller, STM32F407-DISCOVERY development board. We adopt the widely used PQM4~\cite{PQM4} post-quantum cryptographic library and benchmarking framework for performance evaluation. In this framework, the system timer (SisTick) is used to measure the cycle counts. This framework uses a 24MHz main system clock and a 48MHz TRNG clock. We take advantage of the on-chip TRNG for sampling masking randomness instead of generating in advance and storing random bits in a table like Kyber~\cite{ho-mask-comparator-kyber-bos-2021}. This TRNG generates 32 random bits per 40 TRNG clock cycles, which is equal to 20 main system clock cycles. We include the cost of randomness sampling with the benchmarks. We use \texttt{arm-none-eabi-gcc} version \texttt{9.2.1} to accomplish the measurements of our implementations. 

\subsection{Performance analysis of comparison algorithms for Saber}

We present the cycle counts of the implementation for arbitrary order masked comparison algorithms of Saber. In Saber, the parameters are: $\epsilon_q=13$, $\epsilon_p=10$, $\epsilon_t=4$ and $l=3$. We break down the cycle counts into three parts: spent during all the \texttt{A2B} conversion, spent in computing the function \texttt{BooleanAllBitsOneTest} for the corresponding parameter, and spent in performing all other operations. Table~\ref{tab:Compararator} contains the performance details of masked ciphertext algorithms presented in Sections~\ref{subsubsec:decompressed_masked_comparison} and Sections~\ref{subsubsec:new_masked_comparison}. 

%Improvement
In Table~\ref{tab:Compararator}, we include two versions of the decompressed comparison algorithm and the simple comparison algorithm. We use the bitsliced \texttt{A2B} conversion technique of masked simple comparator proposed in~\cite{D'AnversVV22} for the first version, and we improve this bitsliced \texttt{A2B} converter by employing the technique introduced in~\cite{BronchainC22}. It can be seen from the table the performance of the decompressed comparison algorithm gains 9\%, 16\%, and 17\% improvements for first-, second-, and third-order masking after using~\cite{BronchainC22}, respectively. Side by side, the improved decompressed comparison algorithm requires 21\% fewer random bytes for any order masking. The performance of the simple comparison algorithm improves by 9\%, 15\%, and 16\% for first-, second-, and third-order masking after using~\cite{BronchainC22}, respectively. The improved simple comparison algorithm requires approximately 19\% fewer random bytes for any order masking.   

 As we can see from the table, the cycle count for all \texttt{A2B} conversions employed in the decompressed comparison algorithm is almost double for all orders compared to the simple comparison algorithm. However, for all the orders, the clock cycle required to compute the function \texttt{BooleanAllBitsOneTest} with corresponding parameters is approximately one-fourth in the decompressed comparison algorithm than the simple comparison algorithm. As we can see from Table~\ref{tab:Compararator}, the improved simple comparison algorithm is approximately $45\%$ faster and employ roughly 42\% fewer random bytes than the improved decompressed comparison algorithm for any order masking of Saber. Similar results can be found for the higher-order masked uSaber. So, we use the improved simple comparison algorithm in our higher-order masked Saber and uSaber decapsulation algorithms.   


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\centering
\caption{Performance breakdown of the implementation of masked comparison algorithms in the Cortex-M4 platform.}
\label{tab:Compararator}
\begin{tabular}{lllllrlrrrr}
\hline
                         &                       & \multicolumn{1}{c}{}                                    &  &  & \multicolumn{6}{c}{CPU [k]cycles}                                                                                                                                                                                                           \\ \cline{4-11} 
                         &                       & \multicolumn{1}{c}{\multirow{-2}{*}{Masked Comparator}} &  &  & \multicolumn{2}{c}{1st}                                                           & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{2nd}                 & \multicolumn{1}{c}{}             & \multicolumn{1}{c}{3rd}                 \\ \hline
\multicolumn{3}{l}{\textbf{Decompressed comparison} [This work]}                                           &  &  & \multicolumn{2}{r}{649}                                                           & \textbf{}                        & 2,101                                   & \textbf{}                        & 3,594                                   \\
                         & \multicolumn{1}{l|}{} & all \texttt{A2B} conversion                             &  &  & \multicolumn{2}{r}{612}                                                           &                                  & 2,047                                   &                                  & 3,519                                   \\
                         & \multicolumn{1}{l|}{} & \texttt{BooleanAllBitsOneTest}                          &  &  & \multicolumn{2}{r}{7}                                                             &                                  & 22                                      &                                  & 38                                      \\
                         & \multicolumn{1}{l|}{} & Other operations                                        &  &  & \multicolumn{2}{r}{28}                                                            &                                  & 31                                      &                                  & 36                                      \\
\rowcolor[HTML]{EFEFEF} 
                         & \multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}\# random bytes}                     &  &  & \multicolumn{2}{r}{\cellcolor[HTML]{EFEFEF}11,984}                                &                                  & 47,728                                  &                                  & 95,456                                  \\ \hline
\multicolumn{3}{l}{\textbf{Improved decompressed comparison} [This work]}                                  &  &  & \multicolumn{2}{r}{{\color[HTML]{000000} \textbf{586}}}                           & {\color[HTML]{000000} \textbf{}} & {\color[HTML]{000000} \textbf{1,750}}   & {\color[HTML]{000000} \textbf{}} & {\color[HTML]{000000} \textbf{2,950}}   \\
                         & \multicolumn{1}{l|}{} & all \texttt{A2B} conversion                             &  &  & \multicolumn{2}{r}{549}                                                           &                                  & 1,696                                   &                                  & 2,875                                   \\
                         & \multicolumn{1}{l|}{} & \texttt{BooleanAllBitsOneTest}                          &  &  & \multicolumn{2}{r}{7}                                                             &                                  & 22                                      &                                  & 38                                      \\
                         & \multicolumn{1}{l|}{} & Other operations                                        &  &  & \multicolumn{2}{r}{28}                                                            &                                  & 31                                      &                                  & 36                                      \\
\rowcolor[HTML]{EFEFEF} 
                         & \multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}\# random bytes}                     &  &  & \multicolumn{2}{r}{\cellcolor[HTML]{EFEFEF}\textbf{9,360}}                        &                                  & \cellcolor[HTML]{EFEFEF}\textbf{37,232} &                                  & \cellcolor[HTML]{EFEFEF}\textbf{74,464} \\ \hline
\multicolumn{3}{l}{\textbf{Simple comparison}~\cite{D'AnversVV22}}                                         &  &  & \multicolumn{2}{r}{352}                                                           & \multicolumn{1}{l}{}             & 1,126                                   & \multicolumn{1}{l}{}             & 1,934                                   \\
                         & \multicolumn{1}{l|}{} & all \texttt{A2B} conversion                             &  &  & \multicolumn{2}{r}{308}                                                           & \multicolumn{1}{l}{}             & 1,023                                   &                                  & 1,766                                   \\
                         & \multicolumn{1}{l|}{} & \texttt{BooleanAllBitsOneTest}                          &  &  & \multicolumn{2}{r}{27}                                                            & \multicolumn{1}{l}{}             & 83                                      &                                  & 143                                     \\
                         & \multicolumn{1}{l|}{} & Other operations                                        &  &  & \multicolumn{2}{r}{16}                                                            & \multicolumn{1}{l}{}             & 20                                      &                                  & 24                                      \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}\# random bytes}                     &  &  & \multicolumn{2}{r}{\cellcolor[HTML]{EFEFEF}6,672}                                 &                                  & 25,904                                  &                                  & 51,808                                  \\ \hline
\multicolumn{3}{l}{\textbf{Improved simple comparison} [This work]}                                        &  &  & \multicolumn{2}{r}{{\color[HTML]{3531FF} \textbf{320}}}                           & \multicolumn{1}{l}{}             & {\color[HTML]{3531FF} \textbf{951}}     & {\color[HTML]{3531FF} }          & {\color[HTML]{3531FF} \textbf{1,612}}   \\
                         & \multicolumn{1}{l|}{} & all \texttt{A2B} conversion                             &  &  & \multicolumn{2}{r}{276}                                                           & \multicolumn{1}{l}{}             & 848                                     &                                  & 1,444                                   \\
                         & \multicolumn{1}{l|}{} & \texttt{BooleanAllBitsOneTest}                          &  &  & \multicolumn{2}{r}{27}                                                            & \multicolumn{1}{l}{}             & 83                                      &                                  & 143                                     \\
                         & \multicolumn{1}{l|}{} & Other operations                                        &  &  & \multicolumn{2}{r}{16}                                                            & \multicolumn{1}{l}{}             & 20                                      &                                  & 24                                      \\
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \multicolumn{2}{l}{\cellcolor[HTML]{EFEFEF}\# random bytes}                     &  &  & \multicolumn{2}{r}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{3531FF} \textbf{5,360}}} & {\color[HTML]{3531FF} \textbf{}} & {\color[HTML]{3531FF} \textbf{20,656}}  & {\color[HTML]{3531FF} \textbf{}} & {\color[HTML]{3531FF} \textbf{41,312}}  \\ \hline
\end{tabular}
\end{table}


\subsection{Performance analysis for masked Saber decapsulation }

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\centering
\caption{Performance cost of all the modules of the higher-order masked decapsulation procedure of Saber.}
\label{tab:masked_saber_performance}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllrcrrlrrlrr}
\hline
                      &  & \multicolumn{5}{l}{}                                                         &  & \multicolumn{10}{c}{CPU [k]cycles}                                                                                                                                                                        \\ \cline{9-18} 
                      &  & \multicolumn{5}{c}{Order}                                                    &  & \multicolumn{1}{l|}{Unmask}               &  & \multicolumn{2}{c|}{1st}                               &  & \multicolumn{2}{c|}{2nd}                               &  & \multicolumn{2}{c}{3rd}           \\ \hline
\multicolumn{7}{l}{{\color[HTML]{3531FF} \textbf{Saber-Decapsulation}}}                                 &  & \multicolumn{1}{r|}{1,121}                 &  & 3,011 & \multicolumn{1}{r|}{(2.68x)}                   &  & 5,534 & \multicolumn{1}{r|}{(4.93x)}                   &  & 8,591 & (7.66x)                   \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{CPA-PKE-Decryption}}                              &  & \multicolumn{1}{r|}{129}                   &  & 297   & \multicolumn{1}{r|}{(2.30x)}                   &  & 527   & \multicolumn{1}{r|}{(4.08x)}                   &  & 775   & (6.00x)                   \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial arithmetic}         &  & \multicolumn{1}{r|}{126}                   &  & 237   & \multicolumn{1}{r|}{(1.88x)}                   &  & 349   & \multicolumn{1}{r|}{(2.76x)}                   &  & 464   & (3.68x)                   \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Compression}                   &  & \multicolumn{1}{r|}{2}                     &  & 59    & \multicolumn{1}{r|}{(29.50x)}                  &  & 178   & \multicolumn{1}{r|}{(89.00x)}                  &  & 310   & (155.00x)                 \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{Hash $\mathcal{G}$ (SHA3-512)}}                   &  & \multicolumn{1}{r|}{13}                    &  & 123   & \multicolumn{1}{r|}{(9.46x)}                   &  & 242   & \multicolumn{1}{r|}{(18.61x)}                  &  & 379   & (29.15x)                  \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{CPA-PKE-Encryption}}                              &  & \multicolumn{1}{r|}{853}                   &  & 2,466 & \multicolumn{1}{r|}{(2.89x)}                   &  & 4,636 & \multicolumn{1}{r|}{(5.43x)}                   &  & 7,311 & (8.57x)                   \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Secret generation}             &  & \multicolumn{1}{r|}{69}                    &  & 909   & \multicolumn{1}{r|}{(13.17x)}                  &  & 1,995 & \multicolumn{1}{r|}{(28.91x)}                  &  & 3,561 & (51.60x)                  \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & XOF (SHAKE-128)        &  & \multicolumn{1}{r|}{63}                    &  & 611   & \multicolumn{1}{r|}{(9.69x)}                   &  & 1,210 & \multicolumn{1}{r|}{(19.20x)}                  &  & 1,887 & (29.95x)                  \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & CBD (Binomial Sampler) &  & \multicolumn{1}{r|}{6}                     &  & 297   & \multicolumn{1}{r|}{(49.50x)}                  &  & 785   & \multicolumn{1}{r|}{(130.83x)}                 &  & 1,674 & (279.00x)                 \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial arithmetic}         &  & \multicolumn{1}{r|}{}                      &  & 1,235 & \multicolumn{1}{r|}{}                          &  & 1,688 & \multicolumn{1}{r|}{}                          &  & 2,136 &                           \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial Comparison}         &  & \multicolumn{1}{r|}{\multirow{-2}{*}{783}} &  & 320   & \multicolumn{1}{r|}{\multirow{-2}{*}{(1.98x)}} &  & 952   & \multicolumn{1}{r|}{\multirow{-2}{*}{(3.37x)}} &  & 1,612 & \multirow{-2}{*}{(4.78x)} \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{Other operations}                                         &  & \multicolumn{1}{r|}{126}                   &  & 126   & \multicolumn{1}{r|}{(1.00x)}                   &  & 126   & \multicolumn{1}{r|}{(1.00x)}                   &  & 126   & (1.00x)                   \\ \hline
\end{tabular}%
}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\centering
\caption{Randomness cost of all the modules of the higher-order masked decapsulation algorithm of Saber.}
\label{tab:masked_saber_randomness}
\begin{tabular}{llllllllrrrlrrlrr}
\hline
                      &  & \multicolumn{5}{l}{}                                                         &  & \multicolumn{9}{c}{\# Random bytes}                                                                                    \\ \cline{9-17} 
                      &  & \multicolumn{5}{c}{Order}                                                    &  & \multicolumn{1}{l}{} & \multicolumn{2}{c|}{1st}       &  & \multicolumn{2}{c|}{2nd}       &  & \multicolumn{2}{c}{3rd} \\ \hline
\multicolumn{7}{l}{{\color[HTML]{3531FF} \textbf{Saber-Decapsulation}}}                                 &  &                      & 12,432 & \multicolumn{1}{r|}{} &  & 42,800 & \multicolumn{1}{r|}{} &  & 91,744        &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{CPA-PKE-Decryption}}                              &  &                      & 928    & \multicolumn{1}{r|}{} &  & 3,712  & \multicolumn{1}{r|}{} &  & 7,424         &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial arithmetic}         &  &                      & 0      & \multicolumn{1}{r|}{} &  & 0      & \multicolumn{1}{r|}{} &  & 0             &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Compression}                   &  &                      & 928    & \multicolumn{1}{r|}{} &  & 3,712  & \multicolumn{1}{r|}{} &  & 7,424         &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{Hash $\mathcal{G}$ (SHA3-512)}}                   &  &                      & 192    & \multicolumn{1}{r|}{} &  & 576    & \multicolumn{1}{r|}{} &  & 1,152         &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{CPA-PKE-Encryption}}                              &  &                      & 11,312 & \multicolumn{1}{r|}{} &  & 38,512 & \multicolumn{1}{r|}{} &  & 83,168        &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Secret generation}             &  &                      & 5,952  & \multicolumn{1}{r|}{} &  & 17,856 & \multicolumn{1}{r|}{} &  & 41,856        &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & XOF (SHAKE-128)        &  &                      & 960    & \multicolumn{1}{r|}{} &  & 2880   & \multicolumn{1}{r|}{} &  & 5,760         &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & CBD (Binomial Sampler) &  &                      & 4,992  & \multicolumn{1}{r|}{} &  & 14,976 & \multicolumn{1}{r|}{} &  & 36,096        &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial arithmetic}         &  &                      & 0      & \multicolumn{1}{r|}{} &  & 0      & \multicolumn{1}{r|}{} &  & 0             &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial Comparison}         &  &                      & 5,360  & \multicolumn{1}{r|}{} &  & 20,656 & \multicolumn{1}{r|}{} &  & 41,312        &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{Other operations}                                         &  &                      & 0      & \multicolumn{1}{r|}{} &  & 0      & \multicolumn{1}{r|}{} &  & 0             &         \\ \hline
\end{tabular}
\end{table}

%The performance of the Saber's decapsulation algorithm also is obtained using the PQM4~\cite{PQM4} framework. 
We present the performance cost of the Saber algorithm for higher-order masking in Table~\ref{tab:masked_saber_performance}. This table also provides the breakdown of the performance cost of the higher-order masking for all the modules of the masked Saber decapsulation algorithm. As mentioned earlier, for masked Saber implementations we use the hybrid polynomial multiplication, a combination of Toom-Cook-4, Karatsuba, and schoolbooks multiplication. Therefore, we use the Saber implementation which uses the hybrid polynomial multiplication to get the overhead factor for $n$-th order masked Saber. To maintain simplicity, most of the implementation is written in C. Only the hybrid multiplication is in assembly and generated by using the optimal implementation proposed in~\cite{polymul-z2mx-m4}. 

From Table~\ref{tab:masked_saber_performance}, we can see that the performance overhead factor of masked Saber decapsulation implementation for first-order is $2.68$x, for second-order is $4.93$x, and for third-order is $7.66$x. From the table, we can see that the overhead factor for arithmetic operations approximately is $(n+1)$ for $n$th-order masking due to $n+1$ time repetitions of each operation. On the other hand, the non-linear operations on arithmetic shares, for example, hash functions, binomial sampler, compression operation, and ciphertext comparison, have much larger overhead factors in the masked setting. To maintain the security assumption, we need to use random bytes in some masking algorithms (example: SecAnd, SecAdd, SecRefresh, etc). Table~\ref{tab:masked_saber_randomness} shows random bytes requirements for all the components of the higher-order masked Saber decapsulation algorithm. It can be seen from Table~\ref{tab:masked_saber_randomness} that the random bytes requirement increases with the order. The first-order implementation requires $12$k random bytes, the second-order and third-order implementations require $43$k ($3.44$x) and $92$k ($7.37$x) random bytes, respectively.    


\subsection{Performance analysis for masked uSaber decapsulation }

The performance cost and breakdown of the performance cost of the higher-order masking for all the modules of the masked uSaber decapsulation algorithm are presented in Table~\ref{tab:masked_usaber_performance}. As we mentioned before, the main advantage of uSaber against Saber is the coefficients of the secret vector are sampled from $\mathcal{U}_2$ instead of $\beta_8$. Thanks to the parameter choice of secret distribution in uSaber, it needs fewer numbers of pseudorandom bits than Saber. This fact reduces the cycle cost of \texttt{XOF} by almost $60\%$ for the unmasked version of uSaber compared to Saber. Another advantage is that the hamming weight computation of $\mu$ bits in the centered binomial sampler $\beta_\mu$ is swapped by the sign extension of $u$ bits in the centered uniform sampler $\mathcal{U}_u$. It reduces the performance cost of the secret sampler in unmasked uSaber by $50\%$ compared to Saber. Altogether, the secret generation is almost $59\%$ faster for the unmasked decapsulation algorithm of uSaber compared to Saber. The performance cost of the secret generation is lower in uSaber compared to Saber also after integrating masking. The performances of the secret generation in masked uSaber are $55\%$, $52\%$, and $45\%$ faster compared to masked Saber for first-, second-, and third-order, respectively. Additionally, the value of $q$ for uSaber is $2^{12}$, whereas it is $2^{13}$ for Saber. This factor reduces one bit in the \texttt{A2B} conversion for uSaber during the masked polynomial comparison. It makes the masked polynomial comparison $5\%$, $5\%$, and $2\%$ faster in uSaber than Saber for first-, second-, and third-order, respectively.

As we can observe from Table~\ref{tab:masked_usaber_performance}, the approximate performance overhead factor of masked uSaber decapsulation implementation for first-order is $2.31$x, for second-order is $4.16$x, and for third-order is $6.48$x. Table~\ref{tab:masked_usaber_randomness} presents random bytes requirements for all the segments of the higher-order masked uSaber decapsulation. We obtain from Table~\ref{tab:masked_usaber_randomness} that here also the random bytes requirement grows with the order of masking. The first-order implementation needs $10$k random bytes, the second-order and third-order implementations use $36$k ($3.51$x) and $78$k ($7.62$x) random bytes, respectively. 


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\centering
\caption{Performance cost of all the modules of higher-order masked decapsulation procedure of uSaber.}
\label{tab:masked_usaber_performance}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllrrrrrrrrrr}
\hline
                      &  & \multicolumn{5}{l}{}                                                       &  & \multicolumn{10}{c}{CPU [k]cycles}                                                                                                                                                                                                                                    \\ \cline{9-18} 
                      &  & \multicolumn{5}{c}{Order}                                                  &  & \multicolumn{1}{c|}{Unmask}               & \multicolumn{3}{c|}{1st}                                                      & \multicolumn{3}{c|}{2nd}                                                      & \multicolumn{3}{c}{3rd}                                  \\ \hline
\multicolumn{7}{l}{{\color[HTML]{3531FF} \textbf{uSaber-Decapsulation}}}                              &  & \multicolumn{1}{r|}{1,062}                 &                      & 2,462 & \multicolumn{1}{r|}{(2.31x)}                   &                      & 4,419 & \multicolumn{1}{r|}{(4.16x)}                   &                      & 6,888 & (6.48x)                   \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{CPA-PKE-Decryption}}                            &  & \multicolumn{1}{r|}{130}                   &                      & 297   & \multicolumn{1}{r|}{(2.28x)}                   &                      & 527   & \multicolumn{1}{r|}{(4.05x)}                   &                      & 775   & (5.96x)                   \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial arithmetic}       &  & \multicolumn{1}{r|}{128}                   &                      & 237   & \multicolumn{1}{r|}{(1.85x)}                   &                      & 349   & \multicolumn{1}{r|}{(2.72x)}                   &                      & 464   & (3.62x)                   \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Compression}                 &  & \multicolumn{1}{r|}{2}                     &                      & 59    & \multicolumn{1}{r|}{(29.50x)}                  &                      & 178   & \multicolumn{1}{r|}{(89.00x)}                  &                      & 310   & (155.00x)                 \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{Hash $\mathcal{G}$ (SHA3-512)}}                 &  & \multicolumn{1}{r|}{13}                    &                      & 122   & \multicolumn{1}{r|}{(9.38x)}                   &                      & 242   & \multicolumn{1}{r|}{(18.61x)}                  &                      & 379   & (29.15x)                  \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{CPA-PKE-Encryption}}                            &  & \multicolumn{1}{r|}{791}                   &                      & 1,917 & \multicolumn{1}{r|}{(2.42x)}                   &                      & 3,522 & \multicolumn{1}{r|}{(4.45x)}                   &                      & 5,608 & (7.08x)                   \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Secret generation}           &  & \multicolumn{1}{r|}{28}                    &                      & 400   & \multicolumn{1}{r|}{(14.28x)}                  &                      & 954   & \multicolumn{1}{r|}{(34.07x)}                  &                      & 1,928 & (68.85x)                  \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & XOF (SHAKE-128)      &  & \multicolumn{1}{r|}{25}                    &                      & 245   & \multicolumn{1}{r|}{(9.80x)}                   &                      & 484   & \multicolumn{1}{r|}{(19.36x)}                  &                      & 756   & (30.24x)                  \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & Uniform distribution &  & \multicolumn{1}{r|}{3}                     &                      & 155   & \multicolumn{1}{r|}{(51.66x)}                  &                      & 469   & \multicolumn{1}{r|}{(156.33x)}                 &                      & 1,172 & (390.66x)                 \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial arithmetic}       &  & \multicolumn{1}{r|}{}                      &                      & 1,214 & \multicolumn{1}{r|}{}                          &                      & 1,667 & \multicolumn{1}{r|}{}                          &                      & 2,114 &                           \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial Comparison}       &  & \multicolumn{1}{r|}{\multirow{-2}{*}{763}} & \multicolumn{1}{c}{} & 302   & \multicolumn{1}{r|}{\multirow{-2}{*}{(1.98x)}} & \multicolumn{1}{l}{} & 900   & \multicolumn{1}{r|}{\multirow{-2}{*}{(3.36x)}} & \multicolumn{1}{l}{} & 1,564 & \multirow{-2}{*}{(4.82x)} \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{Other operations}                                       &  & \multicolumn{1}{r|}{126}                   &                      & 126   & \multicolumn{1}{r|}{(1.00x)}                   &                      & 126   & \multicolumn{1}{r|}{(1.00x)}                   &                      & 126   & (1.00x)                   \\ \hline
\end{tabular}%
}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\centering
\caption{Randomness cost of all the modules of higher-order masked decapsulation algorithm of uSaber.}
\label{tab:masked_usaber_randomness}
\begin{tabular}{llllllllrrrlrrlrr}
\hline
                      &  & \multicolumn{5}{l}{}                                                       &  & \multicolumn{9}{c}{\# Random bytes}                                                                                    \\ \cline{9-17} 
                      &  & \multicolumn{5}{c}{Order}                                                  &  & \multicolumn{1}{l}{} & \multicolumn{2}{c|}{1st}       &  & \multicolumn{2}{c|}{2nd}       &  & \multicolumn{2}{c}{3rd} \\ \hline
\multicolumn{7}{l}{{\color[HTML]{3531FF} \textbf{uSaber-Decapsulation}}}                              &  &                      & 10,224 & \multicolumn{1}{r|}{} &  & 35,888 & \multicolumn{1}{r|}{} &  & 77,920        &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{CPA-PKE-Decryption}}                            &  &                      & 928    & \multicolumn{1}{r|}{} &  & 3,712  & \multicolumn{1}{r|}{} &  & 7,424         &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial arithmetic}       &  &                      & 0      & \multicolumn{1}{r|}{} &  & 0      & \multicolumn{1}{r|}{} &  & 0             &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Compression}                 &  &                      & 928    & \multicolumn{1}{r|}{} &  & 3,712  & \multicolumn{1}{r|}{} &  & 7,424         &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{Hash $\mathcal{G}$ (SHA3-512)}}                 &  &                      & 192    & \multicolumn{1}{r|}{} &  & 576    & \multicolumn{1}{r|}{} &  & 1,152         &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{\textbf{CPA-PKE-Encryption}}                            &  &                      & 9,104  & \multicolumn{1}{r|}{} &  & 31,600 & \multicolumn{1}{r|}{} &  & 69,344        &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Secret generation}           &  &                      & 4,032  & \multicolumn{1}{r|}{} &  & 12,096 & \multicolumn{1}{r|}{} &  & 30,336        &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & XOF (SHAKE-128)      &  &                      & 960    & \multicolumn{1}{r|}{} &  & 2880   & \multicolumn{1}{r|}{} &  & 5,760         &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & Uniform distribution &  &                      & 3,072  & \multicolumn{1}{r|}{} &  & 9,216  & \multicolumn{1}{r|}{} &  & 24,576        &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial arithmetic}       &  &                      & 0      & \multicolumn{1}{r|}{} &  & 0      & \multicolumn{1}{r|}{} &  & 0             &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{} &  & \multicolumn{3}{l}{Polynomial Comparison}       &  &                      & 5,072  & \multicolumn{1}{r|}{} &  & 19,504 & \multicolumn{1}{r|}{} &  & 39,008        &         \\
\multicolumn{1}{l|}{} &  & \multicolumn{5}{l}{Other operations}                                       &  &                      & 0      & \multicolumn{1}{r|}{} &  & 0      & \multicolumn{1}{r|}{} &  & 0             &         \\ \hline
\end{tabular}
\end{table}

\subsection{Comparison with state-of-the-art}

In this section, we compare our masked Saber and uSaber implementations with the state-of-the-art masked implementations of Saber and Kyber. We present the performances of our masked implementations in the Cortex-M4 platform and present them in Table~\ref{tab:performance_comp}. Bronchain et al.~\cite{BronchainC22} introduced faster implementations of higher-order masked \texttt{A2B} and \texttt{B2A} conversion utilizing bitsliced techniques and used these conversions to propose higher-order masking implementations of Saber and Kyber. The performances of Bronchain et al.'s masked Saber and Kyber implementations in the Cortex-M4 platform are presented in Table~\ref{tab:performance_comp}. As we mentioned before, the integration of NTT multiplication in masked Saber can provide a significant performance boost. In~\cite{BronchainC22}, authors use NTT multiplication for Saber to receive better performance. In order to use NTT multiplication, the authors use a multi-moduli approach that extends the modulus \cite{DBLP:journals/tches/AbdulrahmanCCHK22}. Even so, the performance of our 1st, 2nd and 3rd order masked implementations of Saber achieve 40\%, 24\%, and 13\% improvement than their masked implementation of Saber, respectively. 

In~\cite{ho-mask-comparator-kyber-bos-2021}, Bos et al. proposed higher-order masked implementations of Kyber. The masked kyber implementation in~\cite{ho-mask-comparator-kyber-bos-2021} is faster and uses fewer random bytes than the implementation of masked kyber presented in~\cite{BronchainC22} only for first-order because this masked Kyber uses an optimized implementation for first-order, while Bronchain et al.'s one uses the generalized one. The performance for 2nd and 3rd order masked implementations of Kyber in~\cite{BronchainC22} receives 73\% and 85\% improvement over the masked Kyber of~\cite{ho-mask-comparator-kyber-bos-2021}, respectively. However, our implementation of masked Saber is faster than masked Kyber presented in~\cite{BronchainC22} 60\% for first-order, 53\% for second-order, and 48\% for third-order. Also, the performance of our first-order masked Saber is 3\% faster than the optimized implementation of the first-order masked Kyber presented in~\cite{ho-mask-comparator-kyber-bos-2021}. In terms of random bytes requirement, our masked Saber receives factor 21.07x and 26.53x improvement over the masked Kyber in~\cite{ho-mask-comparator-kyber-bos-2021} for 2nd and 3rd order masked implementations, respectively.  

As discussed in Section~\ref{sec:masking_usaber}, masked uSaber uses less number of operations and random numbers than masked Saber due to the choice of secret distribution and parameters in uSaber.  Table~\ref{tab:performance_comp} shows the performances of higher-order masked implementations of uSaber. Further, this table contains the performance of first-order masked Saber~\cite{FO-masked-saber} and first-order masked Kyber~\cite{FO-masked-kyber-HeinzKLPSS22}, which are specially optimized to prevent the first-order differential power attacks. We can observe from Table~\ref{tab:performance_comp} that our generalized implementation of first-order masked uSaber is 13\% faster than the optimized implementation of masked Saber and is 17\% faster than the optimized implementation of masked Kyber. The implementation of masked uSaber is faster than the fastest implementation of higher-order masked Saber 20\% for second-order and 19\% for third-order. Masked uSaber also needs 16\% less random numbers for second-order and 15\% less random numbers for third-order over masked Saber. In conclusion, we observe from the reported results of Table~\ref{tab:performance_comp} that higher-order masked uSaber achieves better performance and needs fewer random bytes than masked Saber and Kyber for any order. 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\caption{The comparison between Saber and Kyber regarding the performance and the random bytes requirement.}
\label{tab:performance_comp}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cllccccccccccccc|cccccccll}
\hline
\multicolumn{3}{c}{}                                                                                                      &                      &                      & \multicolumn{11}{c|}{Performance CPU [k]cycles}                                                           & \multicolumn{9}{c}{\# Random bytes}                                                                                                                    \\ \cline{5-25} 
\multicolumn{3}{c}{\multirow{-2}{*}{Scheme}}                                                                              &                      &                      & Unmask &  & 1st            &  &  & 2nd            &           &           & 3rd            &           &  & 1st             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 2nd             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 3rd             &  &  \\ \hline
\multicolumn{1}{l}{\textbf{uSaber}}                     & This paper                               &                      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 1,062  &  & \textbf{2,462} &  &  & \textbf{4,419} &           &           & \textbf{6,888} &           &  & \textbf{10,224} &                      &                      & \textbf{35,888} &                      &                      & \textbf{77,920} &  &  \\ \hline
{\color[HTML]{000000} }                                 & {\color[HTML]{000000} This paper}        & \multicolumn{1}{c}{} &                      &                      & 1,121  &  & \textbf{3,011} &  &  & \textbf{5,534} & \textbf{} & \textbf{} & \textbf{8,591} & \textbf{} &  & \textbf{12,432} &                      &                      & \textbf{42,800} &                      &                      & \textbf{91,744} &  &  \\
{\color[HTML]{000000} }                                 & \cite{BronchainC22}                      &                      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 773    &  & 5,027          &  &  & 7,320          &           &           & 9,988          &           &  & -               &                      &                      & -               &                      &                      & -               &  &  \\
\multirow{-3}{*}{{\color[HTML]{000000} \textbf{Saber}}} & \cite{FO-masked-saber}$\dagger$                   &                      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 1,123  &  & 2,833          &  &  & -              &           &           & -              &           &  & 11,656          &                      &                      & -               &                      &                      & -               &  &  \\ \hline
                                                        & \cite{ho-mask-comparator-kyber-bos-2021}$\dagger$ & \multicolumn{1}{c}{} &                      &                      & 882    &  & 3,116*         &  &  & 44,347         &           &           & 115,481        &           &  & 12,072*         &                      &                      & 902,126         &                      &                      & 2,434,170       &  &  \\
                                                        & \cite{BronchainC22}                      &                      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & 804    &  & 7,716          &  &  & 11,880         &           &           & 16,715         &           &  & -               &                      &                      & -               &                      &                      & -               &  &  \\
\multirow{-3}{*}{\textbf{Kyber}}                        & \cite{FO-masked-kyber-HeinzKLPSS22}$\dagger$      & \multicolumn{1}{c}{} &                      &                      & 816    &  & 2,978$^*$          &  &  & -              &           &           & -              &           &  & -               &                      &                      & -               &                      &                      & -               &  &  \\ \hline
\end{tabular}%
}
\text{$\dagger$: measurements are taken from the paper}\\
\text{*: uses optimized implementation for first-order masking}
\end{table}

==> sections/application_fa.tex <==
\section{Application of Our Fault Attack on LWE-Based Schemes}

As concrete examples, we describe how to realize this attack on MLWE-based KEM Kyber and MLWR-based KEM Saber. However, with some modification, our attack can be applied to other LWE-based KEMs, for example, NewHope \cite{newhope}, Scabbard \cite{scabbard}, Lizard \cite{lizard}, and RLWE \cite{1st-order_masked_comparator}.

% \section{Application of Our Fault Attack on Kyber}\label{subsec:fault-attack-kyber}







\subsection{Application of our \texttt{stuck-at} fault attack on Saber:}

\begin{figure}[!tbp]
  \centering
  \subfloat[Stuck-at-1 fault]{\includegraphics[width=0.35\textwidth]{images/saber-fault-stuck-at1.png}\label{fig:stuck-at-1}}
  \hfill
  \subfloat[Stuck-at-0 fault]{\includegraphics[width=0.35\textwidth]{images/saber-fault-stuck-at0.png}\label{fig:stuck-at-0}}
  \caption{Results of \texttt{stuck-at} fault attacks on Saber. The probability distribution of $z$ is shown in these figures. The solid curve represents all the values of $z$ that decoded to the message value $0$, and the dashed curve represents all the values of $z$ that decoded to the message value $1$. The inserted fault will corrupt the message value with probability $1/2$ whenever the value of $z$ lies on the red part.}
\end{figure}


In Saber, $q=p$ is power-of-two and $k = \epsilon_p$. The decoding algorithm in Saber is 




Usually, $z$ follows a bell-shaped distribution with a peak at $p/4$ when $z^k$ is 0, \textit{i.e.} for the corresponding message bit $0$. The values of $z$ follow a bell-shaped distribution with a peak at $3p/4$ when $z^k$ is 1, \textit{i.e.} for the corresponding message bit $1$. From Lemma~\ref{lemma:stuck-at-1-for-k}, we get that the injected \texttt{stuck-at-1} fault at the $(\epsilon_p-1)$-th bit of a share of $z$ propagates and causes decryption failure if it is active and $z \in \{(p/4),\ (p/4)+1,\ \ldots,\ (p/2)-1\} \cup \{3(p/4),\ 3(p/4)+1,\ \ldots,\ p-1\}$. The injected fault is active with $1/2$ probability. Also, if $z \in \{0,\ 1,\ \ldots,\ (p/4)-1\} \cup \{(p/2),\ (p/2)+1,\ \ldots,\ 3(p/4)-1\}$, then the fault does not propagate and hence doe not cause decryption failure. We use Figure \ref{fig:stuck-at-1} to show the values of $z$ in which the \texttt{stuck-at-1} fault propagation is successful and the values of $z$ in which this fault will not cause decryption failure. In this figure, we use a solid bell curve to denote the distribution for the message bit $0$ and a dashed bell curve to indicate the distribution for the message bit $1$. From Lemma~\ref{lemma:stuck-at-0-for-k}, we get that the injected \texttt{stuck-at-0} fault at the $(\epsilon_p-1)$-th bit of a share of $z$ propagates and causes decryption failure if it is active and $z \in \{0,\ 1,\ \ldots,\ (p/4)-1\} \cup \{(p/2),\ (p/2)+1,\ \ldots,\ 3(p/4)-1\}$. Also, if $z \in \{(p/4),\ (p/4)+1,\ \ldots,\ (p/2)-1\} \cup \{3(p/4),\ 3(p/4)+1,\ \ldots,\ p-1\}$ then decryption failure does not arise. Figure \ref{fig:stuck-at-0} represents the values of $z$ for both cases when the \texttt{stuck-at-0} fault propagation is successful and when fault propagation is not. 



% In this section, we describe the specifics of how to apply our fault attack idea when $q$ is prime to recover the non-ephemeral secret key by exploiting the carry chain of the adder in the \texttt{A2B} conversion. We have chosen Kyber for demonstration as it has been selected as standard by NIST. 



%old

A pictorial version of the masked decoding algorithm as presented in Algorithm \ref{algo:masked-decode} is shown in Figure \ref{fig:masked-decoding}. Here, the first figure shows the distribution of a coefficient of $m''$,\ $m''[i]$, and the second figure presents the distribution of that coefficient after the subtraction with $q/4$. The third figure expresses the distribution of that coefficient after the transformation from $\mathbb{Z}_{q}$ to $\mathbb{Z}_{2^{13}}$, and the last figure display the distribution of that coefficient after the subtraction with $q/2$. After this, the \texttt{A2B} conversion takes place and produces Boolean shares $(d_1[i],\ d_2[i])$ in Algorithm \ref{algo:masked-decode}. Then the $13$-th bits of $(d_1[i],\ d_2[i])$ are calculated and act as the shares of $m'[i] = (m'_1[i],\ m'_2[i])$. However, here the $12$-th bits of $(d_1[i],\ d_2[i])$ can also act as the shares of $m'[i]$. That means $(d_1^{13}[i],\ d_2^{13}[i]) = (d_1^{12}[i],\ d_2^{12}[i]) = (m'_1[i],\ m'_2[i])$. This happens due to the application of \texttt{transform-power-of-2} followed by $q/2$ subtraction (shown in \autoref{fig:masked-decoding}) in the masked \texttt{Decode} algorithm. 

Here, we inject fault at $11$th bit of $i$th coefficient in one of the arithmetic shares $(c_1[i],\ c_2[i])$. These are inputs of \texttt{A2B} as shown in Algorithm \ref{algo:masked-decode}. Let us assume that $\tilde{c} = (c_1 + c_2) \bmod{q}$ Suppose after the fault is injected the message polynomial $m'$ becomes $m^*$ if we consider $12$-th bit of the Boolean masked output of \texttt{A2B} or becomes $m^{**}$ if we consider $13$-th bit of the Boolean masked output of \texttt{A2B}. In any case, the fault will result in a decryption failure ($m'[i] \neq m^*[i]$ or $m'[i] \neq m^{**}[i]$, for some $i$) depending on the fault type, the value of the specific input share where the fault has been introduced, and the unmasked value of the input. We provide a more thorough analysis in the following paragraphs.



%\subsubsection*{\texttt{Stuck-at-1} fault:}\label{subsubsec:fault-attack-kyber-1}

% In this attack, we apply a \texttt{stuck-at-1} fault at $11$-th bit of a coefficient in one of the arithmetic shares of $\tilde{c}$, $(c_1[i],\ c_2[i])$, which is an input to \texttt{A2B}. Let us assume that after the injection of the fault the unmasked value of the output of \texttt{A2B} $d^*$ and the $i$-th coefficient is $d^*[i]$. Also, presume that after fault, the message polynomial $m'$ becomes $m^*$ or $m^{**}$. Here, the result of the fault also relies on the assignment of $(m'_1[i],\ m'_2[i])$ as $(d_1^{12}[i],\ d_2^{12}[i])$ or $(d_1^{13}[i],\ d_2^{13}[i])$. 
\noindent
\textbf{\texttt{Stuck-at-1} fault:}
% In this attack, we apply a \texttt{stuck-at-1} fault at $11$-th bit of a coefficient in one of the arithmetic shares of $\tilde{c}$, $(c_1[i],\ c_2[i])$, which is an input to \texttt{A2B}. 
$\tilde{c}$ is the unmasked value of the input arithmetic shares of \texttt{A2B}. Here, we use a \texttt{stuck-at-1} fault at $c_1[i]^{11}$ which is $11$th bit of $i$th coefficient of an arithmetic share of $\tilde{c}$.
Let us assume that after the fault injection, the message polynomial $m'$ becomes $m^*$ or $m^{**}$. Here, the result of the fault also relies on the assignment of $(m'_1[i],\ m'_2[i])$ as $(d_1^{12}[i],\ d_2^{12}[i])$ or $(d_1^{13}[i],\ d_2^{13}[i])$. 

\textbf{If} $\mathbf{(m'_1[i],m'_2[i]) = (d_1^{12}[i],\ d_2^{12}[i])):}$ In this situation, we use Figure \ref{fig:kyber-fault-at1-1} to illustrate in which cases the fault will propagate and cause decryption failure and in which cases the fault will not cause decryption failure. The values of $\tilde{c}[i]$ would cause decryption failure are $\{2^{10},\ 2^{10}+1,\ \ldots,\ \lfloor q/2 \rceil-1\}$ when $m'[i]=0$ and  $\{2^{12}+2^{11}+2^{10},\ 2^{12}+2^{11}+2^{10}+1,\ \ldots,\ q-1\}$ when $m'[i]=1$. Here we insert a \texttt{stuck-at-1} fault at the $11$th bit of $c_1[i]$ (without loss of generality). This fault will only be active if the $11$th bit of $c_1[i] = 0$, and propagate if $11$th bit of $\tilde{c}[i]=1$. Also, $c_1[i]$ is random in $\mathbb{Z}_{2^{13}}$, the $11$th bit of $c_1[i]$ will be $0$ for $2^{12}$ cases in between $2^{13}$ probable cases. So, the injected fault at $c_1[i]^{11}$ is active with probability $1/2$.
%So, for a random value of $c_1[i]^{11}$ will be $0$ with probability $1/2$.

\textbf{If} $\mathbf{(m'_1[i],\ m'_2[i]) = (d_1^{13}[i],\ d_2^{13}[i]):}$ Figure \ref{fig:kyber-fault-at1-2} presents in which situations the fault will propagate and cause decryption failure and in which situations the fault will not cause decryption failure. The values of $\tilde{c}[i]$ would cause decryption failure are $\{2^{12}+2^{11}+2^{10},\  2^{12}+2^{11}+2^{10}+1,\ \ldots,\ q-1\}$ and only when $m'[i]=1$. As discussed in the previous paragraph, here also, the injected fault at $c_1[i]^{11}$ is active with probability $1/2$.
%a random value of $c_1[i]^{11}$ will be $0$ with probability $1/2$. 

Verification: Let us assume $\tilde{c} = (c_1 + c_2) \bmod{q} = (d_1 \xor d_2)$. For simplicity, we rename $c_1[i]$ as $x$ and $c_2[i]$ as $y$. So now, $\tilde{c}[i] = z = x + y \bmod{q}$. $m'[i] = z^{13} = x^{13} \xor y^{13} \xor c^{12}$, where $c^{12}$ is the carry for $12$th bit.
% \begin{center}
%     $m'[i] = z^{13} = x^{13} \xor y^{13} \xor c^{12}$, where $c^{12}$ is the carry for $12$th bit.
% \end{center}
Let us assume that after the fault is injected the carry $c$ becomes $c^*$. Decryption failure will occur if, after injecting fault, the new message $m^{**}[i] \neq m'[i]$. It is possible if $c^{*12} \neq c^{12}$. $c^{11} = (c^{10} \& (x^{11} \xor y^{11})) \xor (x^{11} \& y^{11}) = (x^{11}\& (c^{10} \xor  y^{11})) \xor (c^{10} \& y^{11})$.
% \begin{center}
%     $c^{11} = (c^{10} \& (x^{11} \xor y^{11})) \xor (x^{11} \& y^{11}) = (x^{11}\& (c^{10} \xor  y^{11})) \xor (c^{10} \& y^{11})$.
% \end{center}

The \texttt{stuck-at-1} fault at $x^{11}$ affects the $11$th bit of $z$, if $c^{11} \neq c^{*11}$. This happens if $x^{11} = 0$ and $(c^{10} \xor y^{11}) = 1$. So, $z^{11} = c^{10} \xor y^{11} \xor x^{11} = 1$. So, before fault $11$th carry bit $c^{11} = (x^{11} \& (c^{10} \xor y^{11} )) \xor (c^{10} \& y^{11})$, $x^{11} = 0$, and $c^{10} \xor y^{11} = 1$. $c^{10} \xor y^{11} = 1$ implies that $c^{10} \& y^{11} = 0$. So, $c^{11} = 0$. Also, $c^{12} = (c^{11} \& (x^{12} \xor y^{12})) \xor (x^{12} \& y^{12})$. As mentioned before, the fault at $x^{11}$ affect the $12$th bit of $z$ if $c^{12} \neq c^{*12}$, that means if $x^{12} \xor y^{12} = 1$. It also implies that $z^{12} = c^{11} \xor ( x^{12} \xor y^{12} )=0 \xor 1 = 1$. So, the \texttt{stuck-at-1} fault at $x^{11}$ affects the message bit $m^{**}[i]$ which is the $13$th bit of $z$ if $z^{11} = 1$, $z^{12} = 1$ and $x^{11} = 0$. This is only possible in cases where the message bit $m'[i]$ is 1.
Each $z = x + y \bmod{q}$ can be divided into two shares in $2^{13}$ possible ways when $x,\ y \in \mathbb{Z}_{2^{13}}$, and the injected \texttt{stuck-at-1} fault is active at $x^{11}$ in $2^{12}$ possible ways. It happens because in other $2^{12}$ combinations, $x^{11}$ is already $1$, and \texttt{stuck-at-1} fault does not induce any fault. 
% Each $z = x + y \bmod{q}$ can be divided into two shares in $2^{13}$ possible ways when $x,\ y \in \mathbb{Z}_{2^{13}}$, and the decryption failure only occurs in $2^{12}$ possible ways. It happens because in other $2^{12}$ combinations, $x^{11}$ is already $1$, and \texttt{stuck-at-1} does not induce any fault. 
In summary, the \texttt{stuck-at-1} fault at ${c_1}[i]^{11}$ propagates and results in a decryption failure implies that $\tilde{c}[i]^{11} = 1$ and it is possible only when the corresponding $i$th message bit $m'[i]$ is 1. 
%In summary, the \texttt{stuck-at-1} fault at the $11$-th bit of a share of $i$th coefficient of the inputs of \texttt{A2B} result in a decryption failure implies that $\tilde{c}[i]=1$ and it is possible only when the $i$th message bit $m'[i]$ is 1.
% the unmasked value of the $11$-th bit is $1$ and it is possible only when the $i$th message bit $m'[i]$ is 1. 

\begin{figure}[!tbp]
  \centering
  \subfloat[If considered $12$-th bit as message]{\includegraphics[width=0.4\textwidth]{images/kyber_fault_at1_1.png}\label{fig:kyber-fault-at1-1}}
  \hfill
  \subfloat[If considered $13$-th bit as message]{\includegraphics[width=0.4\textwidth]{images/kyber_fault_at1_2.png}\label{fig:kyber-fault-at1-2}}
  \caption{Results of \texttt{stuck-at-1} fault attacks on Kyber. The solid curve represents the probability distribution of a coefficient that decoded to the message value $m'[i]=0$ and the dashed curve represents the probability distribution of a coefficient that decoded to the message value $m'[i]=1$. This picture also presents that the inserted fault will corrupt the message value $m'$ with probability $1/2$ whenever it lies on the red part.}
\end{figure}

%\subsubsection*{\texttt{Stuck-at-0} fault:}\label{subsubsec:fault-attack-kyber-0}

% Here, we use a \texttt{stuck-at-0} fault at $11$-th bit of $i$-th coefficient in one of the arithmetic shares and the input of \texttt{A2B}, $c_1[i]$. Suppose the unmasked value of the output of \texttt{A2B} is $d^*$ and the $i$-th coefficient is $d^*[i]$. Also, assume that if the fault is not given, then $d^*$ would be $d$, and after the fault is given, the message polynomial $m'$ evolves $m^*$ or $m^{**}$. Like the previous \texttt{stuck-at-1} fault at Kyber, the result of the fault depends on whether we are assigning $(m'_1[i],\ m'_2[i])$ as $(d_1^{12}[i],\ d_2^{12}[i])$ or $(d_1^{13}[i],\ d_2^{13}[i])$. 

\noindent
\textbf{\texttt{Stuck-at-0} fault: }$\tilde{c}$ is the unmasked value of the input arithmetic shares of \texttt{A2B}. Here, we use a \texttt{stuck-at-0} fault at $c_1[i]^{11}$ which is $11$th bit of $i$th coefficient of an arithmetic share of $\tilde{c}$. Suppose after the fault is injected, the message polynomial $m'$ evolves to $m^*$ or $m^{**}$. Like the previous \texttt{stuck-at-1} fault at Kyber, the result of the fault depends on whether we are assigning $(m'_1[i],\ m'_2[i])$ as $(d_1^{12}[i],\ d_2^{12}[i])$ or $(d_1^{13}[i],\ d_2^{13}[i])$.

\textbf{If} $\mathbf{(d_1^{12}[i],\ d_2^{12}[i]) = (m'_1[i],\ m'_2[i]):}$ We use Figure \ref{fig:kyber-fault-at0-1} to show the cases where the fault will propagate and cause decryption failure and where it will not. The values of $\tilde{c}[i]$ can cause decryption failure are $\{0,\ 1,\ \ldots,\ 2^{10}-1\}$ if $m'[i]=0$ and $\{\lfloor q/2 \rceil,\ \lfloor q/2 \rceil+1,\ \ldots,\ 2^{12}+2^{11}+2^{10}-1\}$ if $m'[i]=1$. In this case, we insert a \texttt{stuck-at-0} fault at the $11$th bit of $c_1[i]$. The fault is only effective if the $11$th bit of $c_1[i] = 1$, and propagates if the $11$th bit of $\tilde{c}[i] = 0$. 
%Also, as we use \texttt{stuck-at-0} fault, the fault injection at $c_1[i]^{11}$ will be effective with probability $1/2$. 

\textbf{If} $\mathbf{(d_1^{13}[i],\ d_2^{13}[i]) = (m'_1[i],\ m'_2[i]):}$ The situations where the induced fault will propagate and cause decryption failure and the situations where it will not are shown in Figure \ref{fig:kyber-fault-at0-2}. The values of $\tilde{c}[i]$ would cause decryption failure are $\{0,\ 1,\ \ldots,\ 2^{10}-1\}$ and in all these circumstances $m'[i]=0$. Here as well, the injected fault at $c_1[i]^{11}$ is active with $1/2$ probability. 

Verification: Suppose $\tilde{c} = (c_1 + c_2) \bmod{q} = (d_1 \xor d_2)$. For simplicity, we rename $c_1[i]$ as $x$ and $c_2[i]$ as $y$. So, $\tilde{c}[i] = z = x + y \bmod{q}$. Now, $m'[i] = z^{13} = x^{13} \xor y^{13} \xor c^{12}$, where $c^{12}$ is the carry for $12$th bit.
% \begin{center}
%     $m'[i] = z^{13} = x^{13} \xor y^{13} \xor c^{12}$, where $c^{12}$ is the carry for $12$-th bit.
% \end{center}
Let us assume that after the fault is injected the carry $c$ becomes $c^*$. Decryption failure will happen if, after giving fault, the new message $m^{**}[i] \neq m'[i]$. It is possible if new $c^{*12} \neq c^{12}$.
\begin{equation}
    c^{11} = (c^{10} \& (x^{11} \xor y^{11})) \xor (x^{11} \& y^{11}) = (x^{11} \& (c^{10} \xor  y^{11})) \xor (c^{10} \& y^{11}). \label{eq:stuck0kyber13}
\end{equation}
The \texttt{stuck-at-0} fault at $x^{11}$ affects the $11$th bit of $z$ if $c^{11} \neq c^{*11}$ and it happens if $x^{11} = 1$ and $(c^{10} \xor y^{11}) = 1$. So, $z^{11} = c^{10} \xor y^{11} \xor x^{11} = 1 \xor 1 = 0$. 
% So, $c^{11} = (x^{11} \& (c^{10} \xor y^{11} )) \xor (c^{10} \& y^{11}) = 1 \xor 0 = 1$, because $c^{10} \xor y^{11} = 1$. 
Now, $x^{11} = 1$, and $c^{10} \xor y^{11} = 1$. $c^{10} \xor y^{11} = 1$ implies that $c^{10} \& y^{11} = 0$. So, from Equation \ref{eq:stuck0kyber13} we get $c^{11} = 1$. Also, $c^{12} = (c^{11} \& (x^{12} \xor y^{12})) \xor (x^{12} \& y^{12})$. As mentioned before, the fault at $x^{11}$ affect the $12$th bit of $z$ if $c^{12} \neq c^{*12}$, that means if $x^{12} \xor y^{12} = 1$. It also implies that $z^{12} = c^{11} \xor ( x^{12} \xor y^{12} )=1 \xor 1 = 0$. So, the \texttt{stuck-at-0} fault at $x^{11}$ affects the message bit $m^{**}[i]$ which is the $13$th bit of $z$ if $z^{11} = 0$, $z^{12} = 0$ and $x^{11} = 0$. It happens only in cases where the message bit $m'[i]$ is 0. 
% Each $d[i] = x + y$ can be divided into two shares in $2^{13}$ possible ways when $x,\ y \in \mathbb{Z}_{2^{13}}$, and the decryption failure only happens in $2^{12}$ possible ways. It occurs because in other $2^{12}$ combinations, $x^{11}$ is already $1$, and \texttt{stuck-at-0} does not render any fault. 
Since we apply \texttt{stuck-at-0} fault, it is only effective for half of the total possible cases.
In summary, the \texttt{stuck-at-0} fault at ${c_1}[i]^{11}$ propagates and results in a decryption failure implies that $\tilde{c}[i]^{11} = 0$ and it is possible only when the $i$th message bit $m'[i]$ is 0. 

\begin{figure}[!tbp]
  \centering
  \subfloat[If considered $12$-th bit as message]{\includegraphics[width=0.4\textwidth]{images/kyber_fault_at0_1.png}\label{fig:kyber-fault-at0-1}}
  \hfill
  \subfloat[If considered $13$-th bit as message]{\includegraphics[width=0.4\textwidth]{images/kyber_fault_at0_2.png}\label{fig:kyber-fault-at0-2}}
  \caption{Results of \texttt{stuck-at-0} fault attacks on Kyber. The solid curve represents the probability distribution of a coefficient that decoded to the message value $m'[i]=0$, and the dashed curve represents the probability distribution of a coefficient that decoded to the message value $m'[i]=1$. This picture also presents that the inserted fault will corrupt the message value $m'$ with probability $1/2$ whenever it lies on the red part.}
\end{figure}


==> sections/countermeasure.tex <==
\section{Countermeasure}\label{sec:countermeasure}

% The addition of shuffling techniques in the decoding part of the masked KEM decapsulation implementation can make our attack harder. In this situation, we need to accommodate some non-trivial modification, such as considering side-channel leakages for the permutation used in shuffling together with the inequalities generated by introducing faults during the decapsulation process to recover the secret key. 

Shuffling~\cite{DBLP:conf/acns/HerbstOM06} is a technique that has been used as a countermeasure of SCA by shuffling the order of execution of the independent operations. Adding shuffling techniques in the decoding part of the masked KEM decapsulation implementation by scrambling the coefficient indexes of the input polynomial of the \texttt{A2B} algorithm can make our attack harder. To construct an inequality from an effective propagated fault, we need to know the coefficient index $i$ where the \texttt{stuck-at} fault is injected. In this situation, we need to accommodate some non-trivial modification, such as considering side-channel leakages for the permutation used in shuffling and the inequalities generated by introducing faults during the decapsulation process to recover the secret key. 

==> sections/recover_secret.tex <==
%\section{Recovering Secret Key from Our Fault Attack}\label{sec:inequality-solve}
\section{Recovery of the Secret Key}\label{sec:inequality-solve}

%In this section, we will discuss how we can use our attack to retrieve the secret key of a scheme. 

\textcolor{violet}{This section will describe the final stage of our attack \textit{i.e.} recovering the secret key for Kyber. As mentioned earlier, decryption noise forms a linear equation with the secret key $\pmb{s}$ and error $\pmb{e}$. The decryption noise for LWE-based KEM is equal to $\pmb{e}^T \pmb{s}'[i] - \pmb{s}^T(\pmb{e_1}[i] + \Delta \pmb{u}[i]) + e_2[i] + \Delta v[i]$, where $\Delta \pmb{u}$ and $\Delta {v}$ are the noise introduced because of compression operation over $\pmb{u}$ and $v$, respectively. In our case, a decryption failure is observed only when the message bit $m[i] = 1$, and the corresponding 11th bit is also 1. %If a decryption failure is observed, then the message bit is $m[i] = 1$ (mentioned in Section~\ref{subsec:fault-attack-kyber}). 
The decryption noise satisfies the following inequality. 
%If a decryption failure is observed, then    
\begin{equation}
    (\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] \geq \lfloor q/4 \rfloor - ( 2^{10} - \lfloor q/4 \floor). \label{eq:ky1}
\end{equation}
In case of a decryption success, then the following inequality holds with probability $\frac{1}{2}$. \textcolor{red}{(This is because we also observe decryption success if the fault is not \emph{active}).}}    
\textcolor{violet}{
\begin{equation}
    (\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] < \lfloor q/4 \rfloor - ( 2^{10} - \lfloor q/4 \rfloor). \label{eq:ky2}
\end{equation}
\textcolor{red}{As mentioned in Section \ref{sec:fault-attack},} the attacker has access to the encapsulation oracle and works with self-generated ciphertexts. So, the attacker knows all the values in Equation \ref{eq:ky1} \& \ref{eq:ky2}, except $(\pmb{e},\ \pmb{s})$. The attacker can find the polynomials $(\pmb{e},\ \pmb{s})$ by solving these linear inequalities.}

% In both of these equations, except $(\pmb{e},\ \pmb{s})$, the attacker knows all other values. So, we can find the polynomials $(\pmb{e},\ \pmb{s})$ by solving these linear inequalities. 

% If we apply a \texttt{stuck-at-0} fault on Kyber in the case when $(m'_1[i],\ m'_2[i])$ assign as $(d_1^{12}[i],\ d_2^{12}[i])$ and observe a decryption failure then for message bit $0$ and $1$ we receive the following equations, respectively. 
% \begin{equation*}
%     (\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] < 2^{10},
% \end{equation*}
% \begin{equation*}
%     (\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] < \lfloor q/4 \rceil - ( 2^{10} - \lfloor q/4 \rceil). 
% \end{equation*}
% \begin{center}
%     $(\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] < 2^{10},$\\
%     $(\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] < \lfloor q/4 \rceil - ( 2^{10} - \lfloor q/4 \rceil)$. 
% \end{center}
% If we apply a \texttt{stuck-at-1} fault on Kyber when $(m'_1[i],\ m'_2[i])$ assign as $(d_1^{13}[i],\ d_2^{13}[i])$ and obtain a decryption failure then the message bit is $1$ and we receive the latter equation. 
% \begin{equation*}
%      (\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] \geq \lfloor q/4 \rceil - ( 2^{10} - \lfloor q/4 \rceil). 
% \end{equation*}
% When we use a \texttt{stuck-at-0} fault on Kyber when $(m'_1[i],\ m'_2[i])$ assign as $(d_1^{13}[i],\ d_2^{13}[i])$ and observe a decryption failure then the message bit is $0$ and we get the following equation. 
% \begin{equation*}
%     (\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] < 2^{10}.
% \end{equation*}

% For Saber, $(m'_1[i],\ m'_2[i])$ is assigned as $(m_{b_1}^{10}[i],\ m_{b_2}^{10}[i])$. If a decryption failure is observed and message bit $m'[i]$ is equals to $0$, then $(\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] \geq 2^{8}.$
% % \begin{equation*}
% %     (\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] \geq 2^{8}.  
% % \end{equation*}
% Here, $\pmb{e},\ \pmb{e_1},\ \Delta \pmb{u}$ and $\Delta {v}$ are all rounding errors. If the message bit $m[i] = 1$ and decryption failure is observed, then $(\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] \geq 2^{8}.$   
% % \begin{equation*}
% %     (\pmb{e},\ \pmb{s})^T (\pmb{s}'[i],\  - (\pmb{e_1}[i] + \Delta \pmb{u}[i])) + e_2[i] + \Delta v[i] \geq 2^{8}. 
% % \end{equation*}
% Here, also, in both of these equations, except $(\pmb{e},\ \pmb{s})$, other values are known to the attacker. Similarly, as Kyber, one can retrieve the coefficients of $(\pmb{e},\ \pmb{s})$ by solving these linear inequalities. 

% %A few inequality solvers have been proposed in recent years \cite{PesslP21,HermelinkPP21,Delvaux22,HermelinkMSPR23}. Figure \ref{fig:solver-security-level} provides an idea of how many decryption failures we need to break the masked Kyber-768 using the results we obtain from the \texttt{stuck-at-1} fault on Kyber and the case when $(m'_1[i],\ m'_2[i])$ assign as $(d_1^{12}[i],\ d_2^{12}[i])$ and the inequality solver proposed by Delvaux et al. in \cite{Delvaux22}. Because here, we only receive an inequality when a decryption failure happens. In the case of decryption success, we cannot get any inequality as we have used stuck-at fault, and it affects the output $50\%$ of the time. A decryption success can be obtained for an ineffective fault case as well. Similar results can be obtained when other \texttt{stuck-at} faults are applied on any security versions of Kyber and Saber.

\textcolor{violet}{A few inequality solvers have been proposed in recent years \cite{PesslP21,HermelinkPP21,Delvaux22,HermelinkMSPR23}. All these solvers are based on BP in order to tolerate errors and solve the system with a large number of inequalities in a reasonable amount of time. In this work, we have used the inequality solver proposed by Delvaux et al. in \cite{Delvaux22} to solve the inequalities obtained from the \texttt{stuck-at-1} fault on Kyber.
The fault injected at index $i$ is kept the same for all the inequalities, where $i \in \{0,\ 1,\ \ldots,\ 256\}$. If we consider $\omega$ numbers of inequalities, then the system of inequality contains $\omega$ inequalities with $\psi$ unknowns. Here the value of $\psi$ is the total number of coefficients of $\pmb{s}$ and $\pmb{e}$, which is $2*l*256$, $l=2$ for Kyber-$512$. This inequality solver uses an iterative method to solve the system of $\omega$ inequalities by maintaining a  probability mass function (PMF) for each of $\psi$ unknowns. The PMF for each unknown initiated with the CBD on $[-\eta,\ \eta]$ and updated in each iteration. The updation of PMF for each unknown is performed by calculating the probability to satisfy each of the $\omega$ inequalities for each possible value $[-\eta,\ \eta]$ of the unknown, and then all the $2*\eta*\omega$ probabilities are combined. \cite{Delvaux22} accelerates the computation time of their solver by applying the central limit theorem. The iteration of the updation of PMF for each unknown continues until a suﬃciently approximate one-point distribution on $[-\eta,\ \eta]$ is found.}
% % Figure \ref{fig:solver-security-level} shows how many decryption failures we need to break the masked Kyber-768. Here, we only receive an inequality when a decryption failure happens. 
% Figure \ref{fig:solver-security-level} shows the number of decryption failures required to extract the secret key for masked Kyber-$768$ when $(m'_1[i],\ m'_2[i])$ assign as $(d_1^{12}[i],\ d_2^{12}[i])$.
% In the case of decryption success, we cannot get any inequality as we have used stuck-at fault, and it affects the output $50\%$ of the time. A decryption success can be obtained for an ineffective fault case as well. Similar results can be obtained when other \texttt{stuck-at} faults are applied on any security versions of Kyber and Saber.

% % \begin{figure}[htp]
% %     \centering
% %     \includegraphics[width=0.8\textwidth]{images/solver-security-level.png}
% %     \caption{Solving inequalities for Kyber-768 with Delvaux et al.'s inequality solver \cite{Delvaux22}}
% %     \label{fig:solver-security-level}
% \end{figure}


==> sections/setup.tex <==
\subsection{Attack Platform and Experimental Setup}
For our experiments, we target the reference implementation of the considered scheme built for the ARM Cortex-M4 family of microcontrollers. We ported the reference implementation to the STM32F4DISCOVERY board (DUT) housing the STM32F407, ARM Cortex-M4 microcontroller running at a clock frequency of 24 MHz. We have used a generic USB 2.0 to TTL converter for USART communication with the DUT. We use Electromagnetic Fault injection (EMFI) to inject faults into our device.

The most formidable challenge in executing the aforementioned attack is inducing the faults accurately at specific locations. We have established an injection setup to address this challenge, illustrated in Figure \ref{fig:fault_setup}. This setup consists of several components, including an arbitrary waveform generator (Keysight 81160A), a constant-gain power amplifier (Teseq CBA 400M-260), a high-frequency near field H-probe (Rigol Near-field Probe 30MHz-3GHz), and an XYZ table (Thorlabs SMC100). Figure \ref{fig:probe_pos}
shows the position of the near-field EM probe on the DUT. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{images/fault_setup.png}
    \caption{Schematic of the attack platform}
    \label{fig:fault_setup}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{images/probe_position.jpg}
    \caption{The position of the probe on the STM32F4 Discovery board}
    \label{fig:probe_pos}
\end{figure}

After being triggered by a signal from the evaluation board hosting the target implementation, the waveform generator produces a high-frequency pulse train. Following this, the amplifier boosts the intensity of this pulse train, and the H-probe generates a magnetic field above the target. It's important to highlight that the pulse train's amplitude, frequency, and burst count can be customized to meet particular needs. It was observed that by manipulating the position of the probe over the target using the XYZ table, with some necessary adjustments to the pulse parameters, fault can be induced in the specific bit of the target register. However, this positioning process must rely on a trial-and-error approach due to the absence of internal register visibility. 

Initially, we analyzed the target object file to get an insight into the occurrence of a particular instruction where we can inject the desired fault. We have targeted a specific arithmetic instruction to induce the fault in the desired register. However, even when the fault location is found, repeating the injections an arbitrary number of times by fixing the probe location and pulse
parameters does not guarantee the induction of a single-bit fault at the target register. Initially, after injecting faults at the target location, we observed that multi-bit faults were also induced,  specifically towards the LSB of the target register. After tweaking the pulse and burst parameters from the waveform generator, we were able to obtain $10\%$ single-bit faults at the 11\textsuperscript{th} bit and $90\%$ multi-bit faults at the bit positions $0-7$. The pulse parameters were: \emph{Pulse Amplitude:} -5.6 dBm, \emph{Pulse Frequency:} 200 MHz, \emph{Burst Count:} 2.  


\textcolor{purple}{For the compilation of the reference implementation, we have
used arm-none-eabi-gcc version 15:10.3 with compiler flags \emph{-O3 -std=gnu99 -mthumb
-mcpu=cortex-m4 -mfloat-abi=hard -mfpu=fpv4-sp-d16}.}


==> throw.tex <==
%Therefore, the inputs to the masked centered uniform sampler are Boolean masked pseudorandom numbers. 

%In uSaber, the coefficients of secret vector is sampled according to the centered uniform distribution $\mathcal{U}_u$ instead of the centered binomial distribution $\beta_\mu$. Here, the hamming weight computation of the centered binomial distribution is replaced by sampling from centered uniform distribution, which is essentially sign extension of $u$ bits to $\epsilon_q$ bits, where $u$ bits are chosen uniformly random $[0,2^{u}-1]$. This secret vector sampler is the only different component used in the decapsulation algorithm of uSaber to substitute Saber's centered binomial sampler. The decapsulation algorithm of uSaber is shown in Figure~\ref{fig:usaberdecaps} and the only different component of uSaber from Saber is circled in color blue. One main advantage of uSaber against Saber is the centered uniform sampler has fewer number operations compared to the centered binomial sampler and is easier to mask. 

%In uSaber, each coefficient of the secret vector is generated using the centered uniform sampler generating numbers in the range $[-2^{(u-1)},2^{(u-1)}-1]$. 

, and that the improvements increase with the increase in masking order

In this work, we propose a higher-order side-channel attacks-resistant Saber and uSaber. The performance first-, second- and third-order masked-Saber has factors xxx, 6.2x and 9.4x overhead compared to unmasked Saber in the Cortex-M4 platform. The performance of higher-order masked Saber is better than higher-order masked Kyber due to the advantage of the power-of-two moduli and the use of the MLWR hard problem in masked Saber. 

The performance of masked uSaber has factors xxx, 6.2x and 9.4x overhead compared to unmasked uSaber for first-, second- and third-order, respectively. We obtain that higher-order masked uSaber achieves better performance and requires fewer random bytes than masked Saber and Kyber for any order. uSaber acquires these advantages against Saber while providing the same level of security due to the only difference in its secret sampler and parameters choices.

As we mentioned earlier, integrating NTT multiplication in place of the hybrid multiplication of Saber and uSaber can give a performance boost for masked implementations. We keep this as future work.



Coron et al.~\cite{CoronGMZ21} proposed a simple ciphertext comparison algorithm based on \texttt{A2B} conversion and later D'Anvers et al.~\cite{D'AnversVV22} proposed an improved implementation of this algorithm by using bitsliced \texttt{A2B} conversion. Here We show that we can adapt a little change in this algorithm.  

Remember that the re-encrypted ciphertext $c^*$ is arithmetically masked and uncompressed, but the public ciphertext $c$ is unmasked and compressed. As mentioned earlier, our task is to verify whether $c$ equals $c^*$ after compression. In this method, we perform the following steps: firstly, we transform arithmetic shares of $c^*$ to Boolean shares by using \texttt{A2B} conversion algorithm, secondly, we compress the re-encrypted Boolean masked ciphertext $c^*$ by using coefficient wise logical right shift, thirdly, we subtract the public ciphertext $c$ from the compressed and masked re-encrypted ciphertext $c^*$. Finally, the result of subtraction decides the success or failure of the comparison algorithm. The detailed algorithm is displayed in Appendix~\ref{}.
 
In another way, we can swap the first and third steps. Here, first, we convert public ciphertext $c$ to the decompressed domain and then perform subtraction with the uncompressed and arithmetically masked re-encrypted ciphertext $c^*$. Second, we use \texttt{A2B} conversion on the arithmetic shares, and third, we use coefficient wise logical right shift. Then, we apply Algorithm~\ref{algo:BooleanAllBitsOneTest} on the output bits to determine success or failure. This method is shown in Algorithm~\ref{algo:MaskComp3}, and detailed analysis regarding the correctness of this method is present in Appendix~\ref{}.

%However, integrating NTT multiplication in a masked Saber implementation is not trivial\footnote{The implementation of \cite{tches:ChungHKSSY21} exploits the fact that the secret key is sampled from a small distribution. In a masked setting, however, the shares of the secret are uniformly distributed.}, so we keep this as future work. 

In this work, we propose a higher-order side-channel attacks-resistant Saber and uSaber. The performance of 2nd and 3rd order masked-Saber has factors 6.2x and 9.4x overhead compared to unmasked Saber in the Cortex-M4 platform. The performance of higher-order masked Saber is better than higher-order masked Kyber due to the advantage of the power-of-two moduli and the use of the bitsliced A2B algorithm in masked Saber. 

Our next target is to experimentally demonstrate that our implementation of masked Saber is higher-order side-channel attacks resistant by using the Test Vector Leakage Assessment methodology. 

Masking Saber requires both kinds of masking techniques, arithmetic masking and Boolean masking. Hence, we need to use costly A2B and B2A conversion. If we can reduce the number of conversion algorithms or use efficient algorithms, then the performance of higher-order masked Saber will improve significantly. Therefore, one of our future works is to construct efficient algorithms for masked Saber, maintaining the security assumption.    

Recently, Coron et al.~\cite{CoronGMZ21}, D’Anvers et al.~\cite{D'AnversVV22}, and Bronchain et al.~\cite{BronchainC22}  proposed new masking techniques to improve the performances of the higher-order masking implementations. We did not include all those improvements in our work. In the future, we will incorporate those techniques to improve our higher-order masked Saber implementations.

In~\cite{ho-mask-comparator-kyber-bos-2021}, Bos et al. propose a higher-order masked Kyber. We compare the performances of our masked Saber implementations with the implementation results of masked Kyber in the Cortex-M4 platform and present in Table~\ref{tab:performance_comp}. Further, this table contains the performance of first-order masked Saber~\cite{FO-masked-saber} and first-order masked Kyber~\cite{FO-masked-kyber-HeinzKLPSS22}, which are specially optimized to prevent the first-order differential power attacks. We also add the performances of the decapsulation algorithms of the fastest Kyber~\cite{fast-kyber-AbdulrahmanHKS22} and fastest Saber, Saber NTT~\cite{Abdulrahman_Chen_Chen_Hwang_Kannwischer_Yang_2021}, in the table. 

Table~\ref{tab:performance_comp} shows masked Saber achieves better performance and needs fewer random bytes than masked Kyber for any order. The masked kyber implementation in~\cite{ho-mask-comparator-kyber-bos-2021} is faster and uses fewer random bytes than the implementation of our masked Saber only for first-order because this masked Kyber uses an optimized implementation for first-order, while Saber uses the generalized one. The performance for 2nd and 3rd order masked implementations of Saber achieve factor 6.3x and 10.89x improvement over Kyber, respectively. In terms of random bytes requirement, Saber receives factor 18.3x and 23.3x improvement over Kyber for 2nd and 3rd order masked implementations, respectively. Therefore, the performance improvement factor for masked Saber over masked Kyber increases with the increment of security order, and the random bytes requirement factor for masked Saber over masked Kyber decreases with the increment of security order. Note that the implementations of masked Kyber in ~\cite{ho-mask-comparator-kyber-bos-2021} did not use bitsliced A2B conversion algorithm, and the implementations of masked Kyber can receive significant speed-up by using bitsliced A2B. However, the learning with rounding based construction,  power-of-two moduli, and bitsliced A2B conversion algorithm help higher-order masked Saber implementations to attain better performances than masked Kyber~\cite{ho-mask-comparator-kyber-bos-2021}.
%Note that the implementation of Kyber in ~\cite{ho-mask-comparator-kyber-bos-2021} does not use bitslice A2B conversion algorithm. This bitslice A2B conversion algorithm and power-of-two moduli help higher-order masked Saber implementations to attain better performances.\MVB{But Kyber could also benefit from bit-sliced A2B}



Post-quantum cryptography (PQC) is another branch of PKC, and the cryptographic algorithms of PQC are based on hard mathematical problems that are assumed to be hard in the presence of quantum computers. Considering the rapid evaluation of quantum computers, the National Institute of Standards and Technology (NIST) started a procedure to standardize one or more post-quantum public-key cryptographic algorithms in 2016.



The arithmetic masking is efficient to protect arithmetic operations such as addition, subtraction, multiplication. We perform an $n$-order attack secure addition operation between two variables $x$ and $y$ when at least one of the two operands contains sensitive data in the following ways. If only $x$ contains sensitive data, we split $x$ into $n$ shares $\{x_i\}_{i=1}^n$ such that $\sum_{i=1}^n. x_i=x$, The shares of the resultant variable $z=x+y$ is $\{z_i\}_{i=1}^n$ where $z_i = \left\{ \begin{array}{ll} x_i+y & \mbox{if } i=1 \\ x_i & \mbox{else} \end{array}\right$ and $\sum_{i=1}^n z_i=z$.  


The arithmetic masking is efficient to protect arithmetic operations such as addition, subtraction, multiplication. Boolean operations are easy to defend by using Boolean masking. Bellow, we discuss how to mask a few simple operations, which we use in our implementation. 
\begin{enumerate}
    \item Addition operation when one of the two operands contains sensitive data: This operation is less costly to protect by using arithmetic masking. Split the sensitive data $x$ into $n$ shares $\{x_i\}_{i=1}^n$ such that $\sum_{i=1}^n x_i=x$ and $y$ be an unmasked polynomial. The shares of the resultant masked polynomial $x+y=z$ is $\{z_i\}_{i=1}^n$ where $z_i = \left\{ \begin{array}{ll} x_i+y & \mbox{if } i=1 \\ x_i & \mbox{else} \end{array}\right$ and $\sum_{i=1}^n z_i=z$.
    \item Addition operation when two operands contain sensitive data: This operation also easy to protect by using arithmetic masking. Let shares of masked polynomial $x$ be $\{x_i\}_{i=1}^n$ such that $\sum_{i=1}^n x_i=x$ and another masked polynomial $y$ be $\{y_i\}_{i=1}^n$ such that $\sum_{i=1}^n y_i=y$. The shares of the resultant masked polynomial $x+y=z$ is $\{z_i\}_{i=1}^n$ where $z_i = x_i+y_i, \forall{i}$ and $\sum_{i=1}^n z_i=z$.
    \item Multiplication between one masked and another unmasked polynomial: Let shares of masked polynomial $x$ be $\{x_i\}_{i=1}^n$ such that $\sum_{i=1}^n x_i=x$ and $y$ be an unmasked polynomial. The shares of the resultant masked polynomial $x\cdot y=z$ is $\{z_i\}_{i=1}^n$ where $z_i = x_i \cdot y, \forall{i}$ and $\sum_{i=1}^n z_i=z$.
\end{enumerate}



In $n$-th order masking, all the operations of the algorithms are performed on all the independent $n+1$ shares of the sensitive variable $x$ separately. On the other side, an adversary can exploit at most the leakage that occurs from the computation on the $n$ shares of $x$ for the case of $n$-th order differential power attack. Since all the shares of $x$ are random and any combination of $n$ shares of $x$ are independent with the sensitive variable $x$, the adversary will not receive any information regarding $x$ from the leakage.


In arithmetic masking, to obtain $n$ order security, the sensitive variable $x\in \mathbb{Z}_q$ needs to split into $n+1$ independent shares $x_1,x_2,\ldots,x_{n+1}\in \mathbb{Z}_q $. The relation between the sensitive variable $x$ and the $n+1$ shares of $x$ is $x=x_1+x_2+\cdots+x_{n+1} \mod{q}$. In Boolean masking, to obtain $n$ order security, the sensitive variable $x\in \mathbb{Z}_^k$ needs to split into $n+1$ independent shares $x_1,x_2,\ldots,x_{n+1}\in \mathbb{Z}_2^k $. The relation between the sensitive variable $x$ and the $n+1$ shares of $x$ in the case of Boolean masking is $x=x_1\xor x_2\xor\cdots \xor x_{n+1}$. 
 
Negation of a masked polynomial: Let shares of masked polynomial $x$ be $\{x_i\}_{i=1}^n$ such that $\sum_{i=1}^n x_i=x$. The shares of the resultant masked polynomial $\lnot x=z$ is $\{z_i\}_{i=1}^n$ where $z_i = \left\{ \begin{array}{ll} -x_i & \mbox{if } i=1 \\ x_i & \mbox{else} \end{array}\right$ and $\sum_{i=1}^n z_i=z$.
    
\begin{algorithm}[!ht]
\caption{ Masked Comparison }
\label{algo:MaskedComparison}

\Input{$\{\mathbf{b}'_i\}_{1\leq i \leq n}$ where each $\mathbf{b}'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} \mathbf{b}'_i = \mathbf{b}'$,\\
$\{c'_i\}_{1\leq i \leq n}$ where each $c'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} c'_i = c'$,\\
publicly avilable $\mathbf{b}$ and $c$}
\Output{$\{b_i\}_{1\leq i \leq n}$ with each $b_i \in \{0,1\}$ such that $\bigoplus_{i=1}^{n} b_i = 1$ iff\\ $\mathbf{b}''=\mathbf{b}'>>(\epsilon_q-\epsilon_p)=3$ and $c''=c'>>(\epsilon_p-\epsilon_t)=6$, else $0$}
\BlankLine

$\{w_i\}_{1\leq i \leq n} \leftarrow$ PolComp($\{\mathbf{b}'_i\}_{1\leq i \leq n}$,$\mathbf{b},\{c'_i\}_{1\leq i \leq n}$,$c$)\\
\For{\texttt{j=} $\log_2 256-1$ \texttt{to } $0$}
{
    $\{w'_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n}>>2^j $\\
    $\{w_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n} \mod(2^{2^j}-1)$\\
    $\{w_i\}_{1\leq i \leq n}\leftarrow SecAnd(\{w_i\}_{1\leq i \leq n}, \{w'_i\}_{1\leq i \leq n})$\\
}
\algorithmicreturn{ $\{w_i\}_{1\leq i \leq n}$}
\end{algorithm}



\begin{algorithm}[!ht]
\caption{ PolComp }
\label{algo:PolComp}

\Input{$\{\mathbf{b}'_i\}_{1\leq i \leq n}$ where each $\mathbf{b}'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} \mathbf{b}'_i = \mathbf{b}'$,\\
$\{c'_i\}_{1\leq i \leq n}$ where each $c'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} c'_i = c'$,\\
publicly avilable $\mathbf{b}$ and $c$}
\Output{$\{w_i\}_{1\leq i \leq n}$ where each $w_i \in \{0,1\}^{256}$}
\BlankLine
//\texttt{for $\mathbf{b}$ part of ciphertext}\\
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    $\mathbf{eb}[j]\leftarrow(\mathbf{b}[j]<<3)+4$\\
    $\mathbf{b}'_{n+1}[j]\leftarrow \mathbf{eb}[j]$\\
     $\{\mathbf{y}_i[j]\}_{1\leq i \leq n+1}\leftarrow$ A2B$(\{\mathbf{b}'_i[j]\}_{1\leq i \leq n+1})$
}
\For{\texttt{j1=} $1$ \texttt{to } $l=3$}
{
    \For{\texttt{s=} $1$ \texttt{to } $\epsilon_p=10$}
    {
        $\{\mathbf{x}_i[s][j]\}_{1\leq i \leq n+1}\leftarrow$ Bitslice$(\{\mathbf{y}_i[j]\}_{1\leq i \leq n+1}>>(s+3-1))$\\
        $\mathbf{x}_1[s][j]\leftarrow \mathbf{x}_1[s][j]\xor \mathbf{x}_{n+1}[s][j]$
    }    
}

//\texttt{for $c$ part of ciphertext}\\
$ec\leftarrow(c<<6)+64$\\
$c'_{n+1}\leftarrow ec$\\
$\{y_i\}_{1\leq i \leq n+1}\leftarrow$ A2B$(c'_i\}_{1\leq i \leq n+1})$

\For{\texttt{s=} $1$ \texttt{to } $\epsilon_t=4$}
{
    $\{z_i[s]\}_{1\leq i \leq n+1}\leftarrow$ Bitslice$(\{y_i\}_{1\leq i \leq n+1}>>(s+6-1))$\\
    $z_1[s]\leftarrow z_1[s]\xor z_{n+1}[s]$
}
//Combine the results of both parts of ciphertexts\\
$\{w_i\}_{1\leq i \leq n}\leftarrow \{z_i[1]\}_{1\leq i \leq n}$\\
\For{\texttt{s=} $2$ \texttt{to } $\epsilon_t=4$}
{
    $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\{z_i[s]\}_{1\leq i \leq n})$\\
}
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow \{\mathbf{x}_i[1][j]\}_{1\leq i \leq n}$\\
    \For{\texttt{s=} $2$ \texttt{to } $\epsilon_p=10$}
    {
        $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{\mathbf{y}_i[j]\}_{1\leq i \leq n},\{\mathbf{x}_i[s][j]\}_{1\leq i \leq n})$\\
    }
}
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\mathbf{y}_i[j]\}_{1\leq i \leq n})$\\
}

\algorithmicreturn{ $\{w_i\}_{1\leq i \leq n}$}
\end{algorithm}



\begin{algorithm}[!ht]
\caption{ Masked Comparison }
\label{algo:MaskedComparison}

\Input{$\{\mathbf{b}'_i\}_{1\leq i \leq n}$ where each $\mathbf{b}'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} \mathbf{b}'_i = \mathbf{b}'$,\\
$\{c'_i\}_{1\leq i \leq n}$ where each $c'_i \in \mathbb{R}_q^l$ and $\bigoplus_{i=1}^{n} c'_i = c'$,\\
publicly avilable $\mathbf{b}$ and $c$}
\Output{$\{b_i\}_{1\leq i \leq n}$ with each $b_i \in \{0,1\}$ such that $\bigoplus_{i=1}^{n} b_i = 1$ iff\\ $\mathbf{b}''=\mathbf{b}'>>(\epsilon_q-\epsilon_p)=3$ and $c''=c'>>(\epsilon_p-\epsilon_t)=6$, else $0$}
\BlankLine

//\texttt{for $\mathbf{b}$ part of ciphertext}\\
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    $\mathbf{eb}[j]\leftarrow(\mathbf{b}[j]<<3)+4$\\
    $\mathbf{b}'_{n+1}[j]\leftarrow \mathbf{eb}[j]$\\
     $\{\mathbf{y}_i[j]\}_{1\leq i \leq n+1}\leftarrow$ A2B$(\{\mathbf{b}'_i[j]\}_{1\leq i \leq n+1})$
}
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    \For{\texttt{s=} $1$ \texttt{to } $\epsilon_p=10$}
    {
        $\{\mathbf{x}_i[s][j]\}_{1\leq i \leq n+1}\leftarrow$ Bitslice$(\{\mathbf{y}_i[j]\}_{1\leq i \leq n+1}>>(s+3-1))$\\
        $\mathbf{x}_1[s][j]\leftarrow \mathbf{x}_1[s][j]\xor \mathbf{x}_{n+1}[s][j]$
    }    
}

//\texttt{for $c$ part of ciphertext}\\
$ec\leftarrow(c<<6)+64$\\
$c'_{n+1}\leftarrow ec$\\
$\{y_i\}_{1\leq i \leq n+1}\leftarrow$ A2B$(\{c'_i\}_{1\leq i \leq n+1})$

\For{\texttt{s=} $1$ \texttt{to } $\epsilon_t=4$}
{
    $\{z_i[s]\}_{1\leq i \leq n+1}\leftarrow$ Bitslice$(\{y_i\}_{1\leq i \leq n+1}>>(s+6-1))$\\
    $z_1[s]\leftarrow z_1[s]\xor z_{n+1}[s]$
}
//Combine the results of both parts of ciphertexts\\
$\{w_i\}_{1\leq i \leq n}\leftarrow \{z_i[1]\}_{1\leq i \leq n}$\\
\For{\texttt{s=} $2$ \texttt{to } $\epsilon_t=4$}
{
    $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\{z_i[s]\}_{1\leq i \leq n})$\\
}
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow \{\mathbf{x}_i[1][j]\}_{1\leq i \leq n}$\\
    \For{\texttt{s=} $2$ \texttt{to } $\epsilon_p=10$}
    {
        $\{\mathbf{y}_i[j]\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{\mathbf{y}_i[j]\}_{1\leq i \leq n},\{\mathbf{x}_i[s][j]\}_{1\leq i \leq n})$\\
    }
}
\For{\texttt{j=} $1$ \texttt{to } $l=3$}
{
    $\{w_i\}_{1\leq i \leq n}\leftarrow$ SecAnd$(\{w_i\}_{1\leq i \leq n},\mathbf{y}_i[j]\}_{1\leq i \leq n})$\\
}
\For{\texttt{j=} $\log_2 256-1$ \texttt{to } $0$}
{
    $\{w'_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n}>>2^j $\\
    $\{w_i\}_{1\leq i \leq n}\leftarrow w_{1\leq i \leq n} \mod(2^{2^j}-1)$\\
    $\{w_i\}_{1\leq i \leq n}\leftarrow SecAnd(\{w_i\}_{1\leq i \leq n}, \{w'_i\}_{1\leq i \leq n})$\\
}
\algorithmicreturn{ $\{w_i\}_{1\leq i \leq n}$}
\end{algorithm}


\begin{algorithm}[!ht]
\caption{ centered uniform Sampler }
\label{algo:UniformSampler}

\Input{$\{x_i\}$ where $x_i \in \mathbb{R}_2^u$ such that $\bigoplus_{i=0}^{n} x_i = x$}
\Output{$\{A_i\}_{0\leq i \leq n}$ where  $A_i \in \mathbb{R}_q$ and $\sum_{i=0}^{n} A_i =$ HW$(x)-$ HW$(y) \mod q $}
\BlankLine

$\{z_i\}_{0\leq i \leq n}\leftarrow$ SecBitAdd$(\{x_i\}_{0\leq i \leq n})$~\cite{FO-masked-saber} \\
$\{z_i\}_{0\leq i \leq n}\leftarrow$ SecBitSub$(\{z_i\}_{0\leq i \leq n},\{y_i\}_{0\leq i \leq n})$~\cite{Tobias2019_binomial_sampler} \\
$\{z_i\}_{0\leq i \leq n}\leftarrow$ SecConstAdd$(\{z_i\}_{0\leq i \leq n})$~\cite{FO-masked-saber}\\
$\{A_i\}_{0\leq i \leq n}\leftarrow$ B2A$(\{z_i\}_{0\leq i \leq n})$~\cite{Bettale2018_B2A}\\
$A_1\leftarrow A_1- \mu \mod q$\\

\algorithmicreturn{ $\{y_i\}_{0\leq i \leq n}$}
\end{algorithm}

